Unsupervised Learning for Human Sensing Using Radio Signals

There is a growing literature demonstrating the feasibility of using Radio Frequency (RF) signals to enable key computer vision tasks in the presence of occlusions and poor lighting. It leverages that RF signals traverse walls and occlusions to deliver through-wall pose estimation, action recognition, scene captioning, and human re-identification. However, unlike RGB datasets which can be labeled by human workers, labeling RF signals is a daunting task because such signals are not human interpretable. Yet, it is fairly easy to collect unlabelled RF signals. It would be highly beneficial to use such unlabeled RF data to learn useful representations in an unsupervised manner. Thus, in this paper, we explore the feasibility of adapting RGB-based unsupervised representation learning to RF signals. We show that while contrastive learning has emerged as the main technique for unsupervised representation learning from images and videos, such methods produce poor performance when applied to sensing humans using RF signals. In contrast, predictive unsupervised learning methods learn high-quality representations that can be used for multiple downstream RF-based sensing tasks. Our empirical results show that this approach outperforms state-of-the-art RF-based human sensing on various tasks, opening the possibility of unsupervised representation learning from this novel modality.

==> source/ablation.tex <==
\subsection{Ablation Study on Reconstructive Tasks}
\label{sec:ablation}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c| c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}}c  @{\hspace{0.2cm}}c}\hline
  &  RF-MMD & \multicolumn{2}{c}{Colorful-MNIST}  \\
\hline
Recon. Tasks & Pose Err.   & \begin{tabular}{@{}c@{}}digit cls. \\ error rate\end{tabular} & \begin{tabular}{@{}c@{}}bkgd cls. \\ error rate\end{tabular}  &  \\
\hline
No Recon. & 80.5 & 85.1  & 51.5 \\
\hline
Colorization & N/A & 39.9 & 54.5 \\
Jigsaw Puzzle & N/A & 22.9 & 59.3\\
\hline
Autoencoder & 51.1  & 34.4 & 57.1 \\
Inpainting & 46.6 & 11.7 & 54.0 \\
\hline
\end{tabular}
\caption{Evaluation of different reconstructive tasks.}
\label{tab:ablation}
\end{table}


In \name, we choose the inpainting task for the reconstructive branch. However, other reconstructive tasks can be potentially used for the reconstructive branch. In this section, we evaluate the performance of \name~with different reconstructive tasks including inpainting, auto-encoder, colorization \cite{zhang2016colorful}, and Jigsaw Puzzle \cite{noroozi2016unsupervised}. Table \ref{tab:ablation} shows \name's performance using different reconstructive task on RF-based 3D pose estimation (RF-MMD) and Colorful-MNIST under the fixed feature extractor setting. As shown in the table, all reconstructive tasks significantly reduce errors in comparison to using contrastive learning without any reconstruction task.  The table also shows that inpaintaing compares favorably to other tasks and works across modalities. Hence, we use inpainting as the default reconstructive task  in IPCL. 


==> source/abstract.tex <==
%Unsupervised Learning aims to learn useful feature representations for various downstream tasks from massive unlabelled datasets. However, most published works focus on learning features from Image, Video or Language data. In this paper, we introduce an unsupervised learning approach to learn representations from wireless datasets.


%There is a growing literature demonstrating the feasibility of sensing humans with Radio Frequency (RF) signals. Past papers have shown that RF signals can be used to estimate human skeletons, recognize their actions, or extract identifiable features for person re-identification with high accuracy, even when the person is behind occlusions or under poor lighting conditions. However, unlike vision-based datasets which can typically be labeled by human workers, collecting fully-annotated datasets for RF signals is a daunting task, as RF signals are not human interpretable. As a result, there exists a huge amount of unlabeled RF data which can potentially improves the performance of existing RF-based human sensing models if we can use unsupervised learning to learn useful representations from it. In this paper, we propose predictive-contrastive learning (PreCLR), a novel unsupervised learning method which enables learning high-quality representations for RF-based human sensing from large-scale unlabeled RF datasets. We also demonstrates that, unlike traditional contrastive learning methods, our proposed PreCLR can learn high-quality representation for multiple types of semantics that can be used for different downstream tasks. Our empirical results show that our approach improves RF-based human sensing performances on various tasks and outperforms state-of-the-art unsupervised learning approaches on both synthetic and real-world datasets.

% ---- RF-focused abstract -------
%There is a growing literature demonstrating the feasibility of leveraging Radio Frequency (RF) signals to address key computer vision tasks, in the presence of occlusions and poor lighting conditions. Past papers have shown that RF signals can be used for pose estimation, action recognition, scene captioning, and human re-identification though walls and in dark settings.  However, unlike vision-based datasets which can be labeled by human workers, labeling RF signals is a daunting task because such signals are not human interpretable. Yet, it is fairly easy to collect unlabelled RF signals. Ideally, one would like to leverage such unlabeled RF data to learn useful representations that can improve the accuracy of the aforementioned tasks. 
%
%In this paper, we propose predictive-contrastive learning (PreCLR), a novel unsupervised learning method that learns high-quality representations for RF-based human sensing tasks. While, contrastive learning has emerged as the main technique for unsupervised representation learning from images and videos, we show that such method produces poor performance and cannot generalize to multiple downstream tasks. In contrast, PreCLR  learns high-quality representations for multiple types of semantics that can be used for different downstream tasks. Our empirical results show that our approach improves RF-based human sensing performance on various tasks and outperforms state-of-the-art unsupervised learning approaches on both synthetic and real-world datasets.


% ---- Contrastive learning focused abstract -------

Contrastive learning is very effective at learning useful representations without supervision. Yet contrastive learning has its limitations. It may learn a shortcut that is irrelevant to the downstream task, and discard relevant information. Past work has addressed this limitation via custom data augmentations that eliminate the shortcut. This solution however does not work for data modalities that are not interpretable by humans, e.g., radio signals. For such modalities, it is hard for a human to guess which shortcuts may exist in the signal, or how they can be eliminated. Even for interpretable data like RGB, sometimes eliminating the shortcut may be undesirable. The shortcut may be irrelevant to one downstream task but important to another.  In this case, it is desirable to learn a representation that captures both the shortcut information and the information relevant to the other downstream task.  This paper presents information-preserving contrastive learning (IPCL), a new framework for unsupervised representation learning  that preserves relevant information even in the presence of shortcuts.  We empirically show that the representations learned by IPCL outperforms contrastive learning in supporting different modalities and multiple downstream tasks.  







%Contrastive learning is very effective at learning useful representations without supervision. Yet contrastive learning has its limitations. It can focus on a shortcut (e.g., color distribution) that is irrelevant to the downstream task, and discard relevant information. Past work has addressed this limitation via custom data augmentations that eliminate the shortcut (e.g., color distorted augmentations). This solution however does not work when the data modality is not interpretable by humans, e.g., through-wall pose estimation using radio signals. In this case, it is hard for a human to know which shortcuts may exist or how to alter the radio signals to eliminate the shortcuts. Even for visual data, sometimes eliminating the shortcut may be undesirable. The shortcut may be relevant to one downstream task but irrelevant to another.  In this case, one may be interested in generating a single representation that works for both downstream tasks and hence wants to preserve the shortcut features as well as the features relevant to the other task. This paper presents information-preserving contrastive learning (IPCL), a new framework for unsupervised representation learning that preserves relevant information even in the presence of shortcuts.  We empirically show that IPCL addresses the above problems and outperforms contrastive learning on radio signals and learning from RGB data representation with different features that support different downstream tasks. 








==> source/checklist.tex <==
\section*{Checklist}

%%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
\answerYes{}
  \item Did you describe the limitations of your work?
\answerYes{We discuss the limitations in the Concluding Remarks section.}
  \item Did you discuss any potential negative societal impacts of your work?
\answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
\answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
\answerNA{}
	\item Did you include complete proofs of all theoretical results?
\answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
\answerNo{Code will be released upon acceptance of the paper.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
\answerYes{Please see the implementation details section in the appendix.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{We found our results to be very stable between runs, and omitted standard errors because of space constraints.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
\answerYes{Please see the implementation details section in the appendix.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
\answerYes
  \item Did you mention the license of the assets?
\answerYes{Here we list all license that we can find. MPII is licensed under the Simplified BSD License. FairFace is licensed under License: CC BY 4.0..}
  \item Did you include any new assets either in the supplemental material or as a URL?
\answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
\answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
\answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
\answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
\answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
\answerNA{}
\end{enumerate}

\end{enumerate}

==> source/experiment-rf-10.tex <==
\section{Evaluation on RF Datasets}
\label{sec:rf-exp}
We evaluate \name~on three through-wall RF sensing tasks: pose estimation, action recognition, and re-identification. 

\vspace{-2pt}\noindent\textbf{RF Datasets.} We pre-train \name~on two real-world RF datasets: RF-MMD \cite{li2019making} and RRD \cite{fan2020learning}. RF-MMD is an RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  863 RF sequences from 100 different identities at 5 different locations on a campus, and 6305 RF sequences from 38 different identities in 19 homes.

\vspace{-2pt}\noindent\textbf{Evaluation Metrics.}  We use the performance metrics used by past work for each task. Specifically, for 3D pose estimation, we use the 3D pose error as the evaluation metric. For action recognition, we use mean average precision (mAP) at different IoU thresholds $\theta$ to evaluate the model. For person re-identification, we report the mAP and the cumulative matching characteristic (CMC) at rank-1 and rank-5. Detailed explanations of these evaluation metrics are provided in the Appendix.

\vspace{-2pt}\noindent\textbf{Evaluation Settings.} 
We evaluate the performance of \name~and baselines under both fixed feature extractor setting and fine-tuning setting. In the fixed feature extractor setting, we use the pre-trained RF feature extractor as initialization of the RF feature extractor for each downstream task, and only those task-specific sub-networks (Fig. \ref{fig:rf-framework}) are trained during downstream task training. In the fine-tuning setting, we fine-tune the whole model on the downstream task. 
%We use the RF-MMD dataset for downstream tasks of pose estimation and action recognition, and the RRD dataset for person re-identification. 


\vspace{-2pt}\noindent\textbf{Baselines.} Since there is no prior work that applies existing contrastive learning methods on RF data, we implement SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, CPC \cite{henaff2019data} and BYOL \cite{grill2020bootstrap} on RF data by ourselves as baselines. We also train a supervised baseline from scratch for the fine-tuning setting, and a randomly initialized RF feature extractor serves as a baseline for the fixed feature extractor setting. Detailed implementations of the baselines are provided in the Appendix.


\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l | c |c c|c c c|c c c}
%\hline
\toprule[1.5pt]
  Tasks & 3D Pose Estimation & \multicolumn{2}{c|}{Action Recognition} & \multicolumn{3}{c|}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
\midrule
 \multirow{ 2}{*}{Metrics} &  \multirow{ 2}{*}{Pose \textsc{Err}.$^\downarrow$ (mm)} & \multicolumn{2}{c|}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ & & & & & & \\
\midrule\midrule
Random init & 60.1 & 70.5  & 53.3 & 28.1 & 43.8 & 68.8 & 30.1 & 54.2 & 74.6 \\
\midrule
SimCLR & 80.5 & 4.2 & 0 & 29.8 & 44.1 & 67.5 & 31.2 & 55.1 & 73.8 \\
MoCo & 77.2 & 5.1 & 0.18 & 29.1 & 44.7 & 65.3 & 30.5 & 54.5 & 74.0 \\
CPC & 78.7 & 3.6 & 0 & 30.0 & 42.7 & 69.5 & 30.7 & 54.0 & 75.3 \\
BYOL & 79.3 & 4.7 & 0 & 29.5 & 44.4 & 66.7 & 30.7 & 54.6 & 73.5 \\
%Inpainting & 51.1 & 72.3 & 65.5 & 49.8 & 73.1 & 90.5 & 38.5 & 64.2 & 84.7 \\
\midrule
\textbf{\name(ours)} & \textbf{46.6} & \textbf{86.5} & \textbf{83.1} & \textbf{54.5} & \textbf{78.7} & \textbf{93.0} & \textbf{43.3} & \textbf{72.4} & \textbf{87.6}\\
\bf \textsc{Improvement} 
& \textcolor{darkgreen}{\textbf{-30.6}} 
 & \textcolor{darkgreen}{\textbf{+81.4}} 
 & \textcolor{darkgreen}{\textbf{+82.9}} 
 & \textcolor{darkgreen}{\textbf{+24.5}}  
 & \textcolor{darkgreen}{\textbf{+34.0}} 
 & \textcolor{darkgreen}{\textbf{+23.5}} 
 & \textcolor{darkgreen}{\textbf{+11.8}}
 & \textcolor{darkgreen}{\textbf{+17.3}} 
 & \textcolor{darkgreen}{\textbf{+12.3}}  
\\\midrule\midrule
\textsc{Supervised} & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
%\hline
\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-5pt}
\caption{\footnotesize{Evaluation of different models on different RF tasks under fixed feature extractor setting.
%where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and the weights are frozen during downstream training. 
$\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}}
\label{tab:result-fixed}
\vspace{5pt}
%\end{table*}

%\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l | c |c c|c c c|c c c}
%\hline
\toprule[1.5pt]
  Tasks & 3D Pose Estimation & \multicolumn{2}{c|}{Action Recognition} & \multicolumn{3}{c|}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
\midrule
 \multirow{ 2}{*}{Metrics} &  \multirow{ 2}{*}{Pose \textsc{Err}.$^\downarrow$ (mm)} & \multicolumn{2}{c|}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ & & & & & & \\
\midrule\midrule
Random init & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
\midrule
SimCLR & 38.8 & 89.8 & 87.4 & 59.0 & 81.7 & 94.1 & 45.9 & 73.8 & 88.5 \\
MoCo & 38.3 & 89.7 & 87.2 & 59.3 & 82.0 & 94.5 & 46.4 & 74.3 & 89.7 \\
CPC & 38.6 & 89.9 & 87.5 & 59.4 & 81.5 & 94.0 & 46.0 & 74.5 & 89.1 \\
BYOL & 38.5 & 89.7 & 87.2 & 59.4 & 81.9 & 94.5 & 46.6 & 74.5 & 89.5 \\
%Inpainting & 36.2 &  91.7 & 88.7 & 60.1 & 83.3 & 95.5 & 47.5 & 75.3 & 90.3\\
\midrule
\textbf{\name (ours)} & \textbf{35.1} & \textbf{92.5} & \textbf{89.6} & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} & \textbf{48.1} & \textbf{76.1} & \textbf{91.0}\\
\bf \textsc{Improvement} 
& \textcolor{darkgreen}{\textbf{-3.7}} 
 & \textcolor{darkgreen}{\textbf{+2.6}} 
 & \textcolor{darkgreen}{\textbf{+2.1}}  
 & \textcolor{darkgreen}{\textbf{+1.4}}  
 & \textcolor{darkgreen}{\textbf{+2.2}}  
 & \textcolor{darkgreen}{\textbf{+1.5}}  
 & \textcolor{darkgreen}{\textbf{+1.5}}  
 & \textcolor{darkgreen}{\textbf{+1.6}}  
 & \textcolor{darkgreen}{\textbf{+1.3}}  \\

\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-5pt}
\caption{\footnotesize{Evaluation of different models on different RF tasks under fine-tuning setting.
%where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and then fine-tuned during downstream training. 
$\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}}
\label{tab:result-finetune}
\vspace{-15pt}
\end{table*}

\vspace{-2pt}
\subsection{RF Results}
We evaluate the RF feature extractor learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-fixed} and \ref{tab:result-finetune}. Under the fixed feature extractor setting, \name~ is the only method that is comparable to supervised training. Under the fine-tuning setting, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus, and 3.6\% relative improvement on RRD-Home.

The tables also show that the feature network pre-trained using contrastive learning alone can generate worse results than random initialization. This is likely due to that contrastive learning learns from the Rf signal shortcuts that are irrelevant to human sensing, and thus are harmful to human-related downstream tasks. 


%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
%& $\theta=0.1$ & $\theta=0.5$ \\
%\hline
%Train from Scratch & 90.1  & 87.8 \\
%Contrastive+finetune & 89.8 & 87.4 \\
%Reconstructive+finetune & 91.7 & 88.7 \\
%\name+finetune & \textbf{92.5} & \textbf{89.6} \\
%\hline
%\end{tabular}
%\caption{Action recognition performance of different models on RF-MMD in mAP at different IoU thresholds (the higher the better).}
%\label{tab:result-action}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 59.5 & 82.1 & 95.5 \\
%Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
%Reconstructive+finetune & 60.1 & 83.3 & 95.5  \\
%\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Campus in mAP and CMC (the higher the better).}
%\label{tab:result-reid-campus}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 46.4 & 74.6 & 89.5 \\
%Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
%Reconstructive+finetune & 47.5 & 75.3 & 90.3 \\
%\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Home in mAP and CMC (the higher the better).}
%\label{tab:result-reid-home}
%\vspace{-5pt}
%\end{table}



%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{featreid}
%\end{center}
%\caption{Feature visualization of SimCLR and IPCL using tSNE on RF-RRD-Home.}\label{fig:reid-tsne}
%\vskip -0.1in
%\end{figure}

%We also visualize the features learned by SimCLR and \name~ in Figure \ref{fig:image-tsne} using tSNE on RF-RRD-Home dataset, colored by person identities. As shown in the figure, features learned by SimCLR cannot form clusters when colored using person identities, while features learned by \name shows clear clustering. This  shows that contrastive learning will fall into unknown shortcut that can be totally irrelevant to downstream tasks on RF dataset, while \name~can avoid learning only the shortcut and generate high-quality features.
%



==> source/experiment-rf-11.tex <==
\section{Evaluation on RF Datasets}
\label{sec:rf-exp}
\red{To further demonstrate that \name~works well for non-interpretable modality, which can hardly design effective data augmentations for contrastive learning,} we evaluate \name~on three through-wall RF sensing tasks: \red{3D} pose estimation, action recognition, and re-identification. 

\vspace{-2pt}\noindent\textbf{RF Datasets.} We pretrain \name~on two real-world RF datasets: RF-MMD \cite{li2019making} and RRD \cite{fan2020learning}. RF-MMD is an RF-based \red{3D} pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  863 RF sequences from 100 different identities at 5 different locations on a campus, and 6305 RF sequences from 38 different identities in 19 homes.

\vspace{-2pt}\noindent\textbf{Evaluation Metrics.}  \red{We follow the standard evaluation metrics as previous works for each task.} Specifically, for 3D pose estimation, we use the 3D pose error as the evaluation metric. For action recognition, we use mean average precision (mAP) at different IoU thresholds $\theta$ to evaluate the model. For person re-identification, we report the mAP and the cumulative matching characteristic (CMC) at rank-1 and rank-5. Detailed explanations of these evaluation metrics are provided in the Appendix.


% \vspace{-2pt}\noindent\textbf{\name~ can learn better representation for multiple downstream tasks without elaborate designing of data augmentation.}
\vspace{-2pt}
\subsection{\name~ can learn better representation for multiple downstream tasks without elaborate designing of data augmentation.}
\red{Since there is no prior work that applies existing contrastive learning methods on RF data, we implement SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, CPC \cite{henaff2019data} and BYOL \cite{grill2020bootstrap} on RF data by ourselves as baselines. We first evaluate the performance of the fixed feature extractor setting, in which we fix the pre-trained RF feature extractor for each downstream task, and only train those task-specific sub-networks (Fig. \ref{fig:rf-framework}) during each downstream task training. We also report the results with a fixed random initialized RF feature extractor as well as the supervised results of each task for comparison. The results are shown in Table \ref{tab:result-fixed}. 
}

\red{From Table \ref{tab:result-fixed}, all the contrastive pretraining methods perform much worse on all the downstream tasks, even much worse than random initialization for the 3D pose estimation and action recognition tasks. It is obvious that the shortcut happens since a good contrastive pretraining can not generalize to downstream tasks. It is likely due to several reasons. First, the non-interpretable property of RF signals makes that through elaborate designing of data augmentation operations to remove shortcuts is infeasible. Second, the downstream tasks are much complicated than the contrastive pretraining task which simply distinguishes the positive and negative views. Contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related downstream tasks. However, \name~works much better on all the downstream tasks, and even comparable to the supervised training results. The above results show that \name~is a type of auto-encoder to retain as much as information for downstream tasks, while enforcing the latent codes to have the ``contrastive'' property for better feature representation. It can automatically retain useful information without elaborate designing of data augmentation for specific tasks compared with other contrastive methods.    
}

\vspace{-2pt}
\subsection{\name~ can perform better than supervised learning counterpart of several RF-based tasks for the first time.}
\red{We also evaluate the performance of \name~and baselines under the fine-tuning setting, in which we first initialize the feature extractor network using the pre-trained model and then fine-tune the whole network for each downstream task. Experimental results are shown in Table \ref{tab:result-finetune}. Under the fine-tuning setting, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus, and 3.6\% relative improvement on RRD-Home. However, all the other pre-trained contrastive models work slightly worse than the random initialization method. We for the first time make the self-supervised learning pretraining work on the RF data and consistently work on several different tasks. 
}


% \vspace{-2pt}\noindent\textbf{Evaluation Settings.} 
% We evaluate the performance of \name~and baselines under both fixed feature extractor setting and fine-tuning setting. In the fixed feature extractor setting, we use the pre-trained RF feature extractor as initialization of the RF feature extractor for each downstream task, and only those task-specific sub-networks (Fig. \ref{fig:rf-framework}) are trained during downstream task training. In the fine-tuning setting, we fine-tune the whole model on the downstream task. 
% %We use the RF-MMD dataset for downstream tasks of pose estimation and action recognition, and the RRD dataset for person re-identification. 


% \vspace{-2pt}\noindent\textbf{Baselines.} Since there is no prior work that applies existing contrastive learning methods on RF data, we implement SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, CPC \cite{henaff2019data} and BYOL \cite{grill2020bootstrap} on RF data by ourselves as baselines. We also train a supervised baseline from scratch for the fine-tuning setting, and a randomly initialized RF feature extractor serves as a baseline for the fixed feature extractor setting. Detailed implementations of the baselines are provided in the Appendix.


\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l | c |c c|c c c|c c c}
%\hline
\toprule[1.5pt]
  Tasks & 3D Pose Estimation & \multicolumn{2}{c|}{Action Recognition} & \multicolumn{3}{c|}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
\midrule
 \multirow{ 2}{*}{Metrics} &  \multirow{ 2}{*}{Pose \textsc{Err}.$^\downarrow$ (mm)} & \multicolumn{2}{c|}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ & & & & & & \\
\midrule\midrule
Random init & 60.1 & 70.5  & 53.3 & 28.1 & 43.8 & 68.8 & 30.1 & 54.2 & 74.6 \\
\midrule
SimCLR & 80.5 & 4.2 & 0 & 29.8 & 44.1 & 67.5 & 31.2 & 55.1 & 73.8 \\
MoCo & 77.2 & 5.1 & 0.18 & 29.1 & 44.7 & 65.3 & 30.5 & 54.5 & 74.0 \\
CPC & 78.7 & 3.6 & 0 & 30.0 & 42.7 & 69.5 & 30.7 & 54.0 & 75.3 \\
BYOL & 79.3 & 4.7 & 0 & 29.5 & 44.4 & 66.7 & 30.7 & 54.6 & 73.5 \\
%Inpainting & 51.1 & 72.3 & 65.5 & 49.8 & 73.1 & 90.5 & 38.5 & 64.2 & 84.7 \\
\midrule
\textbf{\name(ours)} & \textbf{46.6} & \textbf{86.5} & \textbf{83.1} & \textbf{54.5} & \textbf{78.7} & \textbf{93.0} & \textbf{43.3} & \textbf{72.4} & \textbf{87.6}\\
\bf \textsc{Improvement} 
& \textcolor{darkgreen}{\textbf{-30.6}} 
 & \textcolor{darkgreen}{\textbf{+81.4}} 
 & \textcolor{darkgreen}{\textbf{+82.9}} 
 & \textcolor{darkgreen}{\textbf{+24.5}}  
 & \textcolor{darkgreen}{\textbf{+34.0}} 
 & \textcolor{darkgreen}{\textbf{+23.5}} 
 & \textcolor{darkgreen}{\textbf{+11.8}}
 & \textcolor{darkgreen}{\textbf{+17.3}} 
 & \textcolor{darkgreen}{\textbf{+12.3}}  
\\\midrule\midrule
\textsc{Supervised} & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
%\hline
\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-5pt}
\caption{\footnotesize{Evaluation of different models on different RF tasks under fixed feature extractor setting.
%where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and the weights are frozen during downstream training. 
$\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}}
\label{tab:result-fixed}
\vspace{5pt}
%\end{table*}

%\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l | c |c c|c c c|c c c}
%\hline
\toprule[1.5pt]
  Tasks & 3D Pose Estimation & \multicolumn{2}{c|}{Action Recognition} & \multicolumn{3}{c|}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
\midrule
 \multirow{ 2}{*}{Metrics} &  \multirow{ 2}{*}{Pose \textsc{Err}.$^\downarrow$ (mm)} & \multicolumn{2}{c|}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ & & & & & & \\
\midrule\midrule
Random init & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
\midrule
SimCLR & 38.8 & 89.8 & 87.4 & 59.0 & 81.7 & 94.1 & 45.9 & 73.8 & 88.5 \\
MoCo & 38.3 & 89.7 & 87.2 & 59.3 & 82.0 & 94.5 & 46.4 & 74.3 & 89.7 \\
CPC & 38.6 & 89.9 & 87.5 & 59.4 & 81.5 & 94.0 & 46.0 & 74.5 & 89.1 \\
BYOL & 38.5 & 89.7 & 87.2 & 59.4 & 81.9 & 94.5 & 46.6 & 74.5 & 89.5 \\
%Inpainting & 36.2 &  91.7 & 88.7 & 60.1 & 83.3 & 95.5 & 47.5 & 75.3 & 90.3\\
\midrule
\textbf{\name (ours)} & \textbf{35.1} & \textbf{92.5} & \textbf{89.6} & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} & \textbf{48.1} & \textbf{76.1} & \textbf{91.0}\\
\bf \textsc{Improvement} 
& \textcolor{darkgreen}{\textbf{-3.7}} 
 & \textcolor{darkgreen}{\textbf{+2.6}} 
 & \textcolor{darkgreen}{\textbf{+2.1}}  
 & \textcolor{darkgreen}{\textbf{+1.4}}  
 & \textcolor{darkgreen}{\textbf{+2.2}}  
 & \textcolor{darkgreen}{\textbf{+1.5}}  
 & \textcolor{darkgreen}{\textbf{+1.5}}  
 & \textcolor{darkgreen}{\textbf{+1.6}}  
 & \textcolor{darkgreen}{\textbf{+1.3}}  \\

\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-5pt}
\caption{\footnotesize{Evaluation of different models on different RF tasks under fine-tuning setting.
%where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and then fine-tuned during downstream training. 
$\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}}
\label{tab:result-finetune}
\vspace{-15pt}
\end{table*}

% \vspace{-2pt}
% \subsection{RF Results}
% We evaluate the RF feature extractor learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-fixed} and \ref{tab:result-finetune}. Under the fixed feature extractor setting, \name~ is the only method that is comparable to supervised training. Under the fine-tuning setting, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus, afnd 3.6\% relative improvement on RRD-Home.

% The tables also show that the feature network pre-trained using contrastive learning alone can generate worse results than random initialization. This is likely due to that contrastive learning learns from the Rf signal shortcuts that are irrelevant to human sensing, and thus are harmful to human-related downstream tasks. 


%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
%& $\theta=0.1$ & $\theta=0.5$ \\
%\hline
%Train from Scratch & 90.1  & 87.8 \\
%Contrastive+finetune & 89.8 & 87.4 \\
%Reconstructive+finetune & 91.7 & 88.7 \\
%\name+finetune & \textbf{92.5} & \textbf{89.6} \\
%\hline
%\end{tabular}
%\caption{Action recognition performance of different models on RF-MMD in mAP at different IoU thresholds (the higher the better).}
%\label{tab:result-action}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 59.5 & 82.1 & 95.5 \\
%Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
%Reconstructive+finetune & 60.1 & 83.3 & 95.5  \\
%\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Campus in mAP and CMC (the higher the better).}
%\label{tab:result-reid-campus}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 46.4 & 74.6 & 89.5 \\
%Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
%Reconstructive+finetune & 47.5 & 75.3 & 90.3 \\
%\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Home in mAP and CMC (the higher the better).}
%\label{tab:result-reid-home}
%\vspace{-5pt}
%\end{table}



%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{featreid}
%\end{center}
%\caption{Feature visualization of SimCLR and IPCL using tSNE on RF-RRD-Home.}\label{fig:reid-tsne}
%\vskip -0.1in
%\end{figure}

%We also visualize the features learned by SimCLR and \name~ in Figure \ref{fig:image-tsne} using tSNE on RF-RRD-Home dataset, colored by person identities. As shown in the figure, features learned by SimCLR cannot form clusters when colored using person identities, while features learned by \name shows clear clustering. This  shows that contrastive learning will fall into unknown shortcut that can be totally irrelevant to downstream tasks on RF dataset, while \name~can avoid learning only the shortcut and generate high-quality features.
%



==> source/experiment-rf-2.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. Our \name~ framework has two branches: Predictive Branch and Contrastive Branch. For the predictive branch, we randomly mask some frames across time for prediction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and use the given ROI align to crop out regions containing humans. The predictive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear head to generate normalized features. The combined loss of predictive learning and contrastive learning is used to train the model.}\label{fig:model-toy}
\end{figure*}


\section{Experiments on RF Datasets}
In this section, we evaluate \name~on real-world RF datasets to show its effectiveness of learning multiple fine-grained semantics. We first apply \name~on large unlabeled RF datasets to train a feature extractor for RF signals, and then evaluate its performance on multiple downstream RF-based human sensing tasks, including pose estimation, action recognition, and human identification.


\subsection{RF-based Human Sensing Framework}
We first introduce the general framework used for various RF-based human sensing tasks, which is illustrated in Figure~\ref{fig:rf-framework}. It first uses a spatio-temporal convolutional feature network to extract features from  input RF frames. It will then crop out the region of interest around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features for downstream tasks, such as pose estimation, action recognition or person re-identification. The feature network structure is typically the same for all tasks, while different tasks can have different sub-network structure specifically designed for each task. The goal of RF-based unsupervised learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{Typical RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and then use ROI Align with the given bounding box to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\subsection{\name~on RF Representation}

As shown in Figure \ref{model-rf}, for contrastive training on RF signals, the anchor and positive sample shares the same input RF frames with different random jitter of its bounding boxes. Negative samples of an anchor sample are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment, so that the environment will not be a shortcut to easily distinguish positive and negative samples. The inpainting task in this case, we consider a sequence of RF frames and randomly mask out some  some segments with random length in it and fill them with zero.

During the unsupervised learning phase, we employ a standard spatio-temporal RF feature extraction network to encode the input RF heatmaps. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from human detection algorithm of WiTrack \cite{xxx}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layer is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the inpainting task, a decoder is added to reconstruct the original RF heatmaps, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed heatmaps and the ground truth heatmaps without temporal mask. For \name, we combine these two losses together to be $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$ in our RF-based experiments.

\subsection{Experiment Setup}
We pre-train \name on two RF datasets: RF-MMD \cite{xxx} and RRD \cite{xxx}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF clips from 100 different identities at 5 different locations on a university campus, and 6305 RF clips from 38 different identities in 19 different homes.

After the contrastive pre-training phase, to evaluate the quality of the learned representation, we apply the learned RF feature extraction network in three different downstream RF-based human sensing tasks: 3D pose estimation, action recognition, and person re-identification. In this downstream training phase, we use the pre-trained RF feature extraction network as initialization of RF feature extractor for each downstream task and fine-tune the model for each task on downstream datasets. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. We also train a supervised baseline from scratch on the same data for each task to compare with the results of unsupervised learning. 

\subsection{Downstream Evaluation Results}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & Skeleton Err. (mm) \\
\hline
Train from Scratch & 3.84 \\
Contrastive+finetune & 3.88 \\
Predictive+finetune & 3.62 \\
\name+finetune & \textbf{3.51} \\
\hline
\end{tabular}
\caption{3D pose estimation error of different models on RF-MMD.}
\label{tab:result-pose}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
& $\theta=0.1$ & $\theta=0.5$ \\
\hline
Train from Scratch & 90.1  & 87.8 \\
Contrastive+finetune & 89.8 & 87.4 \\
Predictive+finetune & 91.7 & 88.7 \\
\name+finetune & \textbf{92.5} & \textbf{89.6} \\
\hline
\end{tabular}
\caption{Action recognition mAP of different models at different thresholds on RF-MMD.}
\label{tab:result-action}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 59.5 & 82.1 & 95.5 \\
Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
Predictive+finetune & 60.1 & 83.3 & 95.5  \\
\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Campus.}
\label{tab:result-reid-campus}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 46.4 & 74.6 & 89.5 \\
Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
Predictive+finetune & 47.5 & 75.3 & 90.3 \\
\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Home.}
\label{tab:result-reid-home}
\end{table}

We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-pose}, \ref{tab:result-action}, \ref{tab:result-reid-campus}, \ref{tab:result-reid-home}. As shown in the results, pre-training the feature network using \name~and fine-tuning it on downstream task  generates the best results in all tasks. Feature network pre-trained by contrastive learning alone generates worse results than random initialization. This may be because contrastive learning learns semantics irrelevant to human and thus is harmful to human-related semantics. Predictive learning can generate better results than training from scratch, but since the features learnt by predictive learning alone is too low-level, the performance is worse than that of PCL which is able to utilize contrastive learning to learn fine-grained high-level features. This demonstrate that the RF feature extraction network learnt by \name~can extract representations that contains multiple fine-grained semantics related to different downstream tasks.


==> source/experiment-rf-3.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. It has two branches: Predictive Branch and Contrastive Branch. For the predictive branch, we randomly mask some frames across time for prediction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and use the given ROI align to crop out regions containing humans. The predictive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear head to generate normalized features. The combined loss of predictive learning and contrastive learning is used to train the model.}\label{fig:model-toy}
\end{figure*}


\section{Experiments on RF Datasets}
In this section, we evaluate \name~on real-world RF datasets to show its effectiveness of learning multiple types of fine-grained semantics. We first apply \name~on large unlabeled RF datasets to train a feature extractor for RF signals, and then evaluate its performance on multiple downstream RF-based human sensing tasks, including pose estimation, action recognition, and human identification.


\subsection{RF-based Human Sensing Framework}
We first introduce the general framework used for various RF-based human sensing tasks, which is illustrated in Figure~\ref{fig:rf-framework}. It first uses a spatio-temporal convolutional feature network to extract features from  input RF frames. It will then crop out the region of interest around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features for downstream tasks, such as pose estimation, action recognition or person re-identification. The feature network structure is typically the same for all tasks, while different tasks can have different sub-network structure specifically designed for each task. The goal of RF-based unsupervised learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{Typical RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and then use ROI Align with the given bounding box to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\subsection{\name~on RF Representation}

As shown in Figure \ref{model-rf}, for contrastive training on RF signals, the anchor and positive sample shares the same input RF frames with different random jitter of its bounding boxes. Negative samples of an anchor sample are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment, so that the environment will not be a shortcut to easily distinguish positive and negative samples. The inpainting task in this case, we consider a sequence of RF frames and randomly mask out some  some segments with random length in it and fill them with zero.

During the unsupervised learning phase, we employ a standard spatio-temporal RF feature extraction network to encode the input RF heatmaps. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from human detection algorithm of WiTrack \cite{xxx}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layer is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the inpainting task, a decoder is added to reconstruct the original RF heatmaps, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed heatmaps and the ground truth heatmaps without temporal mask. For \name, we combine these two losses together to be $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$ in our RF-based experiments.

\subsection{Experiment Setup}
We pre-train \name on two RF datasets: RF-MMD \cite{xxx} and RRD \cite{xxx}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF clips from 100 different identities at 5 different locations on a university campus, and 6305 RF clips from 38 different identities in 19 different homes.

After the contrastive pre-training phase, to evaluate the quality of the learned representation, we apply the learned RF feature extraction network in three different downstream RF-based human sensing tasks: 3D pose estimation, action recognition, and person re-identification. In this downstream training phase, we use the pre-trained RF feature extraction network as initialization of RF feature extractor for each downstream task and fine-tune the model for each task on downstream datasets. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. We also train a supervised baseline from scratch on the same data for each task to compare with the results of unsupervised learning. 

\subsection{Downstream Evaluation Results}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & Skeleton Err. (mm) \\
\hline
Train from Scratch & 3.84 \\
Contrastive+finetune & 3.88 \\
Predictive+finetune & 3.62 \\
\name+finetune & \textbf{3.51} \\
\hline
\end{tabular}
\caption{3D pose estimation error of different models on RF-MMD.}
\label{tab:result-pose}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
& $\theta=0.1$ & $\theta=0.5$ \\
\hline
Train from Scratch & 90.1  & 87.8 \\
Contrastive+finetune & 89.8 & 87.4 \\
Predictive+finetune & 91.7 & 88.7 \\
\name+finetune & \textbf{92.5} & \textbf{89.6} \\
\hline
\end{tabular}
\caption{Action recognition mAP of different models at different thresholds on RF-MMD.}
\label{tab:result-action}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 59.5 & 82.1 & 95.5 \\
Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
Predictive+finetune & 60.1 & 83.3 & 95.5  \\
\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Campus.}
\label{tab:result-reid-campus}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 46.4 & 74.6 & 89.5 \\
Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
Predictive+finetune & 47.5 & 75.3 & 90.3 \\
\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Home.}
\label{tab:result-reid-home}
\end{table}

We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-pose}, \ref{tab:result-action}, \ref{tab:result-reid-campus}, \ref{tab:result-reid-home}. As shown in the results, pre-training the feature network using \name~and fine-tuning it on downstream task  generates the best results in all tasks. Feature network pre-trained by contrastive learning alone generates worse results than random initialization. This may be because contrastive learning learns semantics irrelevant to human and thus is harmful to human-related semantics. Predictive learning can generate better results than training from scratch, but since the features learnt by predictive learning alone is too low-level, the performance is worse than that of PCL which is able to utilize contrastive learning to learn fine-grained high-level features. This demonstrate that the RF feature extraction network learnt by \name~can extract representations that contains multiple fine-grained semantics related to different downstream tasks.


==> source/experiment-rf-4.tex <==
\section{Learning Unsupervised Representations from RF Signals}
Radio Frequency (RF) signals have been used for pose estimation, action recognition, and person re-identification \cite{xx,xx,xx}.  Further, since RF signals can traverse occlusions and are insensitive to visible light,  these three tasks can be performed through walls and in dark settings. However, past works on these tasks are based on supervised learning using labeled RF datasets. We would like to demonstrate the possibility of improving accuracy on these tasks by learning useful representations from unlabeled RF signals.


%In this section, we adapt IPCL to learn useful representations from unlabeled RF signals.  We would like the learned representation to be useful for the following three downstream tasks:
%\begin{Itemize}
%\item (a) RF-Based 3D Pose Estimation~\cite{xxx}, which uses radio signals to infer the 3D locations of 12 keypoints on the human body that denote the head, shoulders, arms, wrists, hip, knees, and feet.
%\item (b) RF-Based action recognition~\cite{xxx}, which analyses radio signals to infer human actions and interactions in the presence of occlusions and in poor lighting conditions. 
%\item (b) RF-Based ReId~\cite{xxx}, which recognizes a person-of-interest across different places and times by analyzing the radio signals that bounce off their bodies. 
%\end{Itemize}

Before delving to the detail of our unsupervised representation learning, we first explain the typical neural models used in these tasks. For all of these tasks, the input to the neural network is a time sequence of RF frames. Where each RF frame is a pair of  2D heatmaps: horizontal heatmaps and vertical heatmaps as illustrated in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio signals on a plane parallel to the ground, while the vertical heatmap is a projection of the radio signals on a plane perpendicular to the ground. There are typically 30 pairs of heatmaps per second, i.e., 30 RF frames per second. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-heatmaps}
\end{center}
\vspace{-10pt}
\caption{Illustration of RF signals expressed as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}\label{fig:rf-heatmaps}
\vspace{-15pt}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{Typical RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and then use ROI Align with the given bounding box to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. It has two branches: Predictive Branch and Contrastive Branch. For the predictive branch, we randomly mask some frames across time for prediction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and use the given ROI align to crop out regions containing humans. The predictive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear head to generate normalized features. The combined loss of predictive learning and contrastive learning is used to train the model.}\label{fig:model-rf}
\end{figure*}


The neural network models used in the above three tasks have the general framework in Figure~\ref{fig:rf-framework}. The model first uses a spatio-temporal convolutional feature network to extract features from the input RF frames. It then crops out a bounding box around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features for downstream tasks, such as pose estimation, action recognition or person re-identification. The feature network structure is typically the same for all tasks, while different tasks can have different sub-network structure specifically designed for each task. The goal of RF-based unsupervised representation learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.


\subsection{Adapting \name\ to RF Representation}
As shown in Figure \ref{fig:model-rf}, for contrastive training on RF signals, the anchor and positive sample share the same input RF frames with different random jitter of its bounding boxes. Negative samples of an anchor sample are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment, so that the environment. For the inpainting task, we consider a sequence of RF frames and randomly mask out some segments with random length and fill them with zero.

During the unsupervised learning phase, we employ a standard spatio-temporal RF feature extraction network to encode the input RF frames. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from the WiTrack localization algorithm \cite{xxx}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layers is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the inpainting task, a decoder is added to reconstruct the original RF heatmaps, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed RF frames and the ground truth RF frames. For \name, we combine these two losses together as $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$ in our RF-based experiments.



\subsection{Experimental Setup}
We pre-train \name on two RF datasets: RF-MMD \cite{xxx} and RRD \cite{xxx}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF clips from 100 different identities at 5 different locations on a university campus, and 6305 RF clips from 38 different identities in 19 different homes.

After pre-training using IPCL, to evaluate the quality of the learned representation, we apply the learned RF feature extraction network in three different downstream RF-based tasks: 3D pose estimation, action recognition, and person re-identification. In this downstream training phase, we use the pre-trained RF feature extraction network as initialization of RF feature extractor for each downstream task and fine-tune the model for each task on downstream datasets. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. We also train a supervised baseline from scratch on the same data for each task to compare with the results of unsupervised learning. 

\subsection{Downstream Evaluation Results}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & Skeleton Err. (mm) \\
\hline
Train from Scratch & 3.84 \\
Contrastive+finetune & 3.88 \\
Predictive+finetune & 3.62 \\
\name+finetune & \textbf{3.51} \\
\hline
\end{tabular}
\caption{3D pose estimation error of different models on RF-MMD.}
\label{tab:result-pose}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
& $\theta=0.1$ & $\theta=0.5$ \\
\hline
Train from Scratch & 90.1  & 87.8 \\
Contrastive+finetune & 89.8 & 87.4 \\
Predictive+finetune & 91.7 & 88.7 \\
\name+finetune & \textbf{92.5} & \textbf{89.6} \\
\hline
\end{tabular}
\caption{Action recognition mAP of different models at different thresholds on RF-MMD.}
\label{tab:result-action}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 59.5 & 82.1 & 95.5 \\
Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
Predictive+finetune & 60.1 & 83.3 & 95.5  \\
\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Campus.}
\label{tab:result-reid-campus}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 46.4 & 74.6 & 89.5 \\
Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
Predictive+finetune & 47.5 & 75.3 & 90.3 \\
\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Home.}
\label{tab:result-reid-home}
\end{table}

We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-pose}, \ref{tab:result-action}, \ref{tab:result-reid-campus}, \ref{tab:result-reid-home}. As shown in the results, pre-training the feature network using \name~and fine-tuning it on the downstream tasks  generates the best results in all tasks. Feature network pre-trained by contrastive learning alone generates worse results than random initialization. This is likely due to that contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related semantics. Using the predictive inpainting task clone without the contrastive loss  can generate better results than training from scratch, but the performance is worse than that of \name. This is likely because inptaining alone tend to learn low-level features too close to the pixels in the RF heatmaps. In contrast,  \name\  is able to utilize the combination of contrastive learning and inpainting loss to learn abstract and information-preserving features that are useful for downstream tasks.  This demonstrates that the RF feature extraction network learned by \name\ can extract representations that contain multiple semantics related to multiple different downstream tasks.


==> source/experiment-rf-5.tex <==
\section{Learning Unsupervised Representations from RF Signals}
Radio Frequency (RF) signals have been used for pose estimation, action recognition, and person re-identification \cite{xx,xx,xx}.  Further, since RF signals can traverse occlusions and are insensitive to visible light,  these three tasks can be performed through walls and in dark settings. However, past works on these tasks are based on supervised learning using labeled RF datasets. We would like to demonstrate the possibility of improving accuracy on these tasks by learning useful representations from unlabeled RF signals.


%In this section, we adapt IPCL to learn useful representations from unlabeled RF signals.  We would like the learned representation to be useful for the following three downstream tasks:
%\begin{Itemize}
%\item (a) RF-Based 3D Pose Estimation~\cite{xxx}, which uses radio signals to infer the 3D locations of 12 keypoints on the human body that denote the head, shoulders, arms, wrists, hip, knees, and feet.
%\item (b) RF-Based action recognition~\cite{xxx}, which analyses radio signals to infer human actions and interactions in the presence of occlusions and in poor lighting conditions. 
%\item (b) RF-Based ReId~\cite{xxx}, which recognizes a person-of-interest across different places and times by analyzing the radio signals that bounce off their bodies. 
%\end{Itemize}

Before delving to the detail of our unsupervised representation learning, we first explain the typical neural models used in these tasks. For all of these tasks, the input to the neural network is a time sequence of RF frames. Where each RF frame is a pair of  2D heatmaps: horizontal heatmaps and vertical heatmaps as illustrated in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio signals on a plane parallel to the ground, while the vertical heatmap is a projection of the radio signals on a plane perpendicular to the ground. There are typically 30 pairs of heatmaps per second, i.e., 30 RF frames per second. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-heatmaps}
\end{center}
\vspace{-10pt}
\caption{Illustration of RF signals expressed as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}\label{fig:rf-heatmaps}
\vspace{-15pt}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{Typical RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and then use ROI Align with the given bounding box to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. It has two branches: Predictive Branch and Contrastive Branch. For the predictive branch, we randomly mask some frames across time for prediction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and use the given ROI align to crop out regions containing humans. The predictive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear head to generate normalized features. The combined loss of predictive learning and contrastive learning is used to train the model.}\label{fig:model-rf}
\end{figure*}


The neural network models used in the above three tasks have the general framework in Figure~\ref{fig:rf-framework}. The model first uses a spatio-temporal convolutional feature network to extract features from the input RF frames. It then crops out a bounding box around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features for downstream tasks, such as pose estimation, action recognition or person re-identification. The feature network structure is typically the same for all tasks, while different tasks can have different sub-network structure specifically designed for each task. The goal of RF-based unsupervised representation learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.


\subsection{Adapting \name\ to RF Representation}
\noindent\textbf{Reconstruction Branch Setting.}
Each input RF clip contains 100 frames. We randomly mask out 25 frames within this clip and fill them with zero for later reconstruction.
 
\noindent\textbf{Contrastive Branch Settings.}
As shown in Figure \ref{model-rf}, for contrastive training on RF signals, the anchor and positive sample shares the same input RF frames with different random jitter of its bounding boxes. Each coordinate is added with a random jitter value $x_\delta \in [-10px, 10px]$.
Negative samples of an anchor sample are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment, so that the environment will not be a shortcut to easily distinguish positive and negative samples.

\noindent\textbf{Training Pipeline.}
During the unsupervised learning phase, we employ a standard spatio-temporal RF feature extraction network to encode the input RF frames. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from the WiTrack localization algorithm \cite{xxx}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layers is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the inpainting task, a decoder is added to reconstruct the original RF heatmaps, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed RF frames and the ground truth RF frames. For \name, we combine these two losses together as $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$ in our RF-based experiments.



\subsection{Experimental Setup}
\noindent\textbf{Datasets} We pre-train \name on two RF datasets: RF-MMD \cite{xxx} and RRD \cite{xxx}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF clips from 100 different identities at 5 different locations on a university campus, and 6305 RF clips from 38 different identities in 19 different homes.


\noindent\textbf{Evaluation Metric.} After pre-training using IPCL, to evaluate the quality of the learned representation, we apply the learned RF feature extraction network in three different downstream RF-based tasks: 3D pose estimation, action recognition, and person re-identification. On 3D pose estimation, we use the average $l_2$ distance between 14 keypoints from predicted and ground-truth skeleton as evaluation metric. On action recognition task, we use mean average precision (mAP) at different intersection-over-union (IoU) thresholds $\theta$ to evaluate the accuracy of the model on detecting and classifying an action event. On person re-identification task, we first separate the dataset into query set and gallery set randomly. The query samples and gallery samples are then encoded to feature vectors using our model. Then we calculate the cosine distance between each query sample’s features and each gallery sample’s features and rank the distance to retrieve the top-N closest gallery samples for each query sample. We compute the standard evaluation metrics for person ReID based on the ranking results: mean average precision score (mAP) and the cumulative matching curve (CMC) at rank-1 and rank-5.

\noindent\textbf{Finetuning Setting.} In the downstream training phase, we use the pre-trained RF feature extraction network as initialization of RF feature extractor for each downstream task and fine-tune the model for each task on downstream datasets. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. We also train a supervised baseline from scratch on the same data for each task to compare with the results of unsupervised learning. 



\subsection{Downstream Evaluation Results}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & Skeleton Err. (cm) \\
\hline
Train from Scratch & 3.84 \\
Contrastive+finetune & 3.88 \\
Predictive+finetune & 3.62 \\
\name+finetune & \textbf{3.51} \\
\hline
\end{tabular}
\caption{3D pose estimation error of different models on RF-MMD.}
\label{tab:result-pose}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
& $\theta=0.1$ & $\theta=0.5$ \\
\hline
Train from Scratch & 90.1  & 87.8 \\
Contrastive+finetune & 89.8 & 87.4 \\
Predictive+finetune & 91.7 & 88.7 \\
\name+finetune & \textbf{92.5} & \textbf{89.6} \\
\hline
\end{tabular}
\caption{Action recognition mAP of different models at different thresholds on RF-MMD.}
\label{tab:result-action}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 59.5 & 82.1 & 95.5 \\
Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
Predictive+finetune & 60.1 & 83.3 & 95.5  \\
\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Campus.}
\label{tab:result-reid-campus}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 46.4 & 74.6 & 89.5 \\
Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
Predictive+finetune & 47.5 & 75.3 & 90.3 \\
\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Home.}
\label{tab:result-reid-home}
\end{table}

We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-pose}, \ref{tab:result-action}, \ref{tab:result-reid-campus}, \ref{tab:result-reid-home}. As shown in the results, pre-training the feature network using \name~and fine-tuning it on the downstream tasks  generates the best results in all tasks. Overall, over its supervised counterparts, \name has 8.6\% relative improvement on pose estimation error, 2.5\% relative improvement on action recognition mAP, and 2.92\% improvement on person ReID mAP.

Feature network pre-trained by contrastive learning alone generates worse results than random initialization. This is likely due to that contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related downstream tasks. Using the predictive inpainting task clone without the contrastive loss  can generate better results than training from scratch, but the performance is worse than that of \name. This is likely because inptaining alone tend to learn low-level features too close to the pixels in the RF heatmaps, and more information about the human dynamics is not extracted. In contrast,  \name\  is able to utilize the combination of contrastive learning and inpainting loss to learn abstract and information-preserving features that are useful for downstream tasks.  This demonstrates that the RF feature extraction network learned by \name\ can extract representations that contain multiple types semantics related to various downstream tasks.


==> source/experiment-rf-6.tex <==
\section{Learning Unsupervised Representations from RF Signals}
\label{sec:rf-exp}
Radio Frequency (RF) signals have been studied a lot recently for pose estimation, action recognition, and person re-identification \cite{zhao2018through,zhao2018rf,li2019making,chetty2017low,zhang2018latern,fan2020home,zhao2019through,adib2015capturing,vasisht2018duet,tian2018rf,zhao2016emotion,zhao2017learning,hsu2019enabling,fan2020learning}, mainly due to its good properties that it can traverse occlusions and are insensitive to visible light. Therefore, these tasks can be performed through walls and in dark settings where RGB-based cameras fail. However, past works on these tasks are based on supervised learning using labeled RF datasets. 
Since RF signals are not interpretable by a human, the annotation is collected by deploying a camera system and synchronizing it with the RF device, which is labor-intensive and hard to scale.  If we can learn useful representation from unlabeled RF signals,  we can reduce overhead and improve the accuracy of the downstream tasks. 


% Radio Frequency (RF) signals have been used for pose estimation, action recognition, and person re-identification \cite{xx,xx,xx}.   Further, since RF signals can traverse occlusions and are insensitive to visible light,  these three tasks can be performed through walls and in dark settings. However, past works on these tasks are based on supervised learning using labeled RF datasets. We would like to demonstrate the possibility of improving accuracy on these tasks by learning useful representations from unlabeled RF signals.


%In this section, we adapt IPCL to learn useful representations from unlabeled RF signals.  We would like the learned representation to be useful for the following three downstream tasks:
%\begin{Itemize}
%\item (a) RF-Based 3D Pose Estimation~\cite{xxx}, which uses radio signals to infer the 3D locations of 12 keypoints on the human body that denote the head, shoulders, arms, wrists, hip, knees, and feet.
%\item (b) RF-Based action recognition~\cite{xxx}, which analyses radio signals to infer human actions and interactions in the presence of occlusions and in poor lighting conditions. 
%\item (b) RF-Based ReId~\cite{xxx}, which recognizes a person-of-interest across different places and times by analyzing the radio signals that bounce off their bodies. 
%\end{Itemize}

Before delving into the details of our unsupervised representation learning, we first explain the typical neural models used in these tasks. For all of these tasks, the input is a time sequence of RF frames. Each RF frame is a pair of  2D heatmaps: one horizontal heatmap and one vertical heatmap, as illustrated in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio signals on a plane parallel to the ground, and the vertical heatmap is a projection of the radio signals on a plane perpendicular to the ground. There are typically 30 pairs of heatmaps per second.
% i.e., 30 RF frames per second.

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-heatmaps}
\end{center}
\vspace{-5pt}
\caption{Illustration of RF signals as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}\label{fig:rf-heatmaps}
\vspace{-5pt}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and ROI Align with the given bounding box is used to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. It has two branches: Reconstructive Branch and Contrastive Branch. For the reconstructive branch, we randomly mask some frames across time for reconstruction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and then use ROI Align with the given bounding box to crop out regions containing humans. The reconstructive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear projection head to generate normalized features. The combination of reconstruction loss and contrastive loss is used to train the model.}\label{fig:model-rf}
\end{figure*}


The neural models used in all the three tasks (i.e., pose estimation, action recognition, and person re-identification) have the general structure in Figure~\ref{fig:rf-framework}. The model first uses a spatio-temporal convolutional feature network to extract features from the input RF frames. It then crops out a bounding box around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features for downstream tasks. The general structure is the same for all tasks, but different tasks can have different sub-networks specifically designed for that task. The goal of RF-based unsupervised representation learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.


\subsection{Adapting \name\ to RF Representations}
\noindent\textbf{Reconstructive Setting.}
Each sample is a sequence of 100 RF frames. We randomly mask out 25 frames within this sequence and fill them with zero for later reconstruction.
 
\noindent\textbf{Contrastive Settings.}
As shown in Figure \ref{fig:model-rf},  the anchor and positive sample share the same input RF frames with different random jitter of the bounding boxes. The jitter value is randomly chosen in  $[-30cm, 30cm]$. Negative samples of an anchor are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment.

\noindent\textbf{Training Pipeline.}
During the unsupervised learning phase, we employ a spatio-temporal RF feature extraction network to encode the input RF frames. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from the WiTrack localization algorithm \cite{adib20143d}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layers is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the reconstruction task, a decoder is added to reconstruct the masked RF frames, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed RF  and the ground truth RF frames. For \name, we combine these two losses together as $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$.



\subsection{Experimental Setup}
\noindent\textbf{Datasets.} We pre-train \name~on two RF datasets: RF-MMD \cite{li2019making} and RRD \cite{fan2020learning}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF sequences from 100 different identities at 5 different locations on a university campus, and 6305 RF sequences from 38 different identities in 19 homes.


\noindent\textbf{Evaluation Metric.} After pre-training using IPCL, we evaluate the quality of the learned representation by applying the learned RF feature extraction network to three downstream RF-based tasks: 3D pose estimation, action recognition, and person re-identification. For 3D pose estimation, we use the average $l_2$ distance between 14 predicted keypoints and their ground-truth values, as evaluation metric. For action recognition, we use mean average precision (mAP) at different intersection-over-union (IoU) thresholds $\theta$ to evaluate the accuracy of the model in detecting and classifying an action event. For person re-identification, we first separate the dataset into query set and gallery set randomly. The query samples and gallery samples are then encoded to feature vectors using our model. Then we calculate the cosine distance between each query sample's features and each gallery sample's features and rank the distance to retrieve the top-N closest gallery samples for each query sample. We compute the standard evaluation metrics for person ReID based on the ranking results: mean average precision score (mAP) and the cumulative matching curve (CMC) at rank-1 and rank-5.

\noindent\textbf{Fine-tuning.} In the downstream training phase, we use the pre-trained RF feature extraction network as initialization of the RF feature extraction network for each downstream task, and fine-tune the model for each task on downstream datasets. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. We also train a supervised baseline from scratch on the same data for each task to compare with the results of unsupervised learning. 



\subsection{Downstream Evaluation Results}
We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-pose}, \ref{tab:result-action}, \ref{tab:result-reid-campus}, \ref{tab:result-reid-home}. As shown in the results, pre-training the feature network using \name~and fine-tuning it on the downstream tasks  generates the best results in all tasks. Overall, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus and 3.6\% relative improvement on RRD-Home.

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & Skeleton Err. (cm) \\
\hline
Train from Scratch & 3.84 \\
z+finetune & 3.88 \\
Reconstructive+finetune & 3.62 \\
\name+finetune & \textbf{3.51} \\
\hline
\end{tabular}
\caption{3D pose estimation performance of different models on RF-MMD in skeleton error (the lower the better).}
\label{tab:result-pose}
\vspace{-5pt}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
& $\theta=0.1$ & $\theta=0.5$ \\
\hline
Train from Scratch & 90.1  & 87.8 \\
Contrastive+finetune & 89.8 & 87.4 \\
Reconstructive+finetune & 91.7 & 88.7 \\
\name+finetune & \textbf{92.5} & \textbf{89.6} \\
\hline
\end{tabular}
\caption{Action recognition performance of different models on RF-MMD in mAP at different IoU thresholds (the higher the better).}
\label{tab:result-action}
\vspace{-5pt}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 59.5 & 82.1 & 95.5 \\
Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
Reconstructive+finetune & 60.1 & 83.3 & 95.5  \\
\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Campus in mAP and CMC (the higher the better).}
\label{tab:result-reid-campus}
\vspace{-5pt}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 46.4 & 74.6 & 89.5 \\
Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
Reconstructive+finetune & 47.5 & 75.3 & 90.3 \\
\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Home in mAP and CMC (the higher the better).}
\label{tab:result-reid-home}
\vspace{-5pt}
\end{table}

The tables also show that the feature network pre-trained using contrastive learning alone generates worse results than random initialization. This is likely due to that contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related downstream tasks. Using the reconstruction task alone without the contrastive loss  can generate better results than training from scratch, but the performance is worse than that of \name. This is likely because inptaining alone tend to learn low-level features too close to the pixels in the RF heatmaps, and fail to learn abstract features about the human body. In contrast,  \name\  is able to utilize the combination of contrastive learning and inpainting loss to learn abstract and information-preserving features that are useful for downstream tasks.  This demonstrates that the RF feature extraction network learned by \name\ can extract representations that contain multiple types of semantics related to various downstream tasks.



==> source/experiment-rf-7.tex <==
\section{Learning Unsupervised Representations from RF Signals}
\label{sec:rf-exp}
Radio Frequency (RF) signals have been studied a lot recently for pose estimation, action recognition, and person re-identification \cite{zhao2018through,zhao2018rf,li2019making,chetty2017low,zhang2018latern,fan2020home,zhao2019through,adib2015capturing,vasisht2018duet,tian2018rf,zhao2016emotion,zhao2017learning,hsu2019enabling,fan2020learning}, mainly due to its good properties that it can traverse occlusions and are insensitive to visible light. Therefore, these tasks can be performed through walls and in dark settings where RGB-based cameras fail. However, past works on these tasks are based on supervised learning using labeled RF datasets. 
Since RF signals are not interpretable by a human, the annotation is collected by deploying a camera system and synchronizing it with the RF device, which is labor-intensive and hard to scale.  If we can learn useful representation from unlabeled RF signals,  we can reduce overhead and improve the accuracy of the downstream tasks. 


% Radio Frequency (RF) signals have been used for pose estimation, action recognition, and person re-identification \cite{xx,xx,xx}.   Further, since RF signals can traverse occlusions and are insensitive to visible light,  these three tasks can be performed through walls and in dark settings. However, past works on these tasks are based on supervised learning using labeled RF datasets. We would like to demonstrate the possibility of improving accuracy on these tasks by learning useful representations from unlabeled RF signals.


%In this section, we adapt IPCL to learn useful representations from unlabeled RF signals.  We would like the learned representation to be useful for the following three downstream tasks:
%\begin{Itemize}
%\item (a) RF-Based 3D Pose Estimation~\cite{xxx}, which uses radio signals to infer the 3D locations of 12 keypoints on the human body that denote the head, shoulders, arms, wrists, hip, knees, and feet.
%\item (b) RF-Based action recognition~\cite{xxx}, which analyses radio signals to infer human actions and interactions in the presence of occlusions and in poor lighting conditions. 
%\item (b) RF-Based ReId~\cite{xxx}, which recognizes a person-of-interest across different places and times by analyzing the radio signals that bounce off their bodies. 
%\end{Itemize}

Before delving into the details of our unsupervised representation learning, we first explain the typical neural models used in these tasks. For all of these tasks, the input is a time sequence of RF frames. Each RF frame is a pair of  2D heatmaps: one horizontal heatmap and one vertical heatmap, as illustrated in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio signals on a plane parallel to the ground, and the vertical heatmap is a projection of the radio signals on a plane perpendicular to the ground. There are typically 30 pairs of heatmaps per second.
% i.e., 30 RF frames per second.

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-heatmaps}
\end{center}
\vspace{-5pt}
\caption{Illustration of RF signals as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}\label{fig:rf-heatmaps}
\vspace{-5pt}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and ROI Align with the given bounding box is used to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. It has two branches: Reconstructive Branch and Contrastive Branch. For the reconstructive branch, we randomly mask some frames across time for reconstruction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and then use ROI Align with the given bounding box to crop out regions containing humans. The reconstructive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear projection head to generate normalized features. The combination of reconstruction loss and contrastive loss is used to train the model.}\label{fig:model-rf}
\end{figure*}


The models used in all the three tasks (i.e., pose estimation, action recognition, and person re-identification) have the general structure in Figure~\ref{fig:rf-framework}. The model first uses a spatio-temporal convolutional feature network to extract features from the input RF frames. It then crops out a bounding box around the person in the feature map. Finally, the cropped features are fed into a task-specific sub-network to generate frame-level features for downstream tasks. The high-level structure is the same for all tasks, but different tasks have different sub-networks specifically designed for that task. The goal of RF-based unsupervised representation learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.


\subsection{Adapting \name\ to RF Representations}
\noindent\textbf{Reconstructive Setting.}
Each sample is a sequence of 100 RF frames. We randomly mask out 25 frames within this sequence and fill them with zero for later reconstruction.
 
\noindent\textbf{Contrastive Settings.}
As shown in Figure \ref{fig:model-rf},  the anchor and positive sample share the same input RF frames with different random jitter of the bounding boxes. The jitter value is randomly chosen in  $[-30cm, 30cm]$. Frames that are within 0.3 seconds of the anchor frame also serves as positive samples. Negative samples of an anchor are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment.

\noindent\textbf{Training Pipeline.}
During the unsupervised learning phase, we employ a spatio-temporal RF feature extraction network to encode the input RF frames. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from the WiTrack localization algorithm \cite{adib20143d}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layers is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the reconstruction task, a decoder is added to reconstruct the masked RF frames, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed RF  and the ground truth RF frames. For \name, we combine these two losses together as $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$.



\subsection{Experimental Setup}
\noindent\textbf{Datasets.} We pre-train \name~on two RF datasets: RF-MMD \cite{li2019making} and RRD \cite{fan2020learning}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF sequences from 100 different identities at 5 different locations on a university campus, and 6305 RF sequences from 38 different identities in 19 homes.


\noindent\textbf{Evaluation Metric.} After pre-training using IPCL, we evaluate the quality of the learned representation by applying the learned RF feature extraction network to three downstream RF-based tasks: 3D pose estimation, action recognition, and person re-identification. For 3D pose estimation, we use the average $l_2$ distance between 14 predicted keypoints and their ground-truth locations, as evaluation metric. For action recognition, we use mean average precision (mAP) at different intersection-over-union (IoU) thresholds $\theta$ to evaluate the accuracy of the model in detecting and classifying an action event. For person re-identification, we first separate the dataset into query set and gallery set randomly. The query samples and gallery samples are then encoded to feature vectors using our model. Then we calculate the cosine distance between each query sample's features and each gallery sample's features and rank the distance to retrieve the top-N closest gallery samples for each query sample. We compute the standard evaluation metrics for person ReID based on the ranking results: mean average precision score (mAP) and the cumulative matching curve (CMC) at rank-1 and rank-5.

\noindent\textbf{Evaluation Settings.} 
%In the downstream training phase, 
We evaluate the performance of the pre-trained RF feature extraction network under both full network fine-tuning setting and fixing feature net setting. In the full fine-tuning setting, we use the pre-trained RF feature extraction network as initialization of the RF feature extraction network for each downstream task, and fine-tune the whole model for each task on downstream datasets. In the fixing feature net setting, we also use the pre-trained RF feature extraction network as initialization of the RF feature extraction network for each downstream task, but this network is frozen during downstream task training, i.e., only those task-specific sub-networks (\ref{fig:rf-framework}) are trained. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. 


\noindent\textbf{Baselines.} Since there is no prior work that applies existing contrastive learning methods on RF data, we implement SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, CPC \cite{henaff2019data} and Inpainting \cite{pathak2016context} on RF data by ourselves as baselines. The SimCLR implementation is similar to the contrastive branch of IPCL, and the inpainting implementation is similar to the reconstructive branch of IPCL. For MoCo, we use the same data augmentation operations as SimCLR, except the positive feature pairs are generated by two feature networks, a normal one and a momentum one. The loss is the same as the one used in \cite{he2020momentum}. For CPC, we follow the design in \cite{henaff2019data}. Specifically, we add a GRU RNN after the RF feature extraction network. The output of the GRU at every frame is then used as the context to predict the features in 1.5s in the future using the contrastive loss. We also train a supervised baseline from scratch for the fine-tuning setting, and a randomly initialized RF feature extraction network serves as a baseline for the fixing feature network setting. 

\subsection{Downstream Evaluation Results}
We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-finetune} and \ref{tab:result-fixed}. As shown in the results, pre-training the feature network using \name~ generates the best results in all tasks under both settings. Under the fixing feature network setting, \name~ is the only method that can achieve results comparable to supervised training. Under the fine-tuning setting, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus and 3.6\% relative improvement on RRD-Home.


\begin{table*}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c |c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
  & 3D Pose Estimation & \multicolumn{2}{c}{Action Recognition} & \multicolumn{3}{c}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
  \hline
 \multirow{ 2}{*}{Methods} &  \multirow{ 2}{*}{Skeleton Err.$^\downarrow$ (mm)} & \multicolumn{2}{c}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ \\
\hline
Random init & 60.1 & 70.5  & 53.3 & 28.1 & 43.8 & 68.8 & 30.1 & 54.2 & 74.6 \\
SimCLR & 80.5 & 8.2 & 0 & 29.8 & 44.1 & 67.5 & 31.2 & 55.1 & 73.8 \\
MoCo & 77.2 & 11.1 & 0.18 & 29.1 & 44.7 & 65.3 & 30.5 & 54.5 & 74.0 \\
CPC & 78.7 & 7.6 & 0 & 30.0 & 42.7 & 69.5 & 30.7 & 54.0 & 75.3 \\
Inpainting & 51.1 & 72.3 & 65.5 & 49.8 & 73.1 & 90.5 & 38.5 & 64.2 & 84.7 \\
\name & \textbf{46.6} & \textbf{86.5} & \textbf{83.1} & \textbf{54.5} & \textbf{78.7} & \textbf{93.0} & \textbf{43.3} & \textbf{72.4} & \textbf{87.6}\\
\hline
Supervised & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
\hline
\end{tabular}
\caption{Evaluation of different models on different RF datasets and tasks under fixing RF feature encoder setting, where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and the weights are frozen during downstream training. $\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}
\label{tab:result-fixed}
\vspace{-5pt}
\end{table*}


\begin{table*}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c |c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
  & 3D Pose Estimation & \multicolumn{2}{c}{Action Recognition} & \multicolumn{3}{c}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
  \hline
 \multirow{ 2}{*}{Methods} &  \multirow{ 2}{*}{Skeleton Err.$^\downarrow$ (mm)} & \multicolumn{2}{c}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ \\
\hline
Random init & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
SimCLR & 38.8 & 89.8 & 87.4 & 59.0 & 81.7 & 94.1 & 45.9 & 73.8 & 88.5 \\
MoCo & 38.3 & 89.7 & 87.2 & 59.3 & 82.0 & 94.5 & 46.4 & 74.3 & 89.7 \\
CPC & 38.6 & 89.9 & 87.5 & 59.4 & 81.5 & 94.0 & 46.0 & 74.5 & 89.1 \\
Inpainting & 36.2 &  91.7 & 88.7 & 60.1 & 83.3 & 95.5 & 47.5 & 75.3 & 90.3\\
\name & \textbf{35.1} & \textbf{92.5} & \textbf{89.6} & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} & \textbf{48.1} & \textbf{76.1} & \textbf{91.0}\\
\hline
\end{tabular}
\caption{Evaluation of different models on different RF datasets and tasks under fine-tuning setting, where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and then fine-tuned during downstream training. $\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}
\label{tab:result-finetune}
\vspace{-5pt}
\end{table*}



%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
%& $\theta=0.1$ & $\theta=0.5$ \\
%\hline
%Train from Scratch & 90.1  & 87.8 \\
%Contrastive+finetune & 89.8 & 87.4 \\
%Reconstructive+finetune & 91.7 & 88.7 \\
%\name+finetune & \textbf{92.5} & \textbf{89.6} \\
%\hline
%\end{tabular}
%\caption{Action recognition performance of different models on RF-MMD in mAP at different IoU thresholds (the higher the better).}
%\label{tab:result-action}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 59.5 & 82.1 & 95.5 \\
%Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
%Reconstructive+finetune & 60.1 & 83.3 & 95.5  \\
%\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Campus in mAP and CMC (the higher the better).}
%\label{tab:result-reid-campus}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 46.4 & 74.6 & 89.5 \\
%Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
%Reconstructive+finetune & 47.5 & 75.3 & 90.3 \\
%\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Home in mAP and CMC (the higher the better).}
%\label{tab:result-reid-home}
%\vspace{-5pt}
%\end{table}

The tables also show that the feature network pre-trained using contrastive learning alone can generate worse results than random initialization. For example, in Tabel \ref{tab:result-fixed}, training a pose sub-network on top of an RF feature extraction network with random weights can get 60.1 pose error, while training a pose sub-network on top of the feature extraction network pre-trained using SimCLR, MoCo and CPC can only get 80.5, 77.2 and 78.7 mm skeleton error, respectively. This is likely due to that contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related downstream tasks. Note that although CPC also uses a predictive task, its prediction is performed on the feature space and thus cannot guarantee the information in the input to be preserved in the learnt representation. Using the reconstruction task alone without the contrastive loss can generate better results than training from scratch, but the performance is worse than that of \name. This is likely because inptaining alone tend to learn low-level features too close to the pixels in the RF heatmaps, and fail to learn abstract features about the human body. In contrast,  \name\  is able to utilize the combination of contrastive learning and inpainting loss to learn abstract and information-preserving features that are useful for downstream tasks.  This demonstrates that the RF feature extraction network learned by \name\ can extract representations that contain multiple types of semantics related to various downstream tasks.



==> source/experiment-rf-8.tex <==
\subsection{Experiments on Real-World RF Datasets}
\label{sec:rf-exp}
In this section, we evaluate IPCL on three real-world RF-based through-wall sensing tasks: 3D pose estimation, human action recognition, and person re-identification, to further demonstrate the effectiveness of \name~on avoiding shortcuts and learning high-quality representations.

\subsubsection{Experiment Setup}

\noindent\textbf{Datasets.} We pre-train \name~on two RF datasets: RF-MMD \cite{li2019making} and RRD \cite{fan2020learning}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF sequences from 100 different identities at 5 different locations on a university campus, and 6305 RF sequences from 38 different identities in 19 homes.


\noindent\textbf{Evaluation Metric.} After pre-training using IPCL, we evaluate the quality of the learned representation by applying the learned RF feature extraction network to three downstream RF-based tasks: 3D pose estimation, action recognition, and person re-identification. For 3D pose estimation, we use the average $l_2$ distance between 14 predicted keypoints and their ground-truth locations, as evaluation metric. For action recognition, we use mean average precision (mAP) at different intersection-over-union (IoU) thresholds $\theta$ to evaluate the accuracy of the model in detecting and classifying an action event. For person re-identification, we first separate the dataset into query set and gallery set randomly. The query samples and gallery samples are then encoded to feature vectors using our model. Then we calculate the cosine distance between each query sample's features and each gallery sample's features and rank the distance to retrieve the top-N closest gallery samples for each query sample. We compute the standard evaluation metrics for person ReID based on the ranking results: mean average precision score (mAP) and the cumulative matching curve (CMC) at rank-1 and rank-5.

\noindent\textbf{Evaluation Settings.} 
%In the downstream training phase, 
We evaluate the performance of the pre-trained RF feature extraction network under both full network fine-tuning setting and fixing feature net setting. In the full fine-tuning setting, we use the pre-trained RF feature extraction network as initialization of the RF feature extraction network for each downstream task, and fine-tune the whole model for each task on downstream datasets. In the fixing feature net setting, we also use the pre-trained RF feature extraction network as initialization of the RF feature extraction network for each downstream task, but this network is frozen during downstream task training, i.e., only those task-specific sub-networks (\ref{fig:rf-framework}) are trained. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. 


\noindent\textbf{Baselines.} Since there is no prior work that applies existing contrastive learning methods on RF data, we implement SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, CPC \cite{henaff2019data} and Inpainting \cite{pathak2016context} on RF data by ourselves as baselines. The SimCLR implementation is similar to the contrastive branch of IPCL, and the inpainting implementation is similar to the reconstructive branch of IPCL. For MoCo, we use the same data augmentation operations as SimCLR, except the positive feature pairs are generated by two feature networks, a normal one and a momentum one. The loss is the same as the one used in \cite{he2020momentum}. For CPC, we follow the design in \cite{henaff2019data}. Specifically, we add a GRU RNN after the RF feature extraction network. The output of the GRU at every frame is then used as the context to predict the features in 1.5s in the future using the contrastive loss. We also train a supervised baseline from scratch for the fine-tuning setting, and a randomly initialized RF feature extraction network serves as a baseline for the fixing feature network setting. 

\subsubsection{Results}
We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-finetune} and \ref{tab:result-fixed}. As shown in the results, pre-training the feature network using \name~ generates the best results in all tasks under both settings. Under the fixing feature network setting, \name~ is the only method that can achieve results comparable to supervised training. Under the fine-tuning setting, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus and 3.6\% relative improvement on RRD-Home.


\begin{table*}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c |c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
  & 3D Pose Estimation & \multicolumn{2}{c}{Action Recognition} & \multicolumn{3}{c}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
  \hline
 \multirow{ 2}{*}{Methods} &  \multirow{ 2}{*}{Skeleton Err.$^\downarrow$ (mm)} & \multicolumn{2}{c}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ \\
\hline
Random init & 60.1 & 70.5  & 53.3 & 28.1 & 43.8 & 68.8 & 30.1 & 54.2 & 74.6 \\
SimCLR & 80.5 & 8.2 & 0 & 29.8 & 44.1 & 67.5 & 31.2 & 55.1 & 73.8 \\
MoCo & 77.2 & 11.1 & 0.18 & 29.1 & 44.7 & 65.3 & 30.5 & 54.5 & 74.0 \\
CPC & 78.7 & 7.6 & 0 & 30.0 & 42.7 & 69.5 & 30.7 & 54.0 & 75.3 \\
Inpainting & 51.1 & 72.3 & 65.5 & 49.8 & 73.1 & 90.5 & 38.5 & 64.2 & 84.7 \\
\name & \textbf{46.6} & \textbf{86.5} & \textbf{83.1} & \textbf{54.5} & \textbf{78.7} & \textbf{93.0} & \textbf{43.3} & \textbf{72.4} & \textbf{87.6}\\
\hline
Supervised & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
\hline
\end{tabular}
\caption{Evaluation of different models on different RF datasets and tasks under fixing RF feature encoder setting, where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and the weights are frozen during downstream training. $\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}
\label{tab:result-fixed}
\vspace{-5pt}
\end{table*}


\begin{table*}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c |c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
  & 3D Pose Estimation & \multicolumn{2}{c}{Action Recognition} & \multicolumn{3}{c}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
  \hline
 \multirow{ 2}{*}{Methods} &  \multirow{ 2}{*}{Skeleton Err.$^\downarrow$ (mm)} & \multicolumn{2}{c}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ \\
\hline
Random init & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
SimCLR & 38.8 & 89.8 & 87.4 & 59.0 & 81.7 & 94.1 & 45.9 & 73.8 & 88.5 \\
MoCo & 38.3 & 89.7 & 87.2 & 59.3 & 82.0 & 94.5 & 46.4 & 74.3 & 89.7 \\
CPC & 38.6 & 89.9 & 87.5 & 59.4 & 81.5 & 94.0 & 46.0 & 74.5 & 89.1 \\
Inpainting & 36.2 &  91.7 & 88.7 & 60.1 & 83.3 & 95.5 & 47.5 & 75.3 & 90.3\\
\name & \textbf{35.1} & \textbf{92.5} & \textbf{89.6} & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} & \textbf{48.1} & \textbf{76.1} & \textbf{91.0}\\
\hline
\end{tabular}
\caption{Evaluation of different models on different RF datasets and tasks under fine-tuning setting, where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and then fine-tuned during downstream training. $\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}
\label{tab:result-finetune}
\vspace{-5pt}
\end{table*}



%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
%& $\theta=0.1$ & $\theta=0.5$ \\
%\hline
%Train from Scratch & 90.1  & 87.8 \\
%Contrastive+finetune & 89.8 & 87.4 \\
%Reconstructive+finetune & 91.7 & 88.7 \\
%\name+finetune & \textbf{92.5} & \textbf{89.6} \\
%\hline
%\end{tabular}
%\caption{Action recognition performance of different models on RF-MMD in mAP at different IoU thresholds (the higher the better).}
%\label{tab:result-action}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 59.5 & 82.1 & 95.5 \\
%Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
%Reconstructive+finetune & 60.1 & 83.3 & 95.5  \\
%\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Campus in mAP and CMC (the higher the better).}
%\label{tab:result-reid-campus}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 46.4 & 74.6 & 89.5 \\
%Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
%Reconstructive+finetune & 47.5 & 75.3 & 90.3 \\
%\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Home in mAP and CMC (the higher the better).}
%\label{tab:result-reid-home}
%\vspace{-5pt}
%\end{table}

The tables also show that the feature network pre-trained using contrastive learning alone can generate worse results than random initialization. For example, in Tabel \ref{tab:result-fixed}, training a pose sub-network on top of an RF feature extraction network with random weights can get 60.1 pose error, while training a pose sub-network on top of the feature extraction network pre-trained using SimCLR, MoCo and CPC can only get 80.5, 77.2 and 78.7 mm skeleton error, respectively. This is likely due to that contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related downstream tasks. Note that although CPC also uses a predictive task, its prediction is performed on the feature space and thus cannot guarantee the information in the input to be preserved in the learnt representation. Using the reconstruction task alone without the contrastive loss can generate better results than training from scratch, but the performance is worse than that of \name. This is likely because inptaining alone tend to learn low-level features too close to the pixels in the RF heatmaps, and fail to learn abstract features about the human body. In contrast,  \name\  is able to utilize the combination of contrastive learning and inpainting loss to learn abstract and information-preserving features that are useful for downstream tasks.  This demonstrates that the RF feature extraction network learned by \name\ can extract representations that contain multiple types of semantics related to various downstream tasks.



==> source/experiment-rf-9.tex <==
\subsection{Experiments with RF Datasets}
\label{sec:rf-exp}




We evaluate \name~on three through-wall RF sensing tasks: pose estimation, action recognition, and re-identification. 

\vspace{-2pt}\noindent\textbf{Datasets.} We pre-train \name~on two real-world RF datasets: RF-MMD \cite{li2019making} and RRD \cite{fan2020learning}. RF-MMD is an RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  863 RF sequences from 100 different identities at 5 different locations on a university campus, and 6305 RF sequences from 38 different identities in 19 homes.

\vspace{-2pt}\noindent\textbf{Evaluation Metrics.}  We use the performance metrics used by past work for each task. Specifically, for 3D pose estimation, we use the average $l_2$ distance between 14 predicted keypoints and their ground-truth locations as the evaluation metric. For action recognition, we use mean average precision (mAP) at different intersection-over-union (IoU) thresholds $\theta$ to evaluate the accuracy of the model in detecting and classifying an action event. For person re-identification, we separate the dataset into query set and gallery set. The query samples and gallery samples are then encoded to feature vectors. We calculate the cosine distance between the features of each query sample and each gallery sample, and rank the distance to get the top-N closest gallery samples for each query sample. Based on the ranking results, we compute the mean average precision (mAP) and the cumulative matching characteristic (CMC) at rank-1 and rank-5.

\vspace{-2pt}\noindent\textbf{Evaluation Settings.} 
We evaluate the performance of \name~and baselines under both fixed feature extractor setting and fine-tuning setting. In the fixed feature extractor setting, we use the pre-trained RF feature extractor as initialization of the RF feature extractor for each downstream task, but this feature network is frozen during downstream task training, i.e., only those task-specific sub-networks (\ref{fig:rf-framework}) are trained. In the fine-tuning setting, we use the self-supervised representation as an initialization, which gets fine-tuned during training on each task --i.e., we use the pre-trained RF feature extractor to initialize the feature extractor for each downstream task, and fine-tune the whole model on the downstream task. We use the RF-MMD dataset for downstream tasks of pose estimation and action recognition, and the RRD dataset for person re-identification. 


\vspace{-2pt}\noindent\textbf{Baselines.} Since there is no prior work that applies existing contrastive learning methods on RF data, we implement SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum}, CPC \cite{henaff2019data} and BYOL \cite{grill2020bootstrap} on RF data by ourselves as baselines. The SimCLR implementation is similar to the contrastive branch of \name. For MoCo, we use the same data augmentation operations as SimCLR, except the positive feature pairs are generated by two feature networks, a normal one and a momentum one. The loss is the same as the one used in \cite{he2020momentum}. For CPC, we follow the design in \cite{henaff2019data}. Specifically, we add a GRU RNN after the RF feature extractor. The output of the GRU at every frame is then used as the context to predict the features in 1.5s in the future using the contrastive loss. We also train a supervised baseline from scratch for the fine-tuning setting, and a randomly initialized RF feature extractor serves as a baseline for the fixed feature extractor setting. 

\vspace{-2pt}
\subsubsection{RF Results}
We evaluate the RF feature extractor learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-fixed} and \ref{tab:result-finetune}. As shown in the results, pre-training the feature network using \name~ performs the best for all tasks in both settings. Under the fixed feature extractor setting, \name~ is the only method that is comparable to supervised training. Under the fine-tuning setting, compared to its supervised counterparts, \name~has 8.6\% relative improvement in 3D pose estimation error, 3.7\% relative improvement in action recognition mAP at $\theta=0.1$, 2.2\% relative improvement in person ReID mAP on RRD-Campus, afnd 3.6\% relative improvement on RRD-Home.




%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
%& $\theta=0.1$ & $\theta=0.5$ \\
%\hline
%Train from Scratch & 90.1  & 87.8 \\
%Contrastive+finetune & 89.8 & 87.4 \\
%Reconstructive+finetune & 91.7 & 88.7 \\
%\name+finetune & \textbf{92.5} & \textbf{89.6} \\
%\hline
%\end{tabular}
%\caption{Action recognition performance of different models on RF-MMD in mAP at different IoU thresholds (the higher the better).}
%\label{tab:result-action}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 59.5 & 82.1 & 95.5 \\
%Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
%Reconstructive+finetune & 60.1 & 83.3 & 95.5  \\
%\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Campus in mAP and CMC (the higher the better).}
%\label{tab:result-reid-campus}
%\vspace{-5pt}
%\end{table}
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
%\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
%\hline
%Train from Scratch & 46.4 & 74.6 & 89.5 \\
%Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
%Reconstructive+finetune & 47.5 & 75.3 & 90.3 \\
%\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
%\hline
%\end{tabular}
%\caption{Person re-identification performance of different models on RRD-Home in mAP and CMC (the higher the better).}
%\label{tab:result-reid-home}
%\vspace{-5pt}
%\end{table}

The tables also show that the feature network pre-trained using contrastive learning alone can generate worse results than random initialization. For example, in Table \ref{tab:result-fixed}, training a pose sub-network on top of an RF feature extractor with random weights can get 60.1 pose error, while training a pose sub-network on top of the feature extractor pre-trained using SimCLR, MoCo and CPC can only get 80.5, 77.2 and 78.7 mm pose error, respectively. This is likely due to that contrastive learning learns shortcut semantics irrelevant to human sensing, and thus is harmful to human-related downstream tasks. Note that although CPC also uses a predictive task, its prediction is performed on the feature space and thus cannot guarantee the information in the input to be preserved in the learned representation. In contrast,  \name\  is able to utilize the combination of contrastive and reconstructive learning to learn abstract and information-preserving features that are useful for downstream tasks.  The above results further show that the feature extractor learned by \name\ can extract representations that contain multiple types of semantics related to various downstream tasks. 

%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{featreid}
%\end{center}
%\caption{Feature visualization of SimCLR and IPCL using tSNE on RF-RRD-Home.}\label{fig:reid-tsne}
%\vskip -0.1in
%\end{figure}

%We also visualize the features learned by SimCLR and \name~ in Figure \ref{fig:image-tsne} using tSNE on RF-RRD-Home dataset, colored by person identities. As shown in the figure, features learned by SimCLR cannot form clusters when colored using person identities, while features learned by \name shows clear clustering. This  shows that contrastive learning will fall into unknown shortcut that can be totally irrelevant to downstream tasks on RF dataset, while \name~can avoid learning only the shortcut and generate high-quality features.
%



==> source/experiment-rf.tex <==
\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. Our \name~ framework has two branches: Predictive Branch and Contrastive Branch. For the predictive branch, we randomly mask some frames across time for prediction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and use the given ROI align to crop out regions containing humans. The predictive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear head to generate normalized features. The combined loss of predictive learning and contrastive learning is used to train the model.}\label{fig:model-toy}
\end{figure*}

\section{RF-based Human Sensing}
In this section, we evaluate \name~on real-world RF datasets to show its effectiveness of learning multiple fine-grained semantics. We first apply \name~on large unlabeled RF datasets to train a feature extractor for RF signals, and then evaluate its performance on multiple downstream RF-based human sensing tasks, including pose estimation, action recognition, and human identification.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{Typical RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and then use ROI Align with the given bounding box to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\subsection{RF-based Human Sensing Framework}
We first introduce the general framework used for various RF-based human sensing tasks, which is illustrated in Figure~\ref{fig:rf-framework}. It first uses a spatio-temporal convolutional feature network to extract features from  input RF frames. It will then crop out the region of interest around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features for downstream tasks, such as pose estimation, action recognition or person re-identification. The feature network structure is typically the same for all tasks, while different tasks can have different sub-network structure specifically designed for each task. The goal of RF-based unsupervised learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.

\subsection{Experiment Setup}
We pre-train \name on two RF datasets: RF-MMD \cite{xxx} and RRD \cite{xxx}. RF-MMD is a RF-based pose estimation and action recognition dataset consisting of 25 hours of RF data with 30 volunteers performing 35 actions in 10 different indoor environments. RRD is an RF-based person re-identification dataset. It contains  
 863 RF clips from 100 different identities at 5 different locations on a university campus, and 6305 RF clips from 38 different identities in 19 different homes.


For contrastive training on RF signals, the anchor and positive sample shares the same input RF frames with different random jitter of its bounding boxes. Negative samples of an anchor sample are all other samples in the batch except for itself and its positive sample. All samples in a batch are randomly sampled from the same environment, so that the environment will not be a shortcut to easily distinguish positive and negative samples. The inpainting task in this case, we consider a sequence of RF frames and randomly mask out some  some segments with random length in it and fill them with zero.

During the unsupervised learning phase, we employ a standard spatio-temporal RF feature extraction network to encode the input RF heatmaps. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from human detection algorithm of WiTrack \cite{xxx}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layer is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the inpainting task, a decoder is added to reconstruct the original RF heatmaps, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed heatmaps and the ground truth heatmaps without temporal mask. For \name, we combine these two losses together to be $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 100$ and $\lambda_2 = 1$ in our RF-based experiments.

After the contrastive pre-training phase, to evaluate the quality of the learned representation, we apply the learned RF feature extraction network in three different downstream RF-based human sensing tasks: 3D pose estimation, action recognition, and person re-identification. In this downstream training phase, we use the pre-trained RF feature extraction network as initialization of RF feature extractor for each downstream task and fine-tune the model for each task on downstream datasets. We use the pre-trained model on RF-MMD for downstream tasks of pose estimation and action recognition, and use the pre-trained model on RRD for person re-identification. We also train a supervised baseline from scratch on the same data for each task to compare with the results of unsupervised learning. 

\subsection{Downstream Evaluation Results}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & Skeleton Err. (mm) \\
\hline
Train from Scratch & 3.84 \\
Contrastive+finetune & 3.88 \\
Predictive+finetune & 3.62 \\
\name+finetune & \textbf{3.51} \\
\hline
\end{tabular}
\caption{3D pose estimation error of different models on RF-MMD.}
\label{tab:result-pose}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 2}{*}{Methods}  &  \multicolumn{2}{c}{mAP} \\
& $\theta=0.1$ & $\theta=0.5$ \\
\hline
Train from Scratch & 90.1  & 87.8 \\
Contrastive+finetune & 89.8 & 87.4 \\
Predictive+finetune & 91.7 & 88.7 \\
\name+finetune & \textbf{92.5} & \textbf{89.6} \\
\hline
\end{tabular}
\caption{Action recognition mAP of different models at different thresholds on RF-MMD.}
\label{tab:result-action}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 59.5 & 82.1 & 95.5 \\
Contrastive+finetune & 59.0 & 81.7 & 94.1 \\
Predictive+finetune & 60.1 & 83.3 & 95.5  \\
\name+finetune & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Campus.}
\label{tab:result-reid-campus}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}  c @{\hspace{0.2cm}} c @{\hspace{0.2cm}} c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
\multirow{ 1}{*}{Methods}  &  mAP & CMC-1 & CMC-5  \\
\hline
Train from Scratch & 46.4 & 74.6 & 89.5 \\
Contrastive+finetune & 45.9 & 73.8 & 88.5 \\
Predictive+finetune & 47.5 & 75.3 & 90.3 \\
\name+finetune & \textbf{48.1} & \textbf{76.1} & \textbf{91.0} \\
\hline
\end{tabular}
\caption{Person re-identification performance of different models on RRD-Home.}
\label{tab:result-reid-home}
\end{table}

We evaluate the RF feature extraction network learned by \name~on multiple downstream RF-based tasks. The results are shown in Table \ref{tab:result-pose}, \ref{tab:result-action}, \ref{tab:result-reid-campus}, \ref{tab:result-reid-home}. As shown in the results, pre-training the feature network using \name~and fine-tuning it on downstream task  generates the best results in all tasks. Feature network pre-trained by contrastive learning alone generates worse results than random initialization. This may be because contrastive learning learns semantics irrelevant to human and thus is harmful to human-related semantics. Predictive learning can generate better results than training from scratch, but since the features learnt by predictive learning alone is too low-level, the performance is worse than that of PCL which is able to utilize contrastive learning to learn fine-grained high-level features. This demonstrate that the RF feature extraction network learnt by \name~can extract representations that contains multiple fine-grained semantics related to different downstream tasks.


==> source/experiment-rgb-3.tex <==
\section{Experiments on RGB Datasets}\label{sec:rf-exp}
We evaluate \name\ on two RGB datasets and compare it to state-of-the-art contrastive learning methods. 

\subsection{Digit \& Background Classification}
To better understand the impact of shortcuts on contrastive learning and \name, we experiment with 
the Colorful-MNIST dataset proposed in~\cite{xxx}. The dataset is constructed by assigning each digit from MNIST a background  image selected randomly from the STL-10 dataset. Hence, each image in the Colorful-MNIST dataset has two types of semantic information that correspond to the digit class and the background class.  




\subsubsection{Experiment Setup}
\noindent\textbf{Reconstructive Branch.}
For each input image, we randomly mask out $3-5$ patches with a random size between $10-16$ at random location from the input images. These masked regions are filled with the average pixel value of the dataset.

\noindent\textbf{Contrastive Branch.}
We follow the setup in \ref{sec:xxx} for contrastive training. Examples of construct positive and negative samples are shown in Figure \ref{fig:toy-dataset}. For contrastive training on digit, we construct positive samples to have the same digit as the anchor on a randomly sampled background. For contrastive training on background, we construct positive samples to have randomly sampled digit on the same background as the anchor. For contrastive training on both digit and background, we construct positive sample to have the same digit as the anchor at a random location on a random patch of the same background as the anchor. We implemented two different contrastive learning baselines: SimCLR which samples negative pairs within batch, and Moco which generate negative using a momentum decoder. For our \name, we sample follow SimCLR and sample negative within batch.

\noindent\textbf{Network Structure}
We use a 6-layer ConvNet as our encoder network $E$. Note that, in \name, the encoder weights for the reconstructive and contrastive branches are shared. The decoder network $D$ is a 6-layer deconvolutional network which is symmetric to $E$. The MLP-Head $H$ for contrastive learning is a 2-layer non-linear head which embed the feature into a 64-dimension normalized space.
For the training of downstream tasks, we freeze the backbone encoder as feature extractor and train a linear classifier for each task to classify the features. 

\noindent\textbf{Evaluation Metric}
After the pre-training phase, to evaluate what semantics are encoded in the latent features, we evaluate the performance on two different downstream classification tasks for an image: Digit classification and Background classification. We report the error rate for each method.

\noindent\textbf{Baselines}
We use state-of-the-art contrastive learning methods, including SimCLR \cite{xxx}, MoCo \cite{xxx} and CPC \cite{xxx} as baselines. We use the same encoder network structure for all methods. The hyper-parameters for each baselines are fine-tuned to achieve its best performance. \red{We include further implementation details of the baselines and \name\ in Appendix A}.

\subsubsection{Results}

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{toy-dataset}
\end{center}
\caption{Illustration of our Colorful-MNIST dataset. During contrastive training on one of the factors, the anchor and the positive sample will be the same for this certain factor, while the other factor will be different (left and right). During contrastive training on both factors, both digit and background of anchor and positive sample are the same (middle).}\label{fig:toy-dataset}
\end{figure}

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.1cm}} c c @{\hspace{0.1cm}}c @{\hspace{0.1cm}}c}\hline
 Method & \begin{tabular}{@{}c@{}}shared factor \& \\ supervised label\end{tabular}  & \begin{tabular}{@{}c@{}}digit cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}bkgd cls. \\ error rate (\%)\end{tabular} \\
\hline
\multirow{ 3}{*}{SimCLR}  & digit  & 12.1  & 86.0  \\
 & bkgd   & 87.8  & 51.9  \\
 & digit \& bkgd & 85.1  & 51.5 \\ 
\hline  
  

\multirow{ 3}{*}{MoCo}  & digit  & 14.4  & 86.5  \\
 & bkgd  & 85.6 & 54.1 \\
 & digit \& bkgd & 84.3 & 53.7 \\ 
\hline     
\multirow{ 1}{*}{CPC}  & - & 84.2  & 64.8 \\
\hline
\multirow{ 1}{*}{Predict}   & - & 15.3  & 65.0 \\
\hline
\multirow{ 1}{*}{\textbf{PreCLR}}  & digit \& bkgd    & 11.7  & 54.0\\
\hline
\hline

\multirow{ 3}{*}{Supervised}  & digit & 3.9  & 88.6  \\
 & bkgd   & 87.1  & 43.3 \\
 & digit \& bkgd & 7.0  & 45.5 \\ 

\hline
\end{tabular}
\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of digit classification and background classification.}}
\label{tab:result-toy}
\end{table}

We first study the representation quality learnt using contrastive learning and show the performance on downstream tasks.
As shown in Table \ref{tab:result-toy}, if the positive samples share only one semantics, the standard contrastive learning approach (SimCLR and Moco) can learn a good representation for the shared semantics while totally failing on the other semantics. This shows that the representation of one of these two semantics cannot help to classify the second semantics. More interestingly, if both semantics are shared between positive samples, only one of them (the background) will be learnt.
On the other hand, predictive unsupervised learning can learn both semantics because the representation should contain enough information to reconstruct the original image. However, the learnt representation's quality is not as good as that learnt using contrastive learning. 

The combination of contrastive and predictive learning (\name) combines the advantages of both world: it can learn representation for both semantics and the representation for each of them is of good quality. This shows that our method's effectiveness on extracting representation that is of high quality on all semantics shared between positive samples. This is quite important in tasks where positive samples share multiple semantics and we only care some certain ones of them, such as RF-based human sensing, since RF signals contain information related to both human and background, and we only care about ones related to human.


\subsection{Face Attribute Classification}

We then evaluate \name~on FairFace\cite{karkkainen2019fairface}, which is a real world human face attribute dataset. One important feature of such dataset is that each face contains multiple types of semantics including gender, age, and ethnicity, each of them requires the network to learn different types features. For example, to better determine the age of the person, the network may need to look at the wrinkles, while this feature can be useless when determine the person's gender where the length and texture of hair serves an important feature. 


\subsubsection{Experiment Setup}
\noindent\textbf{Predictive Setting}
We use similar strategy as \cite{pathak2016context} to mask out input images. $3-5$ rectangles with a random size between $7-12$ at random location are masked out from an input images. We fill the masked rectangles with the mean pixel value.

\noindent\textbf{Contrastive Setting}
We follow similar strategy as \cite{chen2020simple} to sample positive and negative pairs for contrastive learning. We apply random cropping and random color jittering on an image twice to generate positive pairs. The negative pairs are sampled within batch. 

\noindent\textbf{Network Structure}
We use a standard ResNet-18 as our encoder network $E$. The decoder network $D$ is a symmetric deconvolutional network. The MLP-Head $H$ for contrastive learning is a 2-layer non-linear head which embed the feature into a 128-dim normalized space. 

\noindent\textbf{Evaluation Metric}
After the pre-training phase, we evaluate the learnt representation on three downstream tasks: age, gender and ethnicity, to see which semantics the representation captures best. For the training of the downstream tasks, we freeze the encoder and train a linear layer for each task to classify the features. For the supervised baselines, supervised (a), (g) and (e) are trained on single task of age, gender and ethnicity, respectively, while supervised (all) are joint trained on all the three tasks.

\noindent\textbf{Baselines}
We compare our method with SimCLR on FairFace dataset. For SimCLR, we use the same sampling strategy and network structure as our method. We also fine-tune the hyper-parameters of SimCLR to achieve its best performance.


\subsubsection{Results}
\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.1cm}} c@{\hspace{0.1cm}} c @{\hspace{0.1cm}}c @{\hspace{0.1cm}}c}\hline
 Method & \begin{tabular}{@{}c@{}}age cls. \\ error rate (\%)\end{tabular}  & \begin{tabular}{@{}c@{}}gender cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}ethnicity cls. \\ error rate (\%)\end{tabular} \\
\hline
\multirow{ 1}{*}{SimCLR}  & 55.7  & 21.4  & 37.7  \\

\multirow{ 1}{*}{\textbf{PreCLR}}  & 50.0  & 12.8  & 38.8\\

\multirow{ 1}{*}{Supervised (a)}  & 44.5 & 21.3  & 54.9 \\

\multirow{ 1}{*}{Supervised (g)}  & 56.7 & 7.5  & 54.6  \\

\multirow{ 1}{*}{Supervised (e)}  & 57.9 & 23.2  & 28.6  \\

\multirow{ 1}{*}{Supervised (all)}  & 45.2 & 8.1  &  29.2 \\

\hline
\end{tabular}
\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of age, gender and ethnicity classification.}}
\label{tab:result-face}
\end{table}


In Table \ref{tab:result-face} we show the performance of standard contrastive learning (SimCLR) and \name~on FairFace dataset. As shown by the supervised baseline, the three tasks share some common feature since network trained on one of the task can also be used to classify other tasks. However, each task also has its unique features since there are still big performance gaps on each task between network trained on other task and network trained on the exact task. As shown in the table, SimCLR's performance on age and gender are similar to that of supervised learning on ethnicity, while the performance on ethnicity is far beyond the performance of supervised learning on age and gender. This shows that the SimCLR tends to learn task-specific features related to ethnicity and ignore those task-specific features about age and gender. On the other hand, \name~can learn task-specific features about each task. It can achieve much better performance on age and gender classification, while keeps comparable performance as SimCLR on ethnicity classification. This further demonstrates \name's advantage on preserving useful information in the input and avoid learning only one types of `shortcut' semantics.

==> source/experiment-rgb-4.tex <==
\section{Experiments on RGB datasets}
We evaluate \name\ on two RGB datasets, and compare it to state-of-the-art contrastive learning methods. 


\subsection{Digit \& Background Object Classification}
To better understand the impact of shortcuts on contrastive learning and \name, we experiment with 
the Colorful-MNIST dataset proposed in~\cite{tian2020makes}. The dataset is constructed by assigning each digit from MNIST a background object image selected randomly from the STL-10 dataset. Hence, each image in the Colorful-MNIST dataset has two types of semantic information that correspond to the digit class and the background object class.  Figure~\ref{fig:intro} shows an anchor image from this dataset and corresponding positive and negative samples. 
%\red{The positive sample is a cropped version of the anchor with color jittering. The negative samples are all other samples in the same batch. }


\noindent\textbf{Reconstructive Setting.} For each input image with a size of $64$ by $64$ pixels, we randomly mask out $3$ to $5$ rectangle patches at random locations in the image. The size of each square is chosen by setting its side randomly between $10$ and $16$ pixels. These masked patches are filled with the average pixel value of the dataset.
% For each input image, we randomly mask out $3-5$ patches with a random size between $10-16$ at random location from the input images. These masked regions are filled with the average pixel value of the dataset.

\noindent\textbf{Contrastive Setting.}
For the contrastive branch in \name, similar to \cite{chen2020simple}, we apply random cropping and random color jittering on an image twice to generate positive pairs. The negative pairs are sampled within a batch.

\noindent\textbf{Network Structure.}
We use a 6-layer ConvNet for the encoder network $E$. The encoder weights for the predictive and contrastive branches are shared. The decoder network $D$ is a 6-layer deconvolutional network which is symmetric to $E$. The projection head $H$ for contrastive learning is a 2-layer non-linear head which embed the feature into a 64-dim normalized space. 
%For training of downstream tasks, we freeze the backbone encoder as feature extractor and train a linear classifier for each task to classify the features.


\noindent\textbf{Baselines.}
We use state-of-the-art contrastive learning methods as baselines, including SimCLR \cite{chen2020simple}, MoCo \cite{he2020momentum} and CPC \cite{henaff2019data} for unsupervised representation learning from the Colorful-MNIST dataset.  The same network structure is used for all baselines and for \name's contrastive branch.  The hyper-parameters for each baseline are fine-tuned to achieve its best performance. Other implementation details are provided in Appendix.

\noindent\textbf{Evaluation Metric.}
We evaluate the representations learned by \name\ and the baselines by using them to train two linear classifiers for two downstream tasks: digit classification and background object classification.  We report the error rate for each method.  

\subsubsection{Results}
Table \ref{tab:result-toy} reports the performance of the learned representation on two downstream tasks: digit and background object classification. The table compares various contrastive learning methods with \name. It also compares the performance of these unsupervised representation learning methods with supervised methods for learning representation, where the supervision is applied on the digit, background object or both. All methods including the supervised ones use the same encoder network architecture described above. 


\begin{table}[h]
\centering
\begin{tabular}{c |@{\hspace{0.1cm}}c @{\hspace{0.1cm}}c}\hline
 Method  & \begin{tabular}{@{}c@{}}digit cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}bkgd cls. \\ error rate (\%)\end{tabular} \\ 
 \hline
SimCLR   & 85.1  & 51.5 \\
MoCo   & 84.3 & 53.7 \\
CPC  &  84.2  & 64.8 \\\hline
%Recontruction   & 15.3  & 65.0 \\
{\bf \name~(ours) }   & {\bf 11.7}  & {\bf 54.0}\\
\hline
\hline
Supervised on digit  &  3.9  & 88.6  \\
 Supervised on bkgd  & 87.1  & 43.3 \\
 Supervised on digit \& bkgd   & 7.0  & 45.5 \\
\hline
\end{tabular}
\caption{\footnotesize{We study the representation quality learned from Colorful-MNIST using different unsupervised methods. We evaluate the learned representation on the downstream tasks of digit classification and background object classification.}}
\label{tab:result-toy}
\end{table}

Table \ref{tab:result-toy} reveals the following findings:
\begin{Itemize}
\item
 All contrastive learning methods fail to learn features that capture information relevant to digit classification. In fact, their error rate on digit classification (84\% to 85\%) is similar to the error rate  of a supervised method that was trained on background object classification with no information about digits ($\sim$87\%).  In contrast, contrastive learning methods perform reasonably well on background object classification with an error rate about 10\% higher than a supervised method trained on background object classification. This indicates that the background object features played the role of a shortcut for contrastive learning, i.e., those features were sufficient to contrast positive and negative samples, and hence there was no need for contrastive learning to learn digit-related features. 
 \item \name\ on the other hand learned a representation that is useful for both digit and background object classifications. Its error rate on background object classification is as good as the contrastive learning baselines. However, its error rate on digit classification is $\sim$70\% lower than the contrastive baselines.   \name\ was able to learn features related to digit classification because of its reconstructive branch, which forced the representation to keep enough information to reconstruct missing patches in the input. 
\end{Itemize}  
 


%We first study the representation quality learned using contrastive learning and show the performance on downstream tasks.As shown in Table \ref{tab:result-toy}, if we only train the network on one of the factors in a supervised way, the feature cannot be used to classify the other task. If the positive samples share only one type of semantics, the standard contrastive learning approach (SimCLR and MoCo) can learn a good representation for the shared type of semantics and achieve similar performance as supervised training while totally fail on the other one. However, if both semantics are shared between positive samples, only one of them (the background) will be learned and the performance is quite similar to contrastive learning on positive samples that only share the same background. This shows that when two types of independent semantics are presented in the input, contrastive learning will tend to learn only one of them (the shortcut) and ignore the other one.

%On the other hand, representation learning using only the missing patches reconstruction task can learn both semantics because the representation should contain enough information to reconstruct both digit and background. However, the learned representation's quality is not as good as that learned using contrastive learning. This is because the reconstruction task will tend to learn low-level features to recover missing pixels instead of high-level representation that are linearly separable.

%The combination of contrastive learning and the missing patches reconstruction task (\name) combines the advantages of both methods: it can learn representation for both semantics with high qualities. Unlike all traditional contrastive learning methods which only get near random results on digits classification ($\sim$90\% error rate), \name~can achieve 11.7\% error rate on digit classification which is quite close to supervised learning on both factors (7.0\%), while keeps performing well on background classification task and achieve comparable results as contrastive learning baselines. This shows that our method's effectiveness on extracting representation that is of high quality on all semantics shared between positive samples.
%\red{This is important in tasks where positive samples share not only semantics we care but also other potential shortcut semantics. For example in RF-based human sensing, RF signals contain information related to both human and background environments. We do not want expose our model to the risk of losing the information about human during the unsupervised learning. }


\subsection{Face Attribute Classification}
In this section, we evaluate \name~on FairFace \cite{karkkainen2019fairface}, a real world human face attribute dataset, where each image contains multiple semantics including gender, age, and ethnicity, as shown in Figure~\ref{fig:fairface}.

 %One critical property of FairFace is that each face contains multiple semantics including gender, age, and ethnicity. The different semantics require the model to learn different types of features. For example, to better determine the age of a person, the network may need to look at wrinkles, while this feature can be useless when determining a person's gender, where the length and texture of hair serve as important features.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{pos-neg-face}
\end{center}
\caption{Illustration of FairFace dataset. The positive pairs are from random cropping and random color jittering on an image twice. The negative pairs are sampled within batch.}\label{fig:fairface}
\vskip -0.1in
\end{figure}


\subsubsection{Experiment Setup}
\noindent\textbf{Reconstructive Setting.}
We use the strategy in \cite{pathak2016context} to mask out  $3$ to $5$ rectangles with a random sidesize between $7$ to $12$ pixels at random locations in the image. We fill the masked rectangles with the mean pixel value.

\noindent\textbf{Contrastive Setting.}
For contrastive learning, we follow the strategy in \cite{chen2020simple} to sample positive and negative pairs. We apply random cropping and random color jittering on an image twice to generate positive pairs. The negative pairs are sampled within batch. 
%Typical data samples are shown in Figure \ref{fig:fairface}.

\noindent\textbf{Network Structure.}
We use a standard ResNet-18 for the encoder network $E$. The decoder network $D$ is a symmetric deconvolutional network. The projection head $H$ for contrastive learning is a 2-layer non-linear head which embed the feature into a 128-dimensional unit sphere.

\noindent\textbf{Evaluation Metric.}
We evaluate the learned representations on three downstream tasks: age, gender and ethnicity classification. 
For the training of the downstream tasks, we freeze the encoder and train a linear layer for each task to classify the features. For the supervised baselines, supervised (a), (g) and (e) are trained on the single task of age, gender and ethnicity, respectively, while supervised (all) is jointly trained on all the three tasks.

\noindent\textbf{Baselines.}
We compare IPCL with SimCLR. For SimCLR, we use the same sampling strategy and network structure as our \name. We also fine-tune the hyper-parameters of SimCLR to achieve its best performance.

\subsubsection{Results}

Table \ref{tab:result-face} compares the performance of state-of-the-art contrastive learning (SimCLR) and \name~on the FairFace dataset.  
As shown by the supervised baselines, the three tasks share some common features since network trained on one of the task can also be used to classify other tasks with reasonable accuracy. However, each task also has its unique features since there are still big performance gaps between network trained on the specific task of interest and networks trained on the other two tasks. The table also shows that \name's performances on age and gender are significantly better than SimCLR. In fact, SimCLR's performance on age and gender are similar to that of supervised learning on ethnicity alone ($\sim$56\% and $\sim$21\% error rate, respectively).  \name\ improves over SimCLR's performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance to SimCLR on ethnicity classification (38.8\% vs. 37.7\%). This further demonstrates \name's ability to preserve useful information  that could be ignored by contrastive learning. 
 
 

\begin{table}[h]
\centering
\begin{tabular}{l |@{\hspace{0.1cm}} c@{\hspace{0.1cm}} c @{\hspace{0.1cm}}c @{\hspace{0.1cm}}c}\hline
 Method & \begin{tabular}{@{}c@{}}age cls. \\ error rate (\%)\end{tabular}  & \begin{tabular}{@{}c@{}}gender cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}ethnicity cls. \\ error rate (\%)\end{tabular} \\
\hline
\multirow{ 1}{*}{SimCLR}  & 55.7  & 21.4  & 37.7  \\\hline

\multirow{ 1}{*}{\textbf{\name~(ours)}}  & 50.0  & 12.8  & 38.8\\\hline

\multirow{ 1}{*}{Supervised (a)}  & 44.5 & 21.3  & 54.9 \\

\multirow{ 1}{*}{Supervised (g)}  & 56.7 & 7.5  & 54.6  \\

\multirow{ 1}{*}{Supervised (e)}  & 57.9 & 23.2  & 28.6  \\

\multirow{ 1}{*}{Supervised (all)}  & 45.2 & 8.1  &  29.2 \\

\hline
\end{tabular}
\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of age, gender and ethnicity classification.}}
\label{tab:result-face}
\end{table}


==> source/experiment-rgb-6.tex <==
\subsection{Experiments with RGB Data}
\vspace{-2pt}\noindent
\textbf{Dataset.} To demonstrate the ability of \name~on avoiding shortcuts and provide a  more generalized representation, we evaluate \name~on four different RGB datasets:

\textit{ImageNet-100:} ImageNet-100 a subset of ImageNet that contains randomly selected 100 classes from ImageNet and is widely used in prior works \cite{xiao2020should,tian2019contrastive}. We compare \name~with multiple contrastive learning baselines on ImageNet-100 under different data augmentation settings.  

\textit{Colorful-MNIST:} To better understand the impact of shortcuts on contrastive learning and how \name~resolves this issue, we first evaluate \name on a synthetic dataset proposed by the authors of~\cite{tian2020makes}. It is constructed by assigning each digit from MNIST a background object image selected randomly from the STL-10 dataset. Hence, each image in the Colorful-MNIST dataset has two types of semantic information that correspond to the digit class and the background object class. Figure~\ref{fig:intro} shows some typical samples from this dataset.

\textit{FairFace:} FairFace \cite{karkkainen2019fairface} is a real world human face attribute classification dataset, where each image contains multiple semantics including gender, age, and ethnicity. 

\textit{MPII:} MPII~\cite{andriluka20142d} human pose dataset contains images of everyday human activities, and is one of the most common dataset for the task of human pose estimation.


\vspace{-2pt}\noindent
\textbf{Baselines.}
We use state-of-the-art contrastive learning methods as baselines, including SimCLR \cite{chen2020simple}, MoCo \cite{chen2020improved}, CPC \cite{henaff2019data} and BYOL \cite{grill2020bootstrap}. The same network structure, batch size and training epochs is used for all baselines and for \name's contrastive branch. More implementation details are provided in Appendix.

%\noindent\textbf{Evaluation Metric.}
%We evaluate the representations learned by \name\ and the baselines by using them to train two linear classifiers for two downstream tasks: digit classification and background object classification.  We report the error rate for each method.  

\subsubsection{RGB Results}
\label{sec:rgb}

We report the main results in this section for all RGB datasets. All training details, hyper-parameter settings, and additional results are provided in Appendix.


\textbf{ImageNet-100.} We first compare \name~and baseline self-supervised approaches on image classification task on ImageNet-100. The results are shown in Table \ref{tab:imgnet-100}. It is known that shortcuts such as color distribution can be very harmful to the performance of contrastive learning. As a results, previous works uses strong augmentations to remove these shortcuts. On the other hand, \name~is much more robust to the choice of image augmentations than contrastive methods. In Table \ref{tab:imgnet-100}, we show that the performance of \name~is much less affected than the performance of contrastive baselines when removing color distortions from the set of image augmentations. When image augmentations are reduced to mere random crops, \name~still displays good performance (only -7.0 from baseline) while the performance of all other contrastive baselines drops significantly. This demonstrate that \name~can learn good representations even in the presence of shortcut such as color distribution.

\textbf{Digit \& Background Classification.} To explicitly analyze the shortcut problem, we show the performance of different self-supervised learning approaches digit and background classification results on Colorful-MNIST dataset when there exists short-cuts within positive samples.
 
We evaluate the performances of \name~and baselines under both fixed feature extractor setting and fine-tuning setting. Two linear classifiers are added on top of the pre-trained feature extractor for two downstream tasks: digit classification and background object classification. For the fixed feature extractor setting, only the two linear classifiers are trained; for the fine-tuning setting, the feature extractor is trained together with the classifiers.

Table \ref{tab:result-toy} reports the accuracy for each method. It reveals the following findings:
\begin{Itemize}
\item
 None of the contrastive learning baselines can learn features that capture information relevant to digit classification. In fact, their accuracy on digit classification (15\% to 16\%) is similar to the accuracy of a supervised method where the feature extractor was trained only on background object classification with no information about digits ($\sim$12\%).  The contrastive learning baselines perform reasonably well on background object classification with an accuracy $\sim$10\% lower than a supervised method trained on that task. This indicates that the background object features played the role of a shortcut for contrastive learning, i.e., those features were sufficient to contrast positive and negative samples, and hence there was no need for contrastive learning to learn digit-related features. 
 \item \name\ on the other hand learned a representation that is useful for both digit and background object classifications. Its accuracy on background object classification is comparable to the baselines, but its accuracy on digit classification is $\sim$70\% higher than the contrastive baselines.  Further, because of its contrastive branch, \name~can learn better features for both digit and background classification than inpainting. 
 (The Appendix provides a tSNE visualization of the learned features.)
\end{Itemize}  


% \usepackage{multirow}
% \usepackage{hhline}

%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{trainingcurve}
%\end{center}
%\caption{Training curve of contrastive loss using different methods.}\label{fig:trainingcurve}
%\vskip -0.1in
%\end{figure}


 
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{feat-vis}
%\end{center}
%\vskip -0.15in 
%\caption{Feature visualization of supervised learning, SimCLR and IPCL using tSNE on Colorful-Moving-MNIST.}\label{fig:image-tsne}
%\vskip -0.1in
%\end{figure}
%
%
%We further visualize the features learned by SimCLR, \name~and supervised learning in Figure \ref{fig:image-tsne} using tSNE. The left column is colored using background object labels, and the right column is colored using digit labels. Features generated by both supervised learning and \name~forms clusters under both coloring methods, while SimCLR only shows clustering when colored using background object label. This further shows that contrastive learning will focus on certain shortcut and ignore features relevant to other tasks, while features learned by \name~can preserve both information and achieve good performance on both downstream tasks.
\textbf{Face Attribute Classification.} 
% as shown in Figure~\ref{fig:fairface}. 
%\begin{wraptable}{r}{70mm}
%\end{wraptable}
%\begin{table}[h]

%\end{subtable}
%\end{tabular}
%\vspace{-15pt}
%\end{table}
Table \ref{tab:result-face} compares the performance of state-of-the-art contrastive learning and \name~on the FairFace dataset.  
As shown by the supervised baselines, the three tasks share some common features since network trained on one of the task can also be used to classify other tasks with reasonable accuracy. However, each task also has its unique features since there are still big performance gaps between network trained on the specific task of interest and networks trained on the other two tasks. The table also shows that \name's performances on age and gender are significantly better than all baselines. Although achieving the best performance among the four baselines, BYOL's performance on age and gender are similar to that of supervised learning on ethnicity label alone ($\sim$44\% and $\sim$79\% accuracy, respectively). This is possibly because the shortcut for contrastive learning is more related to the ethnicity than to age and gender. \name\ improves over baselines' performances on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%).  This further demonstrates \name's ability to preserve useful information  that could be ignored by contrastive learning. 

\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc} 
\toprule[1.5pt]
Method              & \multicolumn{2}{c|}{SimCLR} & \multicolumn{2}{c|}{MoCo} & \multicolumn{2}{c|}{BYOL} & \multicolumn{2}{c|}{\bf \name (ours)}     & \multicolumn{2}{c}{\bf \textsc{Improvement}}          \\ 
\cmidrule{1-11}
\bf\textsc{Metric}              & \bf\textsc{Top-1} & \bf\textsc{Drop}                & \bf\textsc{Top-1} & \bf\textsc{Drop}              &\bf \textsc{Top-1} &\bf\textsc{Drop}              & \bf\textsc{Top-1}         & \bf\textsc{Drop}          & \bf\textsc{Top-1}          & \bf\textsc{Drop}                    \\ 
\midrule\midrule
Baseline            & 79.1  & /                   & 81.2  & /                 &  81.4  & /                 & 81.0          & /             & \textcolor{lightblue}{\textbf{-0.4}}  & /                       \\ 
%\cmidrule{1-2}\cline{3-3}\cmidrule{4-4}\cline{5-5}\cmidrule{6-6}\cline{7-8}\cmidrule{9-10}\cline{11-11}
\midrule
Remove flip         & 78.6  & -0.5                & 80.8  & -0.6              & \bf 80.7  & -0.5              & 80.6          & \bf -0.4          & \textcolor{lightblue}{\textbf{-0.2}}  & \textcolor{darkgreen}{\textbf{+0.1}}           \\
Remove blur         & 76.5  & -2.6                & 79.5  & -1.9              & 79.6  & -1.8              & \textbf{80.0} & \textbf{-1.0} & \textcolor{darkgreen}{\textbf{+0.4}} & \textcolor{darkgreen}{\textbf{+0.8}}  \\
Crop  color only    & 75.4  & -3.7                & 79.0  & -2.2              & 78.9  & -2.5              & \bf 79.8           & \bf -1.2           & \textcolor{darkgreen}{\textbf{+0.8}}  & \textcolor{darkgreen}{\textbf{+1.0}}  \\
Remove color jitter & 71.3  & -7.8                & 78.1  & -3.1              & \bf 80.0  & \bf-1.4              & 79.5           & -1.5           & \bf\textcolor{lightblue}{{-0.5}}  & \textcolor{lightblue}{\textbf{-0.1}}  \\
Remove grayscale    & 69.7  & -9.4                & 76.5  & -4.7              & 75.4  & -6.0              & \bf 78.0           & \bf -3.0           & \textcolor{darkgreen}{\textbf{+1.5}}  & \textcolor{darkgreen}{\textbf{+1.7}}  \\
Remove color        & 50.4  & -28.7               & 68.0  & -13.2             & 69.9  & -11.5             & \textbf{75.5} & \textbf{-5.5} & \textcolor{darkgreen}{\textbf{+5.6}}  & \textcolor{darkgreen}{\textbf{+6.0}}  \\
Crop  blur only     & 48.8  & -30.3               & 67.5  & -13.7             & 68.4  & -13.0             & \bf 74.9           & \bf -6.1           & \textcolor{darkgreen}{\textbf{+6.5}}  & \textcolor{darkgreen}{\textbf{+6.9}}  \\
Crop flip only      & 47.1  & -32.0               & 67.2  & -14.0             & 67.7  & -13.7             & \textbf{74.2} & \textbf{-6.8} & \textcolor{darkgreen}{\textbf{+6.5}}  & \textcolor{darkgreen}{\textbf{+6.9}}  \\
Crop only           & 46.9  & -32.2               & 66.7  & -14.5             & 66.9  & -14.5             & \textbf{74.0} & \textbf{-7.0} & \textcolor{darkgreen}{\textbf{+7.1}}  & \textcolor{darkgreen}{\textbf{+7.5}}  \\
\bottomrule[1.5pt]
\end{tabular}
}
\end{threeparttable}
\vspace{3pt}
\footnotesize{(a) ImageNet-100 \textsc{Top-1} and its \textsc{Drop} w.r.t. full augmentations.}\vspace{3pt}
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc} 
\toprule[1.5pt]
 Method              & \multicolumn{2}{c|}{SimCLR} & \multicolumn{2}{c|}{MoCo} & \multicolumn{2}{c|}{BYOL} & \multicolumn{2}{c|}{\bf \name (ours)}     & \multicolumn{2}{c}{\bf \textsc{Improvement}}          \\ 
\cmidrule{1-11}
\bf\textsc{Metric}              & \bf\textsc{Top-5} & \bf\textsc{Drop}                & \bf\textsc{Top-5} & \bf\textsc{Drop}              &\bf \textsc{Top-5} &\bf\textsc{Drop}              & \bf\textsc{Top-5}         & \bf\textsc{Drop}          & \bf\textsc{Top-5}          & \bf\textsc{Drop}                    \\ 
\midrule\midrule
Baseline            & 94.2  & /                   & 95.1  & /                 & \bf 95.2  & /                 & 95.0          & /             & \textcolor{lightblue}{\textbf{-0.2}}  & /                       \\ 
%\cmidrule{1-2}\cline{3-3}\cmidrule{4-4}\cline{5-5}\cmidrule{6-6}\cline{7-8}\cmidrule{9-10}\cline{11-11}
\midrule
Remove flip         & 93.9  & -0.3                & 94.9  & -0.2              & \bf 95.0  & -0.2              &   94.7        & -0.3          & \textcolor{lightblue}{\textbf{-0.2}}  & \textcolor{darkgreen}{\textbf{+0.0}}           \\
Remove blur         & 92.6  & -1.6                & 94.7  & -0.4              & 94.7  & -0.5              & \textbf{94.7} & \textbf{-0.3} & \textcolor{darkgreen}{\textbf{+0.0}} & \textcolor{darkgreen}{\textbf{+0.1}}  \\
Crop  color only    & 92.1  & -2.1                & 94.4  & -0.7              & 94.3  & -0.9              & \bf 94.5           & \bf-0.5           & \textcolor{darkgreen}{\textbf{+0.1}}  & \textcolor{darkgreen}{\textbf{+0.2}}  \\
Remove color jitter & 89.4  & -4.7                & 93.9  & -1.2             & \bf 94.7  & -0.5              & 94.2           & -0.9           & \bf\textcolor{lightblue}{{-0.5}}  & \textcolor{lightblue}{\textbf{-0.4}}  \\
Remove grayscale    & 88.7  & -5.5                & 92.6  & -2.5             & 93.2  & -2.0              & \bf 93.7           & \bf -1.3           & \textcolor{darkgreen}{\textbf{+0.5}}  & \textcolor{darkgreen}{\textbf{+0.7}}  \\
Remove color        & 74.7  & -19.5               & 88.9  & -6.2             & 89.5  & -5.7             & \textbf{93.2} & \textbf{-1.8} & \textcolor{darkgreen}{\textbf{+3.7}}  & \textcolor{darkgreen}{\textbf{+3.9}}  \\
Crop  blur only     & 73.0  & -21.2               & 88.7  & -6.4             & 89.0  & -6.2             & 92.9           & -2.1           & \textcolor{darkgreen}{\textbf{+3.9}}  & \textcolor{darkgreen}{\textbf{+4.1}}  \\
Crop flip only      & 71.6  & -22.6               & 88.3  & -6.8             & 88.7  & -6.5             & \textbf{92.7} & \textbf{-2.3} & \textcolor{darkgreen}{\textbf{+4.0}}  & \textcolor{darkgreen}{\textbf{+4.2}}  \\
Crop only           & 71.4  & -22.8               & 88.0  & -7.1             & 88.2  & -7.0             & \textbf{92.5} & \textbf{-2.5} & \textcolor{darkgreen}{\textbf{+4.3}}  & \textcolor{darkgreen}{\textbf{+4.5}}  \\
\bottomrule[1.5pt]
\end{tabular}
}
\end{threeparttable}
\footnotesize{(b) ImageNet-100 \textsc{Top-5} and its \textsc{Drop} w.r.t. full augmentations.}

\vspace{-5pt}
\caption{\footnotesize{Experiment results on ImageNet-100 dataset with different image augmentations using different self-supervised learning techniques. We compare SimCLR, MoCo and BYOL with \name~because they use the same set of augmentations.}}
\label{tab:imgnet-100}

\begin{tabular}{cc}

%\end{tabular}
\begin{minipage}{.44\linewidth}
\centering
\vspace{7pt}
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{c|c|c|c} 
%\hline
\toprule[1.5pt]
\multicolumn{2}{c|}{\textsc{Metric}}                                                                                  & \begin{tabular}[c]{@{}c@{}}\textsc{Digit cls} \\ \textsc{Acc.} (\%) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textsc{Bkgd cls} \\ \textsc{Acc.} (\%) \end{tabular}  \\ 
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fixed}\\\textsc{feature}\\\textsc{extractor} \end{tabular}} &SimCLR                    & 14.9                                                                  & 47.3                                                                  \\
&MoCo                                                                                                         & 15.7                                                                  & 48.5                                                                  \\
&CPC                                                                                                          & 15.8                                                                  & 35.2                                                                  \\ 
&BYOL & 15.5 & \textbf{49.0} \\
%Recontruction   & 15.3  & 65.0 \\
%&Inpainting                                                                                                          & 15.3                                                                 & 65.0\\      
\cmidrule{2-4}
&\bf{\name~(ours)}                                                                                      & \bf 88.3                                                                  & 46.5                                                                  \\ 
&\bf \textsc{Improvement}                                                                                      & \bf \textcolor{darkgreen}{\textbf{+72.5}}                                                                & \textcolor{lightblue}{\textbf{-2.5}} \\ 
%\hhline{=-==}
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fine-}\\\textsc{tuning} \end{tabular}} & SimCLR                               & 92.4                                                                   & 54.8                                                                  \\
& MoCo                                                                                                         & 92.7                                                                   & 54.9                                                                  \\
&CPC                                                                                                      & 92.3                                                                   & 54.7                                                                  \\ 
%&Inpainting                                                                                                          & 7.1                                                                   & 45.5                                                                  \\ 
&BYOL & 92.7 & \textbf{54.9} \\
\cmidrule{2-4}
&\bf{\name~(ours)}                                                                                    & \bf 93.3                                                                   & 54.7                                                                  \\ 
&\bf \textsc{Improvement}                                                                                     & \bf \textcolor{darkgreen}{\textbf{+0.6}}                                                               & \textcolor{lightblue}{\textbf{-0.2}}                                                             \\ 
\midrule\midrule
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{digit}}                                                                      & 96.1                                                                   & 11.4                                                                  \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{bkgd}}                                                                       & 12.9                                                                  & 56.7                                                                  \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{digit} \&  \textsc{bkgd}}                                                                & 93.0                                                                   & 54.5                                                                  \\
%\hline
\bottomrule[1.5pt]
\end{tabular}
\label{tab:result-toy}
}
\end{threeparttable}
\caption{\footnotesize{We study the representation quality learned from Colorful-MNIST using different unsupervised methods. We evaluate the learned representation on the downstream tasks of digit classification and background object classification.}}
%\end{subtable}
%\hfill

%\begin{subtable}
\end{minipage}
&
\begin{minipage}{.53\linewidth}
\centering
\begin{threeparttable}
\resizebox{.98\textwidth}{!}{
\begin{tabular}{c|c|c|c|c} 
%\hline
\toprule[1.5pt]
\multicolumn{2}{c|}{\textsc{Metric}}                                                                                  & \begin{tabular}[c]{@{}c@{}}\textsc{Age cls} \\ \textsc{Acc.} (\%) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textsc{Gender cls} \\ \textsc{Acc.} (\%) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textsc{Ethn. cls} \\ \textsc{Acc.} (\%) \end{tabular} \\ 
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fixed}\\\textsc{feature}\\\textsc{extractor} \end{tabular}} &SimCLR                   & 43.9  & 78.1  & 61.7                                                                  \\
&MoCo                      & 44.5  & 78.6  & 61.9                                                                  \\
&CPC                                                                                                         & 43.5  & 76.2  & 61.0                                                                  \\ 
&BYOL & 44.3  & 78.6  & \textbf{62.3}  \\
%Recontruction   & 15.3  & 65.0 \\
%&Inpainting                                                                                                          & 15.3                                                                 & 65.0\\      
\cmidrule{2-5}
&\bf{\name~(ours)}  & \bf{50.0}  & \bf{87.2}  & 61.2     \\ 
&\bf \textsc{Improvement}                                                                                      & \bf \textcolor{darkgreen}{\textbf{+5.7}}  & \textcolor{darkgreen}{\textbf{+8.6}}  & \textcolor{lightblue}{\textbf{-1.1}} \\ 
%\hhline{=-==}
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fine-}\\\textsc{tuning} \end{tabular}}
& SimCLR  &54.3 & 91.1 & 69.1   \\
& MoCo & 54.7 & 91.3 & 69.2  \\
&CPC  & 54.2 & 91.0 & 68.8    \\ 
%&Inpainting                                                                                                          & 7.1                                                                   & 45.5                                                                  \\ 
&BYOL & 54.6 &91.5 & \textbf{69.3} \\
\cmidrule{2-5}
&\bf{\name~(ours)}                                                                                    &  \textbf{55.3}                                                                  &  \textbf{92.3}                 & 69.0                                                 \\ 
&\bf \textsc{Improvement}                                                                                     & \bf \textcolor{darkgreen}{\textbf{+0.6}}      & \bf \textcolor{darkgreen}{\textbf{+0.8}}                                                         & \textcolor{lightblue}{\textbf{-0.3}}                                                             \\ 
\midrule\midrule
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{Age}}                                                                      & 55.5 & 78.8  & 45.1                                                                 \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{gender}}                                                                        & 43.3 & 92.5  & 45.4                                                                 \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{Ethn.}}                                                                & 42.1 & 76.8  & 69.4                                                                \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{All}}                                                                & 54.8 & 91.9  &  68.8                                                                \\
%\hline
\bottomrule[1.5pt]
\end{tabular}
\label{tab:result-face}
}
\caption{\footnotesize{We study the representation quality learned from FairFace using different unsupervised learning methods. We evaluate the learned representation on downstream tasks of age, gender and ethnicity classification.}}
\end{threeparttable}
\end{minipage}
\end{tabular}

\vspace{-5pt}
\end{table*}

\textbf{Human Pose Estimation.} We list the performance for {\name} and various baseline approaches in Table \ref{tab:result-pose}. Under both settings, \name~outperforms contrastive baselines: 3.7 PCKh under fixed feature encoder setting and 0.7 PCKh under fine-tuning setting. This is possibly because contrastive learning can fall into shortcuts that are irrelevant to human poses such as the texture of the clothes. On the other hand, \name~is able to learn abstract and information-preserving features and thus achieve good performance. 

\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
\toprule[1.5pt]
\multicolumn{2}{c|}{\textsc{Metric}} & Head$^\uparrow$ & Shoulder$^\uparrow$ & Elbow$^\uparrow$ & Wrist$^\uparrow$ & Hip$^\uparrow$ & Knee$^\uparrow$ & Ankle$^\uparrow$ & PCKh$^\uparrow$ \\ 
\midrule
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fixed}\\\textsc{feature}\\\textsc{extractor} \end{tabular}} 
%&Random init & 30.3 & 31.4 & 20.2 & 13.8 & 25.8 & 18.1 & 17.5 & 23.9 \\

&SimCLR & 78.4 & 74.6 & 56.7 & 45.2 & 61.8 & 51.3 & 47.1 & 60.8 \\
&MoCo & 79.2 & 75.1 & 57.4 & 45.9 & 62.4 & 52.0 & 47.6 & 61.4 \\

&CPC & 78.0 & 74.3 & 56.0 & 44.8 & 61.2 & 51.4 & 46.5 & 60.3 \\
&BYOL & 79.1 & 75.0 & 57.1 & 46.0 & 62.4 & 52.2 & 47.7 & 61.4 \\
%&Inpainting  & 83.4 & 75.2 & 53.6 & 44.4 & 56.4 & 44.3 & 45.7 & 59.0  \\ 
%Recontruction   & 15.3  & 65.0 \\   
\cmidrule{2-10}
&\bf \name~(ours)                                                                                      & \bf 85.7 & \bf 78.8 & \bf 61.7 & \bf 51.3 & \bf 64.4 & \bf 55.6 & \bf 49.2 & \bf 65.1                                                                                            \\ 
&\bf \textsc{Improvements}                                                                                      
& \bf \textcolor{darkgreen}{\textbf{+6.5}}
& \bf \textcolor{darkgreen}{\textbf{+3.7}} 
& \bf \textcolor{darkgreen}{\textbf{+4.3}} 
& \bf \textcolor{darkgreen}{\textbf{+5.3}} 
& \bf \textcolor{darkgreen}{\textbf{+2.0}} 
& \bf \textcolor{darkgreen}{\textbf{+3.4}} 
& \bf \textcolor{darkgreen}{\textbf{+1.5}}
& \bf \textcolor{darkgreen}{\textbf{+3.7}}                                                                                          \\ 
%\hhline{=-==}
\midrule
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fine-}\\\textsc{tuning} \end{tabular}} 
& SimCLR & 96.2 & 94.7 & 87.3 & 81.2 & 87.5 & 81.0 & 77.2 & 87.1 \\
& MoCo & 95.9 & 94.7 & 87.5 & 81.6 & 87.4 & 81.7 & 76.9 & 87.2 \\
& CPC & 96.0 & 94.5 & 87.0 & 81.1 & 87.3 & 80.8 & 77.0 & 87.0 \\
& BYOL & 96.2 & 94.8 & 87.5 & 81.4 & 87.6 & 81.5 & 77.0 & 87.2 \\
%&Inpainting & 96.3 & \bf 95.2 & 87.9 & 82.1 & 87.8 & 82.5 & 77.6 & 87.7 \\ 
\cmidrule{2-10}
&\bf \name~(ours)                                                                                     & \bf 96.3 & \bf 94.9 & \bf 88.1 & \bf 82.3 & \bf 87.9 & \bf 82.8 & \bf 77.8 & \bf 87.8                                                                                                                                                                        \\
&\bf \textsc{Improvements}                                                                                      
& \bf \textcolor{darkgreen}{\textbf{+0.1}} 
& \bf \textcolor{darkgreen}{\textbf{+0.1}}  
& \bf \textcolor{darkgreen}{\textbf{+0.6}} 
& \bf \textcolor{darkgreen}{\textbf{+0.7}}
& \bf \textcolor{darkgreen}{\textbf{+0.3}} 
& \bf \textcolor{darkgreen}{\textbf{+1.1}} 
& \bf \textcolor{darkgreen}{\textbf{+0.6}} 
& \bf \textcolor{darkgreen}{\textbf{+0.6}}                                                                                            \\ 

\midrule
\midrule
\multicolumn{2}{c|}{\textsc{Supervised}}     & 96.3 & 95.1 & 87.9 & 82.2 & 87.8 & 82.7 & 77.8 & 87.7\\

\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-7pt}
\caption{We study the representation quality learned from MPII using different unsupervised methods. We evaluate the learned representation on the downstream task of human pose estimation. $\uparrow$ indicates the larger the value, the better the performance. Note that the pose estimation here is in 2D image and the RF-based pose estimation in the main paper is in 3D, so the evaluation metrics are also different.}
\label{tab:result-pose}
\vspace{-5pt}
\end{table*}

\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l | c |c c|c c c|c c c}
%\hline
\toprule[1.5pt]
  Tasks & 3D Pose Estimation & \multicolumn{2}{c|}{Action Recognition} & \multicolumn{3}{c|}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
\midrule
 \multirow{ 2}{*}{Metrics} &  \multirow{ 2}{*}{Pose \textsc{Err}.$^\downarrow$ (mm)} & \multicolumn{2}{c|}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ & & & & & & \\
\midrule\midrule
Random init & 60.1 & 70.5  & 53.3 & 28.1 & 43.8 & 68.8 & 30.1 & 54.2 & 74.6 \\
\midrule
SimCLR & 80.5 & 4.2 & 0 & 29.8 & 44.1 & 67.5 & 31.2 & 55.1 & 73.8 \\
MoCo & 77.2 & 5.1 & 0.18 & 29.1 & 44.7 & 65.3 & 30.5 & 54.5 & 74.0 \\
CPC & 78.7 & 3.6 & 0 & 30.0 & 42.7 & 69.5 & 30.7 & 54.0 & 75.3 \\
BYOL & 79.3 & 4.7 & 0 & 29.5 & 44.4 & 66.7 & 30.7 & 54.6 & 73.5 \\
%Inpainting & 51.1 & 72.3 & 65.5 & 49.8 & 73.1 & 90.5 & 38.5 & 64.2 & 84.7 \\
\midrule
\textbf{\name(ours)} & \textbf{46.6} & \textbf{86.5} & \textbf{83.1} & \textbf{54.5} & \textbf{78.7} & \textbf{93.0} & \textbf{43.3} & \textbf{72.4} & \textbf{87.6}\\
\bf \textsc{Improvement} 
& \textcolor{darkgreen}{\textbf{-30.6}} 
 & \textcolor{darkgreen}{\textbf{+81.4}} 
 & \textcolor{darkgreen}{\textbf{+82.9}} 
 & \textcolor{darkgreen}{\textbf{+24.5}}  
 & \textcolor{darkgreen}{\textbf{+34.0}} 
 & \textcolor{darkgreen}{\textbf{+23.5}} 
 & \textcolor{darkgreen}{\textbf{+11.8}}
 & \textcolor{darkgreen}{\textbf{+17.3}} 
 & \textcolor{darkgreen}{\textbf{+12.3}}  
\\\midrule\midrule
\textsc{Supervised} & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
%\hline
\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-5pt}
\caption{Evaluation of different models on different RF datasets and tasks under fixed feature extractor setting, where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and the weights are frozen during downstream training. $\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}
\label{tab:result-fixed}
\vspace{5pt}
%\end{table*}

%\begin{table*}[t]
\centering
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l | c |c c|c c c|c c c}
%\hline
\toprule[1.5pt]
  Tasks & 3D Pose Estimation & \multicolumn{2}{c|}{Action Recognition} & \multicolumn{3}{c|}{Person Re-ID (Campus)} & \multicolumn{3}{c}{Person Re-ID (Home)} \\
\midrule
 \multirow{ 2}{*}{Metrics} &  \multirow{ 2}{*}{Pose \textsc{Err}.$^\downarrow$ (mm)} & \multicolumn{2}{c|}{mAP$^\uparrow$}  & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} & \multirow{ 2}{*}{mAP$^\uparrow$} & \multirow{ 2}{*}{CMC-1$^\uparrow$} & \multirow{ 2}{*}{CMC-5$^\uparrow$} \\
 & & $\theta=0.1$ & $\theta=0.5$ & & & & & & \\
\midrule\midrule
Random init & 38.4 & 90.1  & 87.8 & 59.5 & 82.1 & 95.5 & 46.4 & 74.6 & 89.5 \\
\midrule
SimCLR & 38.8 & 89.8 & 87.4 & 59.0 & 81.7 & 94.1 & 45.9 & 73.8 & 88.5 \\
MoCo & 38.3 & 89.7 & 87.2 & 59.3 & 82.0 & 94.5 & 46.4 & 74.3 & 89.7 \\
CPC & 38.6 & 89.9 & 87.5 & 59.4 & 81.5 & 94.0 & 46.0 & 74.5 & 89.1 \\
BYOL & 38.5 & 89.7 & 87.2 & 59.4 & 81.9 & 94.5 & 46.6 & 74.5 & 89.5 \\
%Inpainting & 36.2 &  91.7 & 88.7 & 60.1 & 83.3 & 95.5 & 47.5 & 75.3 & 90.3\\
\midrule
\textbf{\name (ours)} & \textbf{35.1} & \textbf{92.5} & \textbf{89.6} & \textbf{60.8} & \textbf{84.2} & \textbf{96.0} & \textbf{48.1} & \textbf{76.1} & \textbf{91.0}\\
\bf \textsc{Improvement} 
& \textcolor{darkgreen}{\textbf{-3.7}} 
 & \textcolor{darkgreen}{\textbf{+2.6}} 
 & \textcolor{darkgreen}{\textbf{+2.1}}  
 & \textcolor{darkgreen}{\textbf{+1.4}}  
 & \textcolor{darkgreen}{\textbf{+2.2}}  
 & \textcolor{darkgreen}{\textbf{+1.5}}  
 & \textcolor{darkgreen}{\textbf{+1.5}}  
 & \textcolor{darkgreen}{\textbf{+1.6}}  
 & \textcolor{darkgreen}{\textbf{+1.3}}  \\

\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-5pt}
\caption{Evaluation of different models on different RF datasets and tasks under fine-tuning setting, where the RF feature encoder is initialized with pre-trained model using unsupervised learning methods, and then fine-tuned during downstream training. $\downarrow$ indicates the smaller the value, the better the performance; $\uparrow$ indicates the larger the value, the better the performance.}
\label{tab:result-finetune}
\vspace{-10pt}
\end{table*}



%We first study the representation quality learned using contrastive learning and show the performance on downstream tasks.As shown in Table \ref{tab:result-toy}, if we only train the network on one of the factors in a supervised way, the feature cannot be used to classify the other task. If the positive samples share only one type of semantics, the standard contrastive learning approach (SimCLR and MoCo) can learn a good representation for the shared type of semantics and achieve similar performance as supervised training while totally fail on the other one. However, if both semantics are shared between positive samples, only one of them (the background) will be learned and the performance is quite similar to contrastive learning on positive samples that only share the same background. This shows that when two types of independent semantics are presented in the input, contrastive learning will tend to learn only one of them (the shortcut) and ignore the other one.

%On the other hand, representation learning using only the missing patches reconstruction task can learn both semantics because the representation should contain enough information to reconstruct both digit and background. However, the learned representation's quality is not as good as that learned using contrastive learning. This is because the reconstruction task will tend to learn low-level features to recover missing pixels instead of high-level representation that are linearly separable.

%The combination of contrastive learning and the missing patches reconstruction task (\name) combines the advantages of both methods: it can learn representation for both semantics with high qualities. Unlike all traditional contrastive learning methods which only get near random results on digits classification ($\sim$90\% error rate), \name~can achieve 11.7\% error rate on digit classification which is quite close to supervised learning on both factors (7.0\%), while keeps performing well on background classification task and achieve comparable results as contrastive learning baselines. This shows that our method's effectiveness in extracting representation that is of high quality on all semantics shared between positive samples.
%\red{This is important in tasks where positive samples share not only semantics we care but also other potential shortcut semantics. For example in RF-based human sensing, RF signals contain information related to both human and background environments. We do not want expose our model to the risk of losing the information about human during the unsupervised learning. }


%\subsection{Face Attribute Classification}
%In this section, we evaluate \name~on FairFace \cite{karkkainen2019fairface}, a real world human face attribute dataset, where each image contains multiple semantics including gender, age, and ethnicity, as shown in Figure~\ref{fig:fairface}.
%
% %One critical property of FairFace is that each face contains multiple semantics including gender, age, and ethnicity. The different semantics require the model to learn different types of features. For example, to better determine the age of a person, the network may need to look at wrinkles, while this feature can be useless when determining a person's gender, where the length and texture of hair serve as important features.
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{pos-neg-face}
%\end{center}
%\caption{Illustration of FairFace dataset. The positive pairs are from random cropping and random color jittering on an image twice. The negative pairs are sampled within batch.}\label{fig:fairface}
%\vskip -0.1in
%\end{figure}
%
%
%\subsubsection{Experiment Setup}
%\noindent\textbf{Reconstructive Setting.}
%We use the strategy in \cite{pathak2016context} to mask out  $3$ to $5$ rectangles with a random sidesize between $7$ to $12$ pixels at random locations in the image. We fill the masked rectangles with the mean pixel value.
%
%\noindent\textbf{Contrastive Setting.}
%For contrastive learning, we follow the strategy in \cite{chen2020simple} to sample positive and negative pairs. We apply random cropping and random color jittering on an image twice to generate positive pairs. The negative pairs are sampled within batch. 
%%Typical data samples are shown in Figure \ref{fig:fairface}.
%
%\noindent\textbf{Network Structure.}
%We use a standard ResNet-18 for the encoder network $E$. The decoder network $D$ is a symmetric deconvolutional network. The projection head $H$ for contrastive learning is a 2-layer non-linear head which embed the feature into a 128-dimensional unit sphere.
%
%\noindent\textbf{Evaluation Metric.}
%We evaluate the learned representations on three downstream tasks: age, gender and ethnicity classification. 
%For the training of the downstream tasks, we freeze the encoder and train a linear layer for each task to classify the features. For the supervised baselines, supervised (a), (g) and (e) are trained on the single task of age, gender and ethnicity, respectively, while supervised (all) is jointly trained on all the three tasks.
%
%\noindent\textbf{Baselines.}
%We compare IPCL with SimCLR. For SimCLR, we use the same sampling strategy and network structure as our \name. We also fine-tune the hyper-parameters of SimCLR to achieve its best performance.
%
%\subsubsection{Results}
%
%Table \ref{tab:result-face} compares the performance of state-of-the-art contrastive learning (SimCLR) and \name~on the FairFace dataset.  
%As shown by the supervised baselines, the three tasks share some common features since network trained on one of the task can also be used to classify other tasks with reasonable accuracy. However, each task also has its unique features since there are still big performance gaps between network trained on the specific task of interest and networks trained on the other two tasks. The table also shows that \name's performances on age and gender are significantly better than SimCLR. In fact, SimCLR's performance on age and gender are similar to that of supervised learning on ethnicity alone ($\sim$56\% and $\sim$21\% error rate, respectively).  \name\ improves over SimCLR's performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance to SimCLR on ethnicity classification (38.8\% vs. 37.7\%). This further demonstrates \name's ability to preserve useful information  that could be ignored by contrastive learning. 
% 
% 
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.1cm}} c@{\hspace{0.1cm}} c @{\hspace{0.1cm}}c @{\hspace{0.1cm}}c}\hline
% Method & \begin{tabular}{@{}c@{}}age cls. \\ error rate (\%)\end{tabular}  & \begin{tabular}{@{}c@{}}gender cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}ethnicity cls. \\ error rate (\%)\end{tabular} \\
%\hline
%\multirow{ 1}{*}{SimCLR}  & 55.7  & 21.4  & 37.7  \\\hline
%
%\multirow{ 1}{*}{\textbf{\name~(ours)}}  & 50.0  & 12.8  & 38.8\\\hline
%
%\multirow{ 1}{*}{Supervised (a)}  & 44.5 & 21.3  & 54.9 \\
%
%\multirow{ 1}{*}{Supervised (g)}  & 56.7 & 7.5  & 54.6  \\
%
%\multirow{ 1}{*}{Supervised (e)}  & 57.9 & 23.2  & 28.6  \\
%
%\multirow{ 1}{*}{Supervised (all)}  & 45.2 & 8.1  &  29.2 \\
%
%\hline
%\end{tabular}
%\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of age, gender and ethnicity classification.}}
%\label{tab:result-face}
%\end{table}


==> source/experiment-rgb-7.tex <==
\section{Evaluation on RGB Data}

\vspace{-2pt}\noindent\textbf{Baselines.}
We use state-of-the-art contrastive learning methods as baselines, including SimCLR \cite{chen2020simple}, MoCo \cite{chen2020improved}, CPC \cite{henaff2019data} and BYOL \cite{grill2020bootstrap}. The same network structure, batch size, and training epochs are used for all baselines and \name's contrastive branch. Here we only compare contrastive learning with \name~, since reconstructive learning typically performs much worse than contrastive learning \cite{chen2020improved}. (In the appendix, we also compare \name\ to different reconstructive baselines.)

\vspace{-2pt}\noindent\textbf{RGB Datasets.} We run our experiments on the following datasets:
\begin{Itemize}
\item 
\textbf{ImageNet-100:} ImageNet-100 is widely used in prior works \cite{xiao2020should,tian2019contrastive}. It is a subset of ImageNet that contains 100 randomly selected classes from ImageNet. %We compare \name~with multiple contrastive learning baselines on ImageNet-100 under different data augmentation settings.  
\item
\textbf{MPII:} MPII~\cite{andriluka20142d}  is one of the most common dataset for the task of human pose estimation. It contains images of everyday human activities.
\item
\textbf{FairFace:} FairFace \cite{karkkainen2019fairface} is a human face attribute classification dataset, where each image contains multiple semantics including gender, age, and ethnicity. 
\item
\textbf{Colorful-MNIST:} This is a synthetic dataset used by~\cite{tian2020makes} to highlight the shortcut problem. It is constructed by assigning each digit from MNIST a background object image selected randomly from the STL-10 dataset. It supports two downstream tasks: digit and background classification.
\end{Itemize}

\begin{table*}[t]
\centering
\vspace{-5pt}
\caption{\footnotesize{Performance on ImageNet-100 with progressive removal of data augmentations for different self-supervised learning techniques. The baseline corresponds to the original set of augmentations used in SimCLR, MoCo and BYOL: random flip, random resized crop, color distortion, and random Gaussian blur.}}
\label{tab:imgnet-100}
\begin{threeparttable}
\footnotesize{(a) ImageNet-100 \textsc{Top-1} accuracy and its \textsc{Drop} w.r.t. inclusion of all augmentations.}\vspace{0pt}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc} 
\toprule[1.5pt]
Method              & \multicolumn{2}{c|}{SimCLR} & \multicolumn{2}{c|}{MoCo} & \multicolumn{2}{c|}{BYOL} & \multicolumn{2}{c|}{\bf \name (ours)}     & \multicolumn{2}{c}{\bf \textsc{Improvement}}          \\ 
\cmidrule{1-11}
\bf\textsc{Metric}              & \bf\textsc{Top-1} & \bf\textsc{Drop}                & \bf\textsc{Top-1} & \bf\textsc{Drop}              &\bf \textsc{Top-1} &\bf\textsc{Drop}              & \bf\textsc{Top-1}         & \bf\textsc{Drop}          & \bf\textsc{Top-1}          & \bf\textsc{Drop}                    \\ 
\midrule\midrule
Baseline            & 79.1  & /                   & 81.2  & /                 &  81.4  & /                 & 81.0          & /             & \textcolor{lightblue}{\textbf{-0.4}}  & /                       \\ 
%\cmidrule{1-2}\cline{3-3}\cmidrule{4-4}\cline{5-5}\cmidrule{6-6}\cline{7-8}\cmidrule{9-10}\cline{11-11}
\midrule
Remove flip         & 78.6  & -0.5                & 80.8  & -0.6              & \bf 80.7  & -0.5              & 80.6          & \bf -0.4          & \textcolor{lightblue}{\textbf{-0.2}}  & \textcolor{darkgreen}{\textbf{+0.1}}           \\
Remove blur         & 76.5  & -2.6                & 79.5  & -1.9              & 79.6  & -1.8              & \textbf{80.0} & \textbf{-1.0} & \textcolor{darkgreen}{\textbf{+0.4}} & \textcolor{darkgreen}{\textbf{+0.8}}  \\
Crop  color only    & 75.4  & -3.7                & 79.0  & -2.2              & 78.9  & -2.5              & \bf 79.8           & \bf -1.2           & \textcolor{darkgreen}{\textbf{+0.8}}  & \textcolor{darkgreen}{\textbf{+1.0}}  \\
%Remove color jitter & 71.3  & -7.8                & 78.1  & -3.1              & \bf 80.0  & \bf-1.4              & 79.5           & -1.5           & \bf\textcolor{lightblue}{{-0.5}}  & \textcolor{lightblue}{\textbf{-0.1}}  \\
%Remove grayscale    & 69.7  & -9.4                & 76.5  & -4.7              & 75.4  & -6.0              & \bf 78.0           & \bf -3.0           & \textcolor{darkgreen}{\textbf{+1.5}}  & \textcolor{darkgreen}{\textbf{+1.7}}  \\
Remove color distort.        & 50.4  & -28.7               & 68.0  & -13.2             & 69.9  & -11.5             & \textbf{75.5} & \textbf{-5.5} & \textcolor{darkgreen}{\textbf{+5.6}}  & \textcolor{darkgreen}{\textbf{+6.0}}  \\
Crop  blur only     & 48.8  & -30.3               & 67.5  & -13.7             & 68.4  & -13.0             & \bf 74.9           & \bf -6.1           & \textcolor{darkgreen}{\textbf{+6.5}}  & \textcolor{darkgreen}{\textbf{+6.9}}  \\
Crop flip only      & 47.1  & -32.0               & 67.2  & -14.0             & 67.7  & -13.7             & \textbf{74.2} & \textbf{-6.8} & \textcolor{darkgreen}{\textbf{+6.5}}  & \textcolor{darkgreen}{\textbf{+6.9}}  \\
Crop only           & 46.9  & -32.2               & 66.7  & -14.5             & 66.9  & -14.5             & \textbf{74.0} & \textbf{-7.0} & \textcolor{darkgreen}{\textbf{+7.1}}  & \textcolor{darkgreen}{\textbf{+7.5}}  \\
\bottomrule[1.5pt]
\end{tabular}
}
\end{threeparttable}
\vspace{3pt}
\begin{threeparttable}
\footnotesize{(b) ImageNet-100 \textsc{Top-5} accuracy and its \textsc{Drop} w.r.t.  inclusion of all augmentations.}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{l|cc|cc|cc|cc|cc} 
\toprule[1.5pt]
 Method              & \multicolumn{2}{c|}{SimCLR} & \multicolumn{2}{c|}{MoCo} & \multicolumn{2}{c|}{BYOL} & \multicolumn{2}{c|}{\bf \name (ours)}     & \multicolumn{2}{c}{\bf \textsc{Improvement}}          \\ 
\cmidrule{1-11}
\bf\textsc{Metric}              & \bf\textsc{Top-5} & \bf\textsc{Drop}                & \bf\textsc{Top-5} & \bf\textsc{Drop}              &\bf \textsc{Top-5} &\bf\textsc{Drop}              & \bf\textsc{Top-5}         & \bf\textsc{Drop}          & \bf\textsc{Top-5}          & \bf\textsc{Drop}                    \\ 
\midrule\midrule
Baseline            & 94.2  & /                   & 95.1  & /                 & \bf 95.2  & /                 & 95.0          & /             & \textcolor{lightblue}{\textbf{-0.2}}  & /                       \\ 
%\cmidrule{1-2}\cline{3-3}\cmidrule{4-4}\cline{5-5}\cmidrule{6-6}\cline{7-8}\cmidrule{9-10}\cline{11-11}
\midrule
Remove flip         & 93.9  & -0.3                & 94.9  & -0.2              & \bf 95.0  & -0.2              &   94.7        & -0.3          & \textcolor{lightblue}{\textbf{-0.2}}  & \textcolor{darkgreen}{\textbf{+0.0}}           \\
Remove blur         & 92.6  & -1.6                & 94.7  & -0.4              & 94.7  & -0.5              & \textbf{94.7} & \textbf{-0.3} & \textcolor{darkgreen}{\textbf{+0.0}} & \textcolor{darkgreen}{\textbf{+0.1}}  \\
Crop  color only    & 92.1  & -2.1                & 94.4  & -0.7              & 94.3  & -0.9              & \bf 94.5           & \bf-0.5           & \textcolor{darkgreen}{\textbf{+0.1}}  & \textcolor{darkgreen}{\textbf{+0.2}}  \\
%Remove color jitter & 89.4  & -4.7                & 93.9  & -1.2             & \bf 94.7  & -0.5              & 94.2           & -0.9           & \bf\textcolor{lightblue}{{-0.5}}  & \textcolor{lightblue}{\textbf{-0.4}}  \\
%Remove grayscale    & 88.7  & -5.5                & 92.6  & -2.5             & 93.2  & -2.0              & \bf 93.7           & \bf -1.3           & \textcolor{darkgreen}{\textbf{+0.5}}  & \textcolor{darkgreen}{\textbf{+0.7}}  \\
Remove color distort.        & 74.7  & -19.5               & 88.9  & -6.2             & 89.5  & -5.7             & \textbf{93.2} & \textbf{-1.8} & \textcolor{darkgreen}{\textbf{+3.7}}  & \textcolor{darkgreen}{\textbf{+3.9}}  \\
Crop  blur only     & 73.0  & -21.2               & 88.7  & -6.4             & 89.0  & -6.2             & \textbf{92.9}           & \textbf{-2.1}           & \textcolor{darkgreen}{\textbf{+3.9}}  & \textcolor{darkgreen}{\textbf{+4.1}}  \\
Crop flip only      & 71.6  & -22.6               & 88.3  & -6.8             & 88.7  & -6.5             & \textbf{92.7} & \textbf{-2.3} & \textcolor{darkgreen}{\textbf{+4.0}}  & \textcolor{darkgreen}{\textbf{+4.2}}  \\
Crop only           & 71.4  & -22.8               & 88.0  & -7.1             & 88.2  & -7.0             & \textbf{92.5} & \textbf{-2.5} & \textcolor{darkgreen}{\textbf{+4.3}}  & \textcolor{darkgreen}{\textbf{+4.5}}  \\
\bottomrule[1.5pt]
\end{tabular}
}
\end{threeparttable}

\vspace{-15pt}
\end{table*}


\begin{table*}[t]
\centering
\vspace{-2pt}
\caption{\footnotesize{Performance on MPII for the downstream task of human pose estimation. $\uparrow$ indicates the larger the value, the better the performance. Note that the results here are for 2D pose estimation from images, whereas RF-based pose estimation is in 3D. So the evaluation metrics are different.}}
\label{tab:result-pose}
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c|c} 
\toprule[1.5pt]
\multicolumn{2}{c|}{\textsc{Metric}} & Head$^\uparrow$ & Shoulder$^\uparrow$ & Elbow$^\uparrow$ & Wrist$^\uparrow$ & Hip$^\uparrow$ & Knee$^\uparrow$ & Ankle$^\uparrow$ & PCKh$^\uparrow$ \\ 
\midrule
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fixed}\\\textsc{feature}\\\textsc{extractor} \end{tabular}} 
%&Random init & 30.3 & 31.4 & 20.2 & 13.8 & 25.8 & 18.1 & 17.5 & 23.9 \\

&SimCLR & 78.4 & 74.6 & 56.7 & 45.2 & 61.8 & 51.3 & 47.1 & 60.8 \\
&MoCo & 79.2 & 75.1 & 57.4 & 45.9 & 62.4 & 52.0 & 47.6 & 61.4 \\

&CPC & 78.0 & 74.3 & 56.0 & 44.8 & 61.2 & 51.4 & 46.5 & 60.3 \\
&BYOL & 79.1 & 75.0 & 57.1 & 46.0 & 62.4 & 52.2 & 47.7 & 61.4 \\
%&Inpainting  & 83.4 & 75.2 & 53.6 & 44.4 & 56.4 & 44.3 & 45.7 & 59.0  \\ 
%Recontruction   & 15.3  & 65.0 \\   
\cmidrule{2-10}
&\bf \name~(ours)                                                                                      & \bf 85.7 & \bf 78.8 & \bf 61.7 & \bf 51.3 & \bf 64.4 & \bf 55.6 & \bf 49.2 & \bf 65.1                                                                                            \\ 
&\bf \textsc{Improvements}                                                                                      
& \bf \textcolor{darkgreen}{\textbf{+6.5}}
& \bf \textcolor{darkgreen}{\textbf{+3.7}} 
& \bf \textcolor{darkgreen}{\textbf{+4.3}} 
& \bf \textcolor{darkgreen}{\textbf{+5.3}} 
& \bf \textcolor{darkgreen}{\textbf{+2.0}} 
& \bf \textcolor{darkgreen}{\textbf{+3.4}} 
& \bf \textcolor{darkgreen}{\textbf{+1.5}}
& \bf \textcolor{darkgreen}{\textbf{+3.7}}                                                                                          \\ 
%\hhline{=-==}
\midrule
\midrule
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fine-}\\\textsc{tuning} \end{tabular}} 
& SimCLR & 96.2 & 94.7 & 87.3 & 81.2 & 87.5 & 81.0 & 77.2 & 87.1 \\
& MoCo & 95.9 & 94.7 & 87.5 & 81.6 & 87.4 & 81.7 & 76.9 & 87.2 \\
& CPC & 96.0 & 94.5 & 87.0 & 81.1 & 87.3 & 80.8 & 77.0 & 87.0 \\
& BYOL & 96.2 & 94.8 & 87.5 & 81.4 & 87.6 & 81.5 & 77.0 & 87.2 \\
%&Inpainting & 96.3 & \bf 95.2 & 87.9 & 82.1 & 87.8 & 82.5 & 77.6 & 87.7 \\ 
\cmidrule{2-10}
&\bf \name~(ours)                                                                                     & \bf 96.3 & \bf 94.9 & \bf 88.1 & \bf 82.3 & \bf 87.9 & \bf 82.8 & \bf 77.8 & \bf 87.8                                                                                                                                                                        \\
&\bf \textsc{Improvements}                                                                                      
& \bf \textcolor{darkgreen}{\textbf{+0.1}} 
& \bf \textcolor{darkgreen}{\textbf{+0.1}}  
& \bf \textcolor{darkgreen}{\textbf{+0.6}} 
& \bf \textcolor{darkgreen}{\textbf{+0.7}}
& \bf \textcolor{darkgreen}{\textbf{+0.3}} 
& \bf \textcolor{darkgreen}{\textbf{+1.1}} 
& \bf \textcolor{darkgreen}{\textbf{+0.6}} 
& \bf \textcolor{darkgreen}{\textbf{+0.6}}                                                                                            \\ 

\midrule
\midrule
\multicolumn{2}{c|}{\textsc{Supervised}}     & 96.3 & 95.1 & 87.9 & 82.2 & 87.8 & 82.7 & 77.8 & 87.7\\

\bottomrule[1.5pt]
\end{tabular}}
\end{threeparttable}
\vspace{-15pt}
\end{table*}


\begin{table*}
\begin{tabular}{cc}
%\end{tabular}

\begin{minipage}{.52\linewidth}
\centering
\caption{\footnotesize{Performance on FairFace with different unsupervised learning methods. The models are evaluated on downstream tasks of age, gender and ethnicity classification.}}
\label{tab:result-face}
\begin{threeparttable}
\resizebox{.98\textwidth}{!}{
\begin{tabular}{c|c|c|c|c} 
%\hline
\toprule[1.5pt]
\multicolumn{2}{c|}{\textsc{Metric}}                                                                                  & \begin{tabular}[c]{@{}c@{}}\textsc{Age cls} \\ \textsc{Acc.} (\%) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textsc{Gender cls} \\ \textsc{Acc.} (\%) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textsc{Ethn. cls} \\ \textsc{Acc.} (\%) \end{tabular} \\ 
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fixed}\\\textsc{feature}\\\textsc{extractor} \end{tabular}} &SimCLR                   & 43.9  & 78.1  & 61.7                                                                  \\
&MoCo                      & 44.5  & 78.6  & 61.9                                                                  \\
&CPC                                                                                                         & 43.5  & 76.2  & 61.0                                                                  \\ 
&BYOL & 44.3  & 78.6  & \textbf{62.3}  \\
%Recontruction   & 15.3  & 65.0 \\
%&Inpainting                                                                                                          & 15.3                                                                 & 65.0\\      
\cmidrule{2-5}
&\bf{\name~(ours)}  & \bf{50.0}  & \bf{87.2}  & 61.2     \\ 
&\bf \textsc{Improvement}                                                                                      & \bf \textcolor{darkgreen}{\textbf{+5.7}}  & \textcolor{darkgreen}{\textbf{+8.6}}  & \textcolor{lightblue}{\textbf{-1.1}} \\ 
%\hhline{=-==}
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fine-}\\\textsc{tuning} \end{tabular}}
& SimCLR  &54.3 & 91.1 & 69.1   \\
& MoCo & 54.7 & 91.3 & 69.2  \\
&CPC  & 54.2 & 91.0 & 68.8    \\ 
%&Inpainting                                                                                                          & 7.1                                                                   & 45.5                                                                  \\ 
&BYOL & 54.6 &91.5 & \textbf{69.3} \\
\cmidrule{2-5}
&\bf{\name~(ours)}                                                                                    &  \textbf{55.3}                                                                  &  \textbf{92.3}                 & 69.0                                                 \\ 
&\bf \textsc{Improvement}                                                                                     & \bf \textcolor{darkgreen}{\textbf{+0.6}}      & \bf \textcolor{darkgreen}{\textbf{+0.8}}                                                         & \textcolor{lightblue}{\textbf{-0.3}}                                                             \\ 
\midrule\midrule
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{Age}}                                                                      & 55.5 & 78.8  & 45.1                                                                 \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{gender}}                                                                        & 43.3 & 92.5  & 45.4                                                                 \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{Ethn.}}                                                                & 42.1 & 76.8  & 69.4                                                                \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{All}}                                                                & 54.8 & 91.9  &  68.8                                                                \\
%\hline
\bottomrule[1.5pt]
\end{tabular}
}
\end{threeparttable}
\end{minipage}
&
\begin{minipage}{.44\linewidth}
\centering
%\vspace{7pt}
\caption{\footnotesize{Performance on Colorful-MNIST under different unsupervised methods. The models are evaluated on the downstream tasks of digit classification and background object classification.}}
\label{tab:result-toy}
\begin{threeparttable}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{c|c|c|c} 
%\hline
\toprule[1.5pt]
\multicolumn{2}{c|}{\textsc{Metric}}                                                                                  & \begin{tabular}[c]{@{}c@{}}\textsc{Digit cls} \\ \textsc{Acc.} (\%) \end{tabular} & \begin{tabular}[c]{@{}c@{}}\textsc{Bkgd cls} \\ \textsc{Acc.} (\%) \end{tabular}  \\ 
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fixed}\\\textsc{feature}\\\textsc{extractor} \end{tabular}} &SimCLR                    & 14.9                                                                  & 47.3                                                                  \\
&MoCo                                                                                                         & 15.7                                                                  & 48.5                                                                  \\
&CPC                                                                                                          & 15.8                                                                  & 35.2                                                                  \\ 
&BYOL & 15.5 & \textbf{49.0} \\
%Recontruction   & 15.3  & 65.0 \\
%&Inpainting                                                                                                          & 15.3                                                                 & 65.0\\      
\cmidrule{2-4}
&\bf{\name~(ours)}                                                                                      & \bf 88.3                                                                  & 46.5                                                                  \\ 
&\bf \textsc{Improvement}                                                                                      & \bf \textcolor{darkgreen}{\textbf{+72.5}}                                                                & \textcolor{lightblue}{\textbf{-2.5}} \\ 
%\hhline{=-==}
\midrule\midrule
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}\textsc{Fine-}\\\textsc{tuning} \end{tabular}} & SimCLR                               & 92.4                                                                   & 54.8                                                                  \\
& MoCo                                                                                                         & 92.7                                                                   & 54.9                                                                  \\
&CPC                                                                                                      & 92.3                                                                   & 54.7                                                                  \\ 
%&Inpainting                                                                                                          & 7.1                                                                   & 45.5                                                                  \\ 
&BYOL & 92.7 & \textbf{54.9} \\
\cmidrule{2-4}
&\bf{\name~(ours)}                                                                                    & \bf 93.3                                                                   & 54.7                                                                  \\ 
&\bf \textsc{Improvement}                                                                                     & \bf \textcolor{darkgreen}{\textbf{+0.6}}                                                               & \textcolor{lightblue}{\textbf{-0.2}}                                                             \\ 
\midrule\midrule
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{digit}}                                                                      & 96.1                                                                   & 11.4                                                                  \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{bkgd}}                                                                       & 12.9                                                                  & 56.7                                                                  \\
\multicolumn{2}{c|}{\textsc{Supervised} on \textsc{digit} \&  \textsc{bkgd}}                                                                & 93.0                                                                   & 54.5                                                                  \\
%\hline
\bottomrule[1.5pt]
\end{tabular}
}
\end{threeparttable}

%\end{subtable}
%\hfill

%\begin{subtable}
\end{minipage}

\end{tabular}

\vspace{-14pt}
\end{table*}
\subsection{RGB Results}
\label{sec:rgb}

We report the main results for all RGB datasets. The experiment setup, training details and hyper-parameter settings are provided in the appendix along with additional results. 

\textbf{ImageNet-100.} Table \ref{tab:imgnet-100} compares \name\ with the contrastive learning baselines on the task of object classification under different data augmentations. Here, we compare with SimCLR, MoCo, and BYOL since they use the same set of data augmentations. The results show that with fewer data augmentations, the accuracy of the contrastive learning baselines drops quickly due to shortcuts. For example, removing the color distortion augmentation significantly degrades the performance of the baseline approaches, as color distribution is known to be a strong shortcut of contrastive learning. In contrast, \name\ is significantly more robust. For example, with only random cropping, \name's Top-1 accuracy drops by only 7.0 whereas the Top-1 accuracy of SimCLR drops by 32.2 and the Top-1 accuracy of  MoCo and BYOL drops by 14.5. 
 



%It is known that shortcuts such as color distribution can be harmful to the performance of contrastive learning. As a result, previous works use strong augmentations to remove such shortcuts. On the other hand, \name~is much more robust to the choice of image augmentation. In Table \ref{tab:imgnet-100}, we show that the performance of \name~is much less affected than the performance of contrastive baselines when removing color distortion from the set of image augmentations. When image augmentations are reduced to mere random crops, \name~still displays good performance (the accuracy drop is only -7.0) while the performance of all other contrastive baselines drops significantly. This demonstrate that \name~can learn good representations even in the presence of shortcut such as color distribution.

\textbf{MPII.} We use \name\ and the contrastive learning baselines to learn representations from MPII, and evaluate them on the task of pose estimation. Table \ref{tab:result-pose} shows that \name\ improves the average PCKh (the standard metric for pose estimation) over the strongest contrastive baseline by 3.7 and achieves even higher gains on important keypoints such as Head and Wrist. This is because contrastive learning is likely to focus on shortcuts irrelevant to the downstream task, such as clothes and appearances.


\textbf{FairFace.}  Table \ref{tab:result-face} compares the contrastive learning baselines to \name~on the task of face-attribute classification.  The results show how contrastive learning struggles with multi-attribute classification. Specifically, the performance of the contrastive learning baselines on ethnicity classification is close to supervised learning of that attribute (62\% vs. 69\%), However, their results on age and gender classifications are significantly worse than supervised learning of those attributes (44\% and 78\% vs. 54\% and 91\%). This indicates that ethnicity acts as a shortcut for contrastive learning. This shortcut is partial since there are dependencies in how ethnicity manifests itself across age and gender. In contrast, \name\ is much more robust to such shortcuts, and its performance results on age and gender classifications are much closer to those of fully-supervised classification of those attributes. 


%The results show that \name's performances on age and gender are significantly better than all contrastive baselines. The best baseline's performance on age and gender are similar to that of supervised learning on ethnicity label alone ($\sim$44\% and $\sim$79\% accuracy, respectively). This is possibly because the shortcut for contrastive learning is more related to the ethnicity than to age and gender. \name\ improves over baselines on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%).  This further demonstrates \name's ability to preserve useful information  that could be ignored by contrastive learning in multi-attribute classification tasks. 

\textbf{Colorful-MNIST.}  We use this dataset to further investigate how contrastive learning performs on multi-attribute classification. Recall that each image in this dataset contains 
a digit from MNIST on a randomly selected background object from the STL-10. We investigate whether the learned representation supports both  digit and background classifications.  Table \ref{tab:result-toy} shows that the contrastive learning baselines learn only the task of background classification, and fail to learn a representation relevant to digit classification.  This shows that information related to the background act as a shortcut preventing contrastive learning from capturing digit-relevant features. Note that the performance gap on digit classification between contrastive learning and supervised learning is very large (the accuracy is 15\% vs. 93\%). This is much larger than the gap we saw on FairFace because the information related to digit and background are totally independent, whereas features related to ethnicity, age, and gender have a significant overlap. 
In contrast, the representation learned by \name\ achieves very good accuracy on both background and digit classifications. 


Figure~\ref{fig:feat_vis} provides a t-SNE visualization \cite{van2008visualizing} of the learned features for SimCLR and \name. The figure shows how contrastive and reconstructive learnings complement each other. Comparing Figures~\ref{fig:feat_vis}(c) and~\ref{fig:feat_vis}(d) reveals that \name's reconstructive branch allows it to capture information about digits that is lost in SimCLR. However, without \name's contrastive branch, images of the same digit would not be cluster together as they appear in Figure~\ref{fig:feat_vis}(d).

\begin{figure*}[h]
\begin{center}
\vspace{-10pt}
\begin{tabular}{ccccc}
\includegraphics[width=0.23\linewidth]{tsne/cl_bg} & \hspace*{-0.2in}
\includegraphics[width=0.23\linewidth]{tsne/rcl_bg}  & \hspace*{-0.06in}
\tikz{\draw[-, gray, densely dashed, thick](0,-1.05) -- (0,1.05);}
&
\hspace*{-0.06in}
\includegraphics[width=0.23\linewidth]{tsne/cl_digit}  & \hspace*{-0.18in}
\includegraphics[width=0.23\linewidth]{tsne/rcl_digit} 
\\
{\footnotesize (a) SimCLR (Background)} & \hspace*{-0.2in} {\footnotesize (b) {\name} (Background)} & & \hspace*{-0.06in} {\footnotesize (c) SimCLR (Digit)} & \hspace*{-0.18in} {\footnotesize (d) {\name} (Digit)}
\end{tabular}
\vspace{-12pt}
\end{center}
\caption{\footnotesize{Visualization of latent features learned using different approaches on Colorful-MNIST dataset. The color of the left two figures corresponds to background object labels, and the color of the right two figures corresponds to the digit label.}}\label{fig:feat_vis}
\vspace{-10pt}
\end{figure*}

%To better understand the latent features learned using different approaches, we visualize the t-SNE projection of features learned using SimCLR and \name~on the Colorful-MNIST dataset. To visualize the background clusters, we select a subset of the dataset with the same background label and different digit labels; To visualize the digit clusters, we select a subset of the dataset with the same background label and different digit labels. The color of each point corresponds to its ground-truth labels. Specifically, we can see in the right two columns that the features learned with SimCLR do not have clear clustering with regard to digit labels. In contrast, \name~forces the features to have separations with respect to both background object and digit labels. 

%This result shows the complementary role of contrastive branch and reconstructive branch in \name~. The reconstructive branch of \name~forces the features to retain as much information in the input as possible. Therefore, the reconstructive branch can regularize the behavior of the contrastive branch so that the information about the digit will not be discarded. On the other hand, the contrastive branch is crucial to boost the performance of \name~, because it forces the learned representation to have the "contrastive" property, which makes it easy for a simple classifier to slice the embedding space to satisfy a desired task (the appendix includes a detailed comparisons between reconstructive learning and \name).

%We first study the representation quality learned using contrastive learning and show the performance on downstream tasks.As shown in Table \ref{tab:result-toy}, if we only train the network on one of the factors in a supervised way, the feature cannot be used to classify the other task. If the positive samples share only one type of semantics, the standard contrastive learning approach (SimCLR and MoCo) can learn a good representation for the shared type of semantics and achieve similar performance as supervised training while totally fail on the other one. However, if both semantics are shared between positive samples, only one of them (the background) will be learned and the performance is quite similar to contrastive learning on positive samples that only share the same background. This shows that when two types of independent semantics are presented in the input, contrastive learning will tend to learn only one of them (the shortcut) and ignore the other one.

%On the other hand, representation learning using only the missing patches reconstruction task can learn both semantics because the representation should contain enough information to reconstruct both digit and background. However, the learned representation's quality is not as good as that learned using contrastive learning. This is because the reconstruction task will tend to learn low-level features to recover missing pixels instead of high-level representation that are linearly separable.

%The combination of contrastive learning and the missing patches reconstruction task (\name) combines the advantages of both methods: it can learn representation for both semantics with high qualities. Unlike all traditional contrastive learning methods which only get near random results on digits classification ($\sim$90\% error rate), \name~can achieve 11.7\% error rate on digit classification which is quite close to supervised learning on both factors (7.0\%), while keeps performing well on background classification task and achieve comparable results as contrastive learning baselines. This shows that our method's effectiveness in extracting representation that is of high quality on all semantics shared between positive samples.
%\red{This is important in tasks where positive samples share not only semantics we care but also other potential shortcut semantics. For example in RF-based human sensing, RF signals contain information related to both human and background environments. We do not want expose our model to the risk of losing the information about human during the unsupervised learning. }


%\subsection{Face Attribute Classification}
%In this section, we evaluate \name~on FairFace \cite{karkkainen2019fairface}, a real world human face attribute dataset, where each image contains multiple semantics including gender, age, and ethnicity, as shown in Figure~\ref{fig:fairface}.
%
% %One critical property of FairFace is that each face contains multiple semantics including gender, age, and ethnicity. The different semantics require the model to learn different types of features. For example, to better determine the age of a person, the network may need to look at wrinkles, while this feature can be useless when determining a person's gender, where the length and texture of hair serve as important features.
%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{pos-neg-face}
%\end{center}
%\caption{Illustration of FairFace dataset. The positive pairs are from random cropping and random color jittering on an image twice. The negative pairs are sampled within batch.}\label{fig:fairface}
%\vskip -0.1in
%\end{figure}
%
%
%\subsubsection{Experiment Setup}
%\noindent\textbf{Reconstructive Setting.}
%We use the strategy in \cite{pathak2016context} to mask out  $3$ to $5$ rectangles with a random sidesize between $7$ to $12$ pixels at random locations in the image. We fill the masked rectangles with the mean pixel value.
%
%\noindent\textbf{Contrastive Setting.}
%For contrastive learning, we follow the strategy in \cite{chen2020simple} to sample positive and negative pairs. We apply random cropping and random color jittering on an image twice to generate positive pairs. The negative pairs are sampled within batch. 
%%Typical data samples are shown in Figure \ref{fig:fairface}.
%
%\noindent\textbf{Network Structure.}
%We use a standard ResNet-18 for the encoder network $E$. The decoder network $D$ is a symmetric deconvolutional network. The projection head $H$ for contrastive learning is a 2-layer non-linear head which embed the feature into a 128-dimensional unit sphere.
%
%\noindent\textbf{Evaluation Metric.}
%We evaluate the learned representations on three downstream tasks: age, gender and ethnicity classification. 
%For the training of the downstream tasks, we freeze the encoder and train a linear layer for each task to classify the features. For the supervised baselines, supervised (a), (g) and (e) are trained on the single task of age, gender and ethnicity, respectively, while supervised (all) is jointly trained on all the three tasks.
%
%\noindent\textbf{Baselines.}
%We compare IPCL with SimCLR. For SimCLR, we use the same sampling strategy and network structure as our \name. We also fine-tune the hyper-parameters of SimCLR to achieve its best performance.
%
%\subsubsection{Results}
%
%Table \ref{tab:result-face} compares the performance of state-of-the-art contrastive learning (SimCLR) and \name~on the FairFace dataset.  
%As shown by the supervised baselines, the three tasks share some common features since network trained on one of the task can also be used to classify other tasks with reasonable accuracy. However, each task also has its unique features since there are still big performance gaps between network trained on the specific task of interest and networks trained on the other two tasks. The table also shows that \name's performances on age and gender are significantly better than SimCLR. In fact, SimCLR's performance on age and gender are similar to that of supervised learning on ethnicity alone ($\sim$56\% and $\sim$21\% error rate, respectively).  \name\ improves over SimCLR's performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance to SimCLR on ethnicity classification (38.8\% vs. 37.7\%). This further demonstrates \name's ability to preserve useful information  that could be ignored by contrastive learning. 
% 
% 
%
%\begin{table}[h]
%\centering
%\begin{tabular}{l |@{\hspace{0.1cm}} c@{\hspace{0.1cm}} c @{\hspace{0.1cm}}c @{\hspace{0.1cm}}c}\hline
% Method & \begin{tabular}{@{}c@{}}age cls. \\ error rate (\%)\end{tabular}  & \begin{tabular}{@{}c@{}}gender cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}ethnicity cls. \\ error rate (\%)\end{tabular} \\
%\hline
%\multirow{ 1}{*}{SimCLR}  & 55.7  & 21.4  & 37.7  \\\hline
%
%\multirow{ 1}{*}{\textbf{\name~(ours)}}  & 50.0  & 12.8  & 38.8\\\hline
%
%\multirow{ 1}{*}{Supervised (a)}  & 44.5 & 21.3  & 54.9 \\
%
%\multirow{ 1}{*}{Supervised (g)}  & 56.7 & 7.5  & 54.6  \\
%
%\multirow{ 1}{*}{Supervised (e)}  & 57.9 & 23.2  & 28.6  \\
%
%\multirow{ 1}{*}{Supervised (all)}  & 45.2 & 8.1  &  29.2 \\
%
%\hline
%\end{tabular}
%\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of age, gender and ethnicity classification.}}
%\label{tab:result-face}
%\end{table}


==> source/experiment-rgb.tex <==
\section{Experiments on RGB datasets}
\subsection{\name~on Visual Representation}
\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{model-toy}
\end{center}
\caption{\name~on RGB dataset. For prediction branch, images are spatially masked and an encoder-decoder architecture is adopted to predict masked regions. For contrastive branch, positive samples are generated with different transformations: $\tau_1$ and $\tau_2$, and a Non-linear MLP head is used to generate normalized features for contrastive loss}\label{fig:model-toy}
\end{figure}
In this section, we apply \name~on RGB modality. As shown in Figure \ref{model-toy}, for the predictive branch, we follow the setup in \ref{sec:xxx} to randomly cropped out several patches with random size at random location from the input images. The cropped region is then filled with the mean pixel value of the dataset. The goal of the predictive branch is to recover the original images from the patched images. For the contrastive branch, we follow the setting in SimCLR \cite{xxx} where random augmentations $\tau$ are added to each image. The two augmented images from the same input image serve as positive pair, and those images from different input images serve as negative pair.

During the unsupervised learning phase, we employ a standard CNN encoder to encode images. For contrastive learning, a non-linear projection head is added on top of the encoded latent features $F$ to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For predictive learning, a decoder is added on $F$ to reconstruct the original image, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed image and the ground truth image with out patching. For \name, we first train the predictive branch alone to let the network learn coarse features about each task. Then we combine these two losses together to be $\lambda_1\cdot l_P + \lambda_2\cdot l_C$ to learn fine-grained features for each task. We set $\lambda_1 = 20$ and $\lambda_2 = 1$ in our experiments.

\subsection{Toy Dataset: Colorful-MNIST}
Directly analyzing natural images can be challenging as it is hard to create orthogonal semantics that can be easily disentangled and manipulated. Therefore, we first use a toy dataset as a starting point to understand the behavior of contrastive training on multiple semantics. Similar to \cite{xxx}, we construct Colorful-MNIST dataset by putting a digit from MNIST on top of an image randomly selected from STL-10 dataset. Specifically, we first select a random image from STL-10 dataset [11] and randomly crop a patch from this image as background. Then we randomly select a digit from MNIST and put it at a random position of the background. As a result, the Colorful-MNIST dataset consist of two semantics with quite different features in each frame: the class of the digit and the and the class of background image.
\\

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{toy-dataset}
\end{center}
\caption{Illustration of our Colorful-MNIST dataset. During contrastive training on one of the semantic, this semantic of anchor and the positive sample will be the same, while the other semantic will be different (left and right). During contrastive training on both semantics, both digit and background of anchor and positive sample are the same (middle).}\label{fig:toy-dataset}
\end{figure}

\begin{table}[t]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & \begin{tabular}{@{}c@{}}shared factor or \\ supervised label\end{tabular}  & \begin{tabular}{@{}c@{}}digit cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}bkgd cls. \\ error rate (\%)\end{tabular} \\
\hline
\multirow{ 3}{*}{SimCLR}  & digit  & 12.1  & 86.0  \\
 & bkgd   & 87.8  & 51.9  \\
 & digit \& bkgd & 85.1  & 51.5 \\ 
\hline  
  

\multirow{ 3}{*}{MoCo}  & digit  & 14.4  & 86.5  \\
 & bkgd  & 85.6 & 54.1 \\
 & digit \& bkgd & 84.3 & 53.7 \\ 
\hline     
\multirow{ 1}{*}{CPC}  & - & 84.2  & 64.8 \\
\hline
\multirow{ 1}{*}{predict}   & - & 15.3  & 65.0 \\
\hline
\multirow{ 1}{*}{\textbf{PreCLR}}  & digit \& bkgd    & 11.7  & 54.0\\
\hline
\hline

\multirow{ 3}{*}{Supervised}  & digit & 3.9  & 88.6  \\
 & bkgd   & 87.1  & 43.3 \\
 & digit \& bkgd & 7.0  & 45.5 \\ 

\hline
\end{tabular}
\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of digit classification and background classification.}}
\label{tab:result-toy}
\end{table}

\subsubsection{Experiment Setup}
We follow the setup in \ref{sec:xxx} for contrastive training. Examples of construct positive and negative samples are shown in Figure \ref{fig:toy-dataset}. For contrastive training on digit, we construct positive sample to have the same digit as the anchor at a random location at a random background. For contrastive training on background, we construct positive samples to have random digit at a random location on a random patch of the same background as the anchor. For contrastive training on both digit and background, we construct positive sample to have the same digit as the anchor at a random location on a random patch of the same background as the anchor. The negative samples are sampled within batch. 

After the pre-training phase, to evaluate what semantics are encoded in the latent features, we consider two different downstream classification tasks for an image: predict the digit class and predict the background class. In this downstream training phase, we freeze the backbone encoder CNN as feature extractor and train a single linear layer for each task to classify the features. We also provide a supervised baseline on the same data for comparison.


\subsubsection{Results}
We first study the representation quality learnt using contrastive learning and show the performance on downstream tasks in Table \ref{tab:result-toy}. As shown in Table \ref{tab:result-toy}, if the positive samples share only one semantics, the contrastive learning can learn a good representation for the shared semantics while totally failing on the other semantics. This shows that the representation of one of these two semantics cannot help to classify the second semantics. More interestingly, if both semantics are shared between positive samples, only one of them (the background) will be learnt.
On the other hand, predictive unsupervised learning can learn both semantics because the representation should contain enough information to reconstruct the original image. However, the learnt representation's quality is not as good as that learnt using contrastive learning. 

The combination of contrastive and predictive learning combines the advantages of both world: it can learn representation for both semantics and the representation for each of them is of good quality. This shows that our method's effectiveness on extracting representation that is of high quality on all semantics shared between positive samples. This is quite important in tasks where positive samples share multiple semantics and we only care some certain ones of them, such as RF-based human sensing, since RF signals contain information related to both human and background, and we only care about ones related to human.


\subsection{FairFace}

We then evaluate \name~on a real world human face recognition dataset, FairFace \cite{xxx}. One important feature of such dataset is that each face contains multiple types of semantics including gender, age, and ethnicity, each of them requires the network to learn unique features. For example, to better determine the age of the person, the network may need to look at the wrinkles, while this feature can be useless when determine the person's gender where the length and texture of hair serves an important feature. 


\subsubsection{Experiment Setup}
We follow similar strategy as \cite{xxx} to sample positive and negative pairs for contrastive learning. We apply random cropping and random color jittering on an image twice to generate positive pairs. The negative pairs are sampled within batch. After the pre-training phase, we evaluate the learnt representation on three downstream tasks: age, gender and ethnicity, to see which semantics the representation captures best. In this downstream training phase, we freeze the encoder CNN and train a single linear layer for each task to classify the features. For the supervised baselines, supervised (a), (g) and (e) are trained on single task of age, gender and ethnicity, respectively, while supervised (all) are joint trained on all the three tasks.

\subsubsection{Results}
\begin{table}[t]
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & \begin{tabular}{@{}c@{}}age cls. \\ error rate (\%)\end{tabular}  & \begin{tabular}{@{}c@{}}gender cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}ethnicity cls. \\ error rate (\%)\end{tabular} \\
\hline
\multirow{ 1}{*}{SimCLR}  & 55.7  & 21.4  & 44.7  \\

\multirow{ 1}{*}{\textbf{PreCLR}}  & 50.5  & 14.5  & 46.1\\

\multirow{ 1}{*}{Supervised (a)}  & 44.5 & 21.3  & 59.9 \\

\multirow{ 1}{*}{Supervised (g)}  & 56.7 & 7.5  & 59.6  \\

\multirow{ 1}{*}{Supervised (e)}  & 57.9 & 23.2  & 33.6  \\

\multirow{ 1}{*}{Supervised (all)}  & 45.2 & 8.1  &  34.2 \\

\hline
\end{tabular}
\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of age, gender and ethnicity classification.}}
\label{tab:result-face}
\end{table}


In Table \ref{tab:result-face} we show the performance of SimCLR and \name~on FairFace dataset. As shown by the supervised baseline, the three tasks share some common feature since network trained on one of the task can also be used to classify other tasks. However, each task also has its unique features since there are still big performance gaps on each task between network trained on other task and network trained on the exact task. As shown in the table, the SimCLR's performance on age and gender are similar to that of supervised learning on ethnicity, while the performance on ethnicity is far beyond the performance of supervised learning on age and gender. This shows that the SimCLR tends to learn task-specific features related to ethnicity and ignore those task-specific features about age and gender. On the other hand, \name~can learn task-specific features about each task. It can achieve much better performance on age and gender classification, while keeps comparable performance as SimCLR on ethnicity classification. This further demonstrates \name's advantage on preserving useful information in the input and avoid learning only one types of 'shortcut' semantics.

==> source/experiment-toy.tex <==
\section{Toy Example: Colorful-MNIST Dataset}
Directly analyzing natural images can be challenging as it is hard to create orthogonal semantics that can be easily disentangled and manipulated. Therefore, we first use a toy dataset as a starting point to understand the behavior of contrastive training on orthogonal semantics. Similar to \cite{xxx}, we construct Colorful-MNIST dataset by putting a digit from MNIST on top of an image randomly selected from STL-10 dataset. Specifically, we first select a random image from STL-10 dataset~\cite{xx} and randomly crop a patch from this image as background. Then we randomly select a digit from MNIST and put it at a random position of the background. As a result, the Colorful-MNIST dataset consist of two semantics with quite different features in each frame: the class of the digit and the and the class of background image.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{toy-dataset}
\end{center}
\caption{Illustration of our Colorful-MNIST dataset. During contrastive training on one of the semantic, this semantic of anchor and the positive sample will be the same, while the other semantic will be different (left and right). During contrastive training on both semantics, both digit and background of anchor and positive sample are the same (middle).}\label{fig:toy-dataset}
\end{figure}

% \red{DK COMMENT -- Should have a separate section to explain \name\ for images and reference Figure 3 and another section for explaining the experiment in which we describe the various baselines.}
 
 
\subsection{\name\ for Visual Tasks}
In this section, we explain how to adapt the \name\ framework to image datasets. 
We follow the setup in \ref{sec:xxx} for contrastive training. Examples of constructed positive and negative samples are shown in Figure \ref{fig:toy-dataset}. For contrastive training on digit, we construct positive sample to have the same digit as the anchor at a random location on a random background. For contrastive training on background, we construct positive samples to have random digit at a random location on a random patch of the same background as the anchor. For contrastive training on both digit and background, we construct positive sample to have the same digit as the anchor at a random location on a random patch of the same background as the anchor. The negative samples are other samples in the batch.  For the inpainting task, we follow the setup in \ref{sec:xxx} to randomly crop out several patches with random sizes at random locations from the input images. The cropped region is then filled with the mean pixel value of the dataset.

\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{model-toy}
\end{center}
\caption{\name~on Colorful-MNIST dataset. For prediction branch, images are spatially masked and an encoder-decoder architecture is adopted to predict masked regions. For contrastive branch, positive samples are generated with different transformations: $\tau_1$ and $\tau_2$, and a Non-linear MLP head is used to generate normalized features for contrastive loss}\label{fig:model-toy}
\end{figure}

During the unsupervised learning phase, we employ a 6-layer ConvNet to encode images. For contrastive learning, a non-linear projection head is added on top of it to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For predictive learning, a decoder is added to reconstruct the original image, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed image and the ground truth image without cropping. For \name, we combine these two losses together to be $\lambda_1\cdot l_P + \lambda_2\cdot l_C$. We set $\lambda_1 = 4$ and $\lambda_2 = 1$ in our experiments.

After the pre-training phase, to evaluate what semantics are encoded in the latent features, we consider two different downstream classification tasks for an image: predict the digit class and predict the background class. In this downstream training phase, we freeze the backbone 6-layer ConvNet as feature extractor and train a single linear layer for each task to classify the features. We also provide a supervised baseline on the same data for comparison.

\begin{table}[t]
{\small
\centering
\begin{tabular}{l |@{\hspace{0.2cm}} c c @{\hspace{0.2cm}}c @{\hspace{0.2cm}}c}\hline
 Method & \begin{tabular}{@{}c@{}}shared factor or \\ supervised label\end{tabular}  & \begin{tabular}{@{}c@{}}digit cls. \\ error rate (\%)\end{tabular} & \begin{tabular}{@{}c@{}}bkgd cls. \\ error rate (\%)\end{tabular} \\
\hline
\multirow{ 3}{*}{SimCLR}  & digit  & 12.1  & 86.0  \\
 & bkgd   & 87.8  & 51.9  \\
 & digit \& bkgd & 85.1  & 51.5 \\ 
\hline  
\multirow{ 3}{*}{MoCo}  & digit  & 14.4  & 86.5  \\
 & bkgd  & 85.6 & 54.1 \\
 & digit \& bkgd & 84.3 & 53.7 \\ 
\hline     
\multirow{ 1}{*}{CPC}  & - & 84.2  & 64.8 \\
\hline
\multirow{ 1}{*}{predict}   & - & 15.3  & 65.0 \\
\hline
\multirow{ 1}{*}{\textbf{PreCLR}}  & digit \& bkgd    & 11.7  & 54.0\\
\hline
\hline
\multirow{ 3}{*}{Supervised}  & digit & 3.9  & 88.6  \\
 & bkgd   & 87.1  & 43.3 \\
 & digit \& bkgd & 7.0  & 45.5 \\ 
\hline
\end{tabular}
}
\caption{\footnotesize{We study the representation quality learnt using different methods. We evaluate the learned representation on downstream tasks of digit classification and background classification.}}
\label{tab:result-toy}
\end{table}


\subsection{Results}
We first study the quality of the representation learned using contrastive learning and show the performance on downstream tasks in Table \ref{tab:result-toy}. As shown in Table \ref{tab:result-toy}, if the positive samples share only one type of semantics (either digit or background), contrastive learning learns a good representation for the shared semantics, but the learned representation totally fails on the other semantics. This shows that the representation of one of these two types of semantics cannot help to classify the second type --i.e., the representation is specific to one of the two classification tasks. 
More interestingly, if both semantics are shared between positive samples (i.e., paired positive samples share both the background and digit), only one type of semantics, particularly the background, will be learned. On the other hand, \name\ can learn both semantics because the representation should contain enough information to reconstruct the original image. 
%However, the learned representation's quality is not as good as that learned using contrastive learning. 

The combination of contrastive and predictive learning combines the advantages of both world: it can learn representation for both semantics and the representation for each of them is of good quality. This shows that our method's effectiveness on extracting representation that is of high quality on all semantics shared between positive samples. This is quite important in tasks where positive samples share multiple semantics and we only care some certain ones of them, such as RF-based human sensing, since RF signals contain information related to both human and background, and we only care about ones related to human.


==> source/experiment.tex <==
\vspace{-5pt}
%\section{Evaluation}
%\input{source/experiment-rgb-7}
\input{source/experiment-rf-12}
%\input{source/ablation}


==> source/intro-1.tex <==
\section{Introduction}

Radio Frequency (RF) signals have been demonstrated effective in capturing the human pose, actions, and identifiable information. Further, since RF signals can traverse occlusions and operate in dark settings,  RF-based human sensing models work through walls and in poor lighting conditions.  RF signals are also privacy-preserving because they cannot be easily interpreted by humans. Hence, deploying such systems in people's homes can help monitor elders' health conditions or patients' well-beings without raising privacy concerns. Such characteristics make RF signals an important complement for RGB-based systems in applications like smart homes and health monitoring.

However, training  high performance RF-based human sensing requires a large RF dataset with accurate labels. But since RF signals are not human interpretable, human labelers cannot just look at the signal and label them the same way as they label RGB-based datasets. To label such datasets, one need to collect synchronized data from another modality that can be interpreted by labelers so that they can label RF signals based on the other synchronized modality. Previous works uses a multi-camera system \cite{zhao2018through,zhao2018rf,zhao2019through,li2019making,fan2020learning,fan2020home} or on-body accelerometers \cite{hsu2019enabling,hsu2017zero,fan2020learning} to provide this second modality. However, this necessity for a second synchronized modality severely limits the diversity and size of labeled RF datasets. For example, it is difficult to deploy cameras in people's home to record their daily life, or ask elders to always wear accelerometer at home. As a result, a large portion of RF datasets has no such synchronized modality and becomes unlabeled data. 

Previous works ignores this unlabeled data and only focus on supervised training on the labeled parts of RF datasets. However, those unlabeled RF data are of much larger size and more diversified than those labeled data. If we could use unsupervised learning methods to learn high-quality representations from those large amount of unlabeled RF data, we can significantly improves the performances and generalization ability of current RF-based human sensing systems.

Unsupervised learning approaches on large scale image and video datasets are being developed rapidly. Recent literatures in the vision community have shown that models trained using unsupervised contrastive learning can outperform models trained in a supervised way \cite{chen2020simple,he2020momentum,chen2020improved}. An easy solution to perform unsupervised learning on RF signals is to directly adapt this contrastive training scheme to RF signals. 

However, it is not easy to directly adapt off-the-shelf unsupervised contrastive learning approaches on RGB inputs to RF signals. Just like RGB data, RF signals can contain multiple types of semantics. During contrastive learning, multiple types of semantics shared between the anchor and positive samples can be similar. Some of them are related to human sensing tasks such as the pose or the identity of the person, while others are completely irrelevant types of semantics such as the degree of background noise or the distance of the person to the device. As a result, current unsupervised contrastive learning can easily bias to those irrelevant 'shortcuts' instead of those  types of semantics that are useful for human sensing downstream tasks like pose estimation or re-identification. Traditional contrastive learning methods on RGB data use various data augmentation methods to force the contrastive training to focus on the desired types of semantics. Those augmentations break the irrelevant types of semantics originally shared between positive samples. However, for modality like RF signals, it is hard to find augmentations to eliminate all irrelevant types of  semantics while keep all the useful ones. Moreover, a type of semantics can be irrelevant to one downstream task while important to another. As a result, it is hard to train a network to extract general human-related representations from RF signals using traditional contrastive learning.

In this paper, we aim to design an effective unsupervised learning mechanism to learn high-quality representations containing multiple types of useful semantics from input modalities. We first show that traditional contrastive learning can easily bias to some types of 'shortcut' semantics and ignore semantics that is useful for downstream tasks, especially when no augmentation is applied to the input. To solve this problem, we add another predictive task to the contrastive training scheme. Since predicting the missing patches in the input requires the learnt representation to be able to reconstruct the original input, the representation must contain information about all semantics in the input. The contrastive learning is then used to learn high-quality features for all semantics. Combining this predictive task and contrastive learning together, we propose Predictive-Contrastive Learning (\name), a learning mechanism that is able to learn high-quality representation for all semantics in the input.

We further evaluate \name~on both synthetic dataset and real RF dataset. We first use a synthesized RGB image dataset to show that when anchor and positive samples of contrastive learning share multiple types of semantics, the traditional contrastive learning approaches can be easily biased to one of them while \name~could learn all types of semantics with high quality. Then we evaluate our \name~on image classification dataset and show that \name~can achieve comparable results as state-of-the-art contrastive learning methods under common unsupervised learning setting, and outperforms those methods when limited augmentations are added on the input. Finally, we evaluate our approach on three real-world RF-based human sensing tasks: 3D Pose Estimation, Human action detection and Person Re-Identification. Our experiment results show that \name~can significantly improve the performance of RF-based models on each tasks and outperform the contrastive learning baselines.

To summarize, our paper has the following contributions:
\begin{Itemize}
    \item We are the first to study unsupervised learning approaches on the modality of RF signals, showing the possibility to boost performance for RF-based human sensing systems with unsupervised learning.  
    \item We demonstrates that when anchor and positive samples of contrastive learning shares multiple types of semantics, traditional contrastive learning can easily bias to one of them and completely ignore the others. We further propose a novel approach which combines predictive task and contrastive learning to prevent the network from only learning one types of semantics.
    \item We conducts extensive experiments on both synthetic RGB image dataset, real-world RGB datasets and RF datasets. Our proposed method outperforms traditional contrastive learning methods on all of those datasets, demonstrating the effectiveness of \name~ especially when data augmentation cannot eliminate all types of shortcut semantics. 
\end{Itemize}



==> source/intro-2.tex <==
\section{Introduction}
The area of unsupervised or self-supervised representation learning is growing rapidly~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,hjelm2018learning,gutmann2010noise,ji2019invariant,sohn2016improved,wu2018unsupervised,ye2019unsupervised}.  
It refers to learning useful data representations that capture potential labels of interest, and doing so without human supervision. Contrastive learning is increasingly considered as a standard and highly competitive method for unsupervised representation learning. Features learned with this method have been shown to generalize well to downstream tasks,  and in some cases surpass the performance of supervised models~\cite{oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,henaff2019data}. 
 
Contrastive learning learns representations by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropped and color distorted version of of the anchor image), whereas negative samples come from other samples in the dataset. 
 
Despite its effectiveness, contrastive learning is vulnerable to shortcuts -- i.e., if simple features are contrastive enough to separate positive samples from negative samples, contrastive learning might learn such simple (or simpler) features though they may be irrelevant to the tasks of interest, and ignore other more relevant features. For example, the authors of \cite{chen2020simple} show that color distribution can be a shortcut to distinguish two patches cropped from the same image, from two patches from different images; yet such feature is not very useful for object classification. Past work addresses this problem by adding data augmentations to break the shortcut semantics, so that the network may learn the desired semantics \cite{chen2020simple, he2020momentum,chen2020big,chen2020improved}. 

However, it is not always possible to address shortcuts via data augmentation. First, machine learning tasks are expanding to new modalities, many of which are not directly interpretable by humans such radio signals~\cite{zhao2018through,zhao2018rf,zhao2019through,li2019making,fan2020learning,fan2020home}, or acceleration data~\cite{hsu2019enabling,hsu2017zero,fan2020learning}. Consider for example the task of through-wall pose estimation~\cite{zhao2018through}. This task leverages that radio signals traverse walls and occlusions and reflect off the human body; it designs neural network models that analyze the radio frequency (RF) signals and infer the human pose, even when people are behind a wall. Such task would benefit significantly from unsupervised representation learning given the limited amount of labeled RF signals, and the difficulties of labeling such modality which is not interpretable by human workers~\cite{zhao2018through,zhao2018rf,zhao2019through,li2019making}. However, like RGB data, RF data can have shortcuts that make contrastive learning ineffective (see the results section for empirical validation). But unlike RGB data, it is hard for humans to guess what the shortcuts may be, or how to alter the RF signal to create data augmentations that eliminate the shortcuts, while preserving useful information. 

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{pos-neg}
\end{center}
\caption{Illustrative example, where the input has two types of information: digit and background object, but existing unsupervised contrastive learning methods generate a representation that captures mostly the background object and ignores the digit.}
\label{fig:intro}
\end{figure}

Second, eliminating shortcut features is not always desirable, even for RGB-based tasks. Sometimes the shortcut features are irrelevant to one downstream task but important to another task. For example, the authors of \cite{tian2020makes} highlight the scenario in Figure~\ref{fig:intro}, where each image shows a digit (from MNIST) on a randomly chosen background object (from STL-10).  They show that features related to the background object can create a shortcut that prevents contrastive learning from learning features related to the digit. However, eliminating features about the background object is not desirable since ideally one would like a representation that works for both downstream tasks: digit classification, and background object classification. 

\red{To address the above problems, we propose a new framework that we call information-preserving contrastive learning (IPCL). The key idea underlying IPCL is to learn representations using contrastive and reconstructive learning simultaneously. We use the term reconstructive learning to refer to tasks that force the representation to reconstruct the input, such as impainting, colorization, or autoencoding. Such tasks counter the effect of shortcuts because they force the learned features to summarize and retain all useful information in the input. Once combined with reconstructive learning,  contrastive learning ensures that all useful features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples. Thus, reconstructive learning maximizes the useful information in the representation, whereas contrastive learning orders the information in the embedding space to make it easy for a simple classifier to slice the embedding space to satisfy a desired task. }

%The key idea underlying IPCL is to ensure that even when the data has potential shortcuts, the representation will learn features about all types of semantic information in the data (digit and background object), and contrastive learning will ensure that all of those features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples.  To ensure that these properties are satisfied, IPCL augments contrastive learning with an auxiliary task that uses the learned representation to restore randomly cropped patches in the anchor sample. By doing so, IPCL ensures that the learned representation summarizes all useful information in the input, but also enjoys contrastive properties. 


We apply the IPCL framework to both RGB-based and RF-based tasks, designing neural network models appropriate for those modalities.   We then evaluate IPCL on both RGB and RF datasets. Specifically, we evaluate IPCL on two image classification datasets. The first is the Colorful-MNIST, a synthetic dataset proposed in \cite{tian2020makes} and illustrated in Figure~\ref{fig:intro}. The results show that IPCL outperforms by a high margin state-of-the-art contrastive learning methods like SimCLR, MoCo, and Contrastive Predictive Coding in its ability to learn a representation that works for both digit classification and background object classification. Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

We also evaluate IPCL on three real-world RF-based through-wall human sensing tasks: 3D pose estimation, human action detection, and person re-identification. Our empirical results show that IPCL can consistently improve the performance of RF-based models on each of these tasks, and outperform the contrastive learning baselines. Specifically, \name~achieves 8.6\% relative improvement in keypoint-localization error of 3D pose estimation, 2.7\% relative improvement on action recognition and 3.6\% relative improvement on person ReID at home.

To summarize, our paper has the following contributions:
\begin{Itemize}
    \item We introduce IPCL, a new framework that allows contrastive learning to be effective in the presence of shortcuts. It is particularly suitable for data modalities that are hard to interpret by humans (e.g., RF signals), and for learning representations that preserve information about multiple aspects of the input data, particularly when these aspects are independent (e.g., digit and background object) or share low mutual information. 
    \item  
    We are the first to study unsupervised representation learning from radio signals, demonstrating the possibility of boosting the performance of RF-based human sensing tasks by leveraging unlabeled RF signals. 
    \item We conduct extensive experiments on a synthetic RGB image dataset, a real-world RGB dataset, and RF datasets demonstrating the impact of shortcuts on contrastive learning, and the ability of IPCL to address those problems. 
\end{Itemize}



==> source/intro-3.tex <==
\section{Introduction}
The area of unsupervised or self-supervised representation learning is growing rapidly~\cite{he2020momentum,doersch2015unsupervised,ye2019unsupervised,hjelm2018learning,grill2020bootstrap,bachman2019learning,zhuang2019local,misra2020self,han2020memory}.
%pathak2016context,noroozi2016unsupervised,he2020momentum}. 
%~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,ji2019invariant,sohn2016improved,icmlunsupervised,ye2019unsupervised}.  
It refers to learning data representations that capture potential labels of interest, and doing so without human supervision. Contrastive learning is increasingly considered as a standard and highly competitive method for unsupervised representation learning. Features learned with this method have been shown to generalize well to downstream tasks,  and in some cases surpass the performance of supervised models~\cite{oord2018representation,caron2020unsupervised,tschannen2019mutual,chen2020simple,chen2020big,chen2020improved}. 
 
Contrastive learning learns representations by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. 
 
Despite its effectiveness, contrastive learning is vulnerable to shortcuts -- i.e., if simple features are contrastive enough to separate positive samples from negative samples, contrastive learning might learn such simple (or simpler) features though they may be irrelevant to the tasks of interest, and ignore other more relevant features. For example, the authors of \cite{chen2020simple} show that color distribution can be a shortcut to distinguish patches cropped from the same image, from patches from different images; yet such feature is not very useful for object classification. Past work manually designs data augmentations to break such shortcuts, so that the network may learn the relevant information \cite{he2020momentum,chen2020simple,chen2020big,chen2020improved}. 

However, it is not always possible to address shortcuts via data augmentation. First, machine learning tasks are expanding to new modalities, many of which are not directly interpretable by humans such as radio signals~\cite{zhao2018through,zhao2018rf,zhao2019through,li2019making,fan2020learning,fan2020home}, or acceleration data~\cite{hsu2019enabling,hsu2017zero,fan2020learning}. Consider for example the task of through-wall pose estimation~\cite{zhao2018through}. This task leverages that radio signals traverse walls and occlusions and reflect off the human body; it designs neural network models that analyze the radio frequency (RF) signals and infer the human pose, even when people are behind a wall. Such task would benefit significantly from unsupervised representation learning given the limited amount of labeled RF signals, and the difficulties of labeling such modality which is not interpretable by human workers~\cite{zhao2018through,zhao2018rf,zhao2019through,li2019making}. However, like RGB data, RF data can have shortcuts that make contrastive learning ineffective (see the results section for empirical validation). But unlike RGB data, it is hard for humans to guess what the shortcuts may be, or how to alter the RF signal to create data augmentations that eliminate the shortcuts, while preserving useful information. %\red{And even for RGB data, as shown in Sec. \ref{sec:shortcut}, it can also be hard to reason about what is the actual shortcut.} 

\begin{wrapfigure}{r}{77mm}
\begin{center}
\includegraphics[width=\linewidth]{pos-neg}
\end{center}
\vspace{-15pt}
\caption{\footnotesize{Shortcut Example. The input has two types of information: digit and background object, but existing contrastive learning methods generate a representation that focuses on the background object and ignores the digit.}}
\label{fig:intro}
\vspace{-5pt}
\end{wrapfigure}

Second, eliminating shortcut features is not always desirable, even for RGB-based tasks. Sometimes the shortcut features are irrelevant to one downstream task but important to another task. For example, the authors of \cite{tian2020makes} highlight the scenario in Figure~\ref{fig:intro}, where each image shows a digit (from MNIST) on a randomly chosen background object (from STL-10).  They show that features related to the background object can create a shortcut that prevents contrastive learning from learning features related to the digit. However, eliminating features about the background object is not desirable since ideally one would like a representation that works for both downstream tasks: digit classification, and background object classification. 

To address the above problems, we propose a new framework that we call information-preserving contrastive learning (IPCL). The key idea underlying IPCL is to learn representations using contrastive and reconstructive learning simultaneously. We use the term reconstructive learning to refer to tasks that force the representation to reconstruct the input, such as inpainting, colorization, or autoencoding. Such tasks counter the effect of shortcuts because they force the learned features to both abstract and retain the information in the input. Once combined with reconstructive learning,  contrastive learning ensures that all useful features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples. Thus, reconstructive learning maximizes the useful information in the representation, whereas contrastive learning orders the information in the embedding space to make it easy for a simple classifier to slice the embedding space to satisfy a desired task. 

%The key idea underlying IPCL is to ensure that even when the data has potential shortcuts, the representation will learn features about all types of semantic information in the data (digit and background object), and contrastive learning will ensure that all of those features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples.  To ensure that these properties are satisfied, IPCL augments contrastive learning with an auxiliary task that uses the learned representation to restore randomly cropped patches in the anchor sample. By doing so, IPCL ensures that the learned representation summarizes all useful information in the input, but also enjoys contrastive properties. 


%We apply the IPCL framework to both RGB-based and RF-based tasks, designing neural network models appropriate for those modalities.   

We evaluate IPCL  and compare it with state-of-the-art contrastive learning baselines such as  SimCLR~\cite{chen2020simple}, MoCo~\cite{he2020momentum}, and Contrastive Predictive Coding (CPC)~\cite{henaff2019data}. We summarize our findings for RF and RGB data as follows:

%\begin{Itemize}
%\item 
{\it (a) Results on RF Data:}
We evaluate IPCL on three real-world RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. 
The results show that IPCL outperforms all contrastive learning baselines on all tasks.  In comparison to the best performing contrastive learning baseline, the IPCL representation improves performance by 30.6 mm, 81.4 mAP, and 24.5 mAP on the tasks of pose estimation, action recognition, and person re-id respectively.  
%Further, initializing supervised learning with the IPCL representation improves performance for all three tasks, confirming that self-supervision is beneficial for learning from non-interpretable data. 
Interestingly, the representations learned by the contrastive learning baselines perform worse than random features on pose estimation and action recognition. This shows that contrastive learning converged on a shortcut, and discarded key information necessary for these two  tasks.  


%\item 
{\it (b) Results on RGB Data:}
Since RF signals are hard to interpret, we apply IPCL to RGB data to gain more insight into its working. We evaluate IPCL on the Colorful-MNIST, a synthetic dataset proposed in \cite{tian2020makes} and illustrated in Figure~\ref{fig:intro}. 
%The results show that the IPCL representation is useful for both digit classification and background object classification, whereas that the representations learned by SimCLR, MoCo, and CPC are useful only for background object classification but fail on digit classification. Specifically, 
In comparison to the contrastive learning baselines, the IPCL representation has 72\% lower error on digit classification and comparable performance on background classification.  This shows that IPCL is better at generating representations that can support multiple downstream tasks. 
Even more, we show that increasing the size of the digit (by 10 to 15 pixels) causes the contrastive learning shortcut to move from background to digit, though the semantic information in each image did not change. In all cases, IPCL learns a representation that performs well on both digit and background classifications, whereas the representation learned by contrastive learning is good only for at most one of the two tasks. 

%\red{We also empirically show the complexity of reasoning about shortcuts even in RGB images, and how IPCL overcomes this complexity.}

%Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

%\end{Itemize}

To summarize, our paper has the following contributions:
\begin{Itemize}
\vspace{-8pt}
    \item We introduce IPCL, the first self-supervised learning framework that integrates contrastive and reconstructive learning to automatically avoid shortcuts and provide a representation that supports multiple different downstream tasks. We note that while both contrastive and reconstructive learning existed prior to our work, no past work has discovered their complementary role or proposed to combine them the way we do.     
        \item We empirically show the negative impact shortcuts have on contrastive learning, and how a shortcut can move from one task to another, though the input semantics did not change.  We also show that IPCL addresses these issues.
        \item We demonstrate that \name~outperforms SOTA contrastive learning methods on its ability to avoid shortcuts on multiple benchmarking RGB datasets. We are also the first to study unsupervised representation learning from radio signals, demonstrating the possibility of boosting the performance of RF-based human sensing tasks by leveraging unlabeled RF signals. 
\vspace{-8pt}
\end{Itemize}



==> source/intro-4.tex <==
\section{Introduction}
The area of unsupervised or self-supervised representation learning is growing rapidly~\cite{he2020momentum,doersch2015unsupervised,ye2019unsupervised,hjelm2018learning,grill2020bootstrap,bachman2019learning,zhuang2019local,misra2020self,han2020memory}.
%pathak2016context,noroozi2016unsupervised,he2020momentum}. 
%~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,ji2019invariant,sohn2016improved,icmlunsupervised,ye2019unsupervised}.  
It refers to learning data representations that capture potential labels of interest, and doing so without human supervision. Contrastive learning is increasingly considered as a standard and highly competitive method for unsupervised representation learning. Features learned with this method have been shown to generalize well to downstream tasks,  and in some cases surpass the performance of supervised models~\cite{oord2018representation,caron2020unsupervised,tschannen2019mutual,chen2020simple,chen2020big,chen2020improved}. 
 
Contrastive learning learns representations by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. 
 
Despite its effectiveness, contrastive learning is vulnerable to shortcuts -- i.e., if simple features are contrastive enough to separate positive samples from negative samples, contrastive learning might learn such simple (or simpler) features though they may be irrelevant to the tasks of interest, and ignore other more relevant features. For example, the authors of \cite{chen2020simple} show that color distribution can be a shortcut to distinguish patches cropped from the same image, from patches from different images; yet such feature is not very useful for object classification. Past work manually designs data augmentations to break such shortcuts, so that the network may learn the relevant information \cite{he2020momentum,chen2020simple,chen2020big,chen2020improved}. 

However, it is not always possible to address shortcuts via data augmentation. First, machine learning tasks are expanding to new modalities, many of which are not directly interpretable by humans such as radio signals~\cite{zhao2018through,zhao2018rf,zhao2019through,li2019making,fan2020learning,fan2020home}, or acceleration data~\cite{hsu2019enabling,hsu2017zero,fan2020learning}. Consider for example the task of through-wall pose estimation~\cite{zhao2018through}. This task leverages that radio signals traverse walls and occlusions and reflect off the human body; it designs neural network models that analyze the radio frequency (RF) signals and infer the human pose, even when people are behind a wall. Such task would benefit significantly from unsupervised representation learning given the limited amount of labeled RF signals, and the difficulties of labeling such modality which is not interpretable by human workers~\cite{zhao2018through,zhao2018rf,zhao2019through,li2019making}. However, like RGB data, RF data can have shortcuts that make contrastive learning ineffective (see the results section for empirical validation). But unlike RGB data, it is hard for humans to guess what the shortcuts may be, or how to alter the RF signal to create data augmentations that eliminate the shortcuts, while preserving useful information. %\red{And even for RGB data, as shown in Sec. \ref{sec:shortcut}, it can also be hard to reason about what is the actual shortcut.} 

\begin{wrapfigure}{r}{77mm}
\begin{center}
\includegraphics[width=\linewidth]{pos-neg}
\end{center}
\vspace{-15pt}
\caption{\footnotesize{Shortcut Example. The input has two types of information: digit and background object, but existing contrastive learning methods generate a representation that focuses on the background object and ignores the digit.}}
\label{fig:intro}
\vspace{-5pt}
\end{wrapfigure}

Second, eliminating shortcut features is not always desirable, even for RGB-based tasks. Sometimes the shortcut features are irrelevant to one downstream task but important to another task. For example, the authors of \cite{tian2020makes} highlight the scenario in Figure~\ref{fig:intro}, where each image shows a digit (from MNIST) on a randomly chosen background object (from STL-10).  They show that features related to the background object can create a shortcut that prevents contrastive learning from learning features related to the digit. However, eliminating features about the background object is not desirable since ideally one would like a representation that works for both downstream tasks: digit classification, and background object classification. Similar problem exists in the task of human face attribute classification, where each face image can be used in multiple downstream tasks including gender, age, and ethnicity classification, but the features learned by contrastive learning can be biased to only one of them and show poor performance on other tasks (Sec. \ref{sec:rgb})

To address the above problems, we propose a new framework that we call information-preserving contrastive learning (IPCL). The key idea underlying IPCL is to learn representations using contrastive and reconstructive learning simultaneously. We use the term reconstructive learning to refer to tasks that force the representation to reconstruct the input, such as inpainting, colorization, or autoencoding. Such tasks counter the effect of shortcuts because they force the learned features to both abstract and retain the information in the input. Once combined with reconstructive learning,  contrastive learning ensures that all useful features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples. Thus, reconstructive learning maximizes the useful information in the representation, whereas contrastive learning orders the information in the embedding space to make it easy for a simple classifier to slice the embedding space to satisfy a desired task. 

%The key idea underlying IPCL is to ensure that even when the data has potential shortcuts, the representation will learn features about all types of semantic information in the data (digit and background object), and contrastive learning will ensure that all of those features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples.  To ensure that these properties are satisfied, IPCL augments contrastive learning with an auxiliary task that uses the learned representation to restore randomly cropped patches in the anchor sample. By doing so, IPCL ensures that the learned representation summarizes all useful information in the input, but also enjoys contrastive properties. 


%We apply the IPCL framework to both RGB-based and RF-based tasks, designing neural network models appropriate for those modalities.   

We evaluate IPCL  and compare it with state-of-the-art contrastive learning baselines such as  SimCLR~\cite{chen2020simple}, MoCo~\cite{he2020momentum}, and Contrastive Predictive Coding (CPC)~\cite{henaff2019data}. We summarize our findings for RGB and RF data as follows:

%\begin{Itemize}
%\item 

%\item 
{\it (a) Results on RGB Data:}
we evaluate IPCL on four different RGB datasets: Colorful-MNIST \cite{tian2020makes}, FairFace \cite{karkkainen2019fairface}, MPII \cite{andriluka20142d} and ImageNet-100 \cite{tian2019contrastive}. On Colorful-MNIST, in comparison to the contrastive learning baselines, the \name~representation has 72\% higher accuracy on digit classification and comparable performance on background classification. On FairFace, \name~improves over baselines performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%). On MPII, \name~outperforms baselines by 3.7 PCKh under fixed feature encoder setting and 0.7 PCKh under fine-tuning setting. And on ImageNet-100, IPCL is much more robust to the choice of image augmentations than contrastive methods. It achieves comparable results as state-of-the-art contrastive learning methods under full sets of augmentations (\red{80.5\%} vs. \red{81.2\%}), and keeps displaying good performance when only a subset of augmentations are applied while the performance of other contrastive baselines drops significantly (\red{74.2\%} vs. \red{67.2}\% when only applying random crop as augmentation).

{\it (a) Results on RF Data:}
We evaluate IPCL on three real-world RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. 
The results show that IPCL outperforms all contrastive learning baselines on all tasks.  In comparison to the best performing contrastive learning baseline, the IPCL representation improves performance by 30.6 mm, 81.4 mAP, and 24.5 mAP on the tasks of pose estimation, action recognition, and person re-id respectively.  
%Further, initializing supervised learning with the IPCL representation improves performance for all three tasks, confirming that self-supervision is beneficial for learning from non-interpretable data. 
Interestingly, the representations learned by the contrastive learning baselines perform worse than random features on pose estimation and action recognition. This shows that contrastive learning converged on a shortcut, and discarded key information necessary for these two  tasks.  

%\red{We also empirically show the complexity of reasoning about shortcuts even in RGB images, and how IPCL overcomes this complexity.}

%Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

%\end{Itemize}

To summarize, our paper has the following contributions:
\begin{Itemize}
\vspace{-8pt}
    \item We introduce IPCL, the first self-supervised learning framework that integrates contrastive and reconstructive learning to automatically avoid shortcuts and provide a representation that supports multiple different downstream tasks. Note that while both contrastive and reconstructive learning existed prior to our work, no past work has discovered their complementary role or proposed to combine them the way we do.     
        \item We empirically show the negative impact shortcuts have on contrastive learning, and how IPCL addresses these issues.
        \item We demonstrate that \name~outperforms SOTA contrastive learning methods on its ability to avoid shortcuts on multiple RGB datasets under various tasks. We are also the first to study unsupervised representation learning from radio signals, demonstrating the possibility of boosting the performance of RF-based human sensing tasks by leveraging unlabeled RF signals. 
\vspace{-8pt}
\end{Itemize}



==> source/intro-5.tex <==
\section{Introduction}
\vspace{-4pt}
The area of unsupervised or self-supervised representation learning is growing rapidly~\cite{he2020momentum,doersch2015unsupervised,ye2019unsupervised,hjelm2018learning,grill2020bootstrap,bachman2019learning,zhuang2019local,misra2020self,han2020memory}.
%pathak2016context,noroozi2016unsupervised,he2020momentum}. 
%~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,ji2019invariant,sohn2016improved,icmlunsupervised,ye2019unsupervised}.  
It refers to learning data representations that capture potential labels of interest, and doing so without human supervision. Contrastive learning is increasingly considered as a standard and highly competitive method for unsupervised representation learning. Features learned with this method have been shown to generalize well to downstream tasks,  and in some cases surpass the performance of supervised models~\cite{oord2018representation,caron2020unsupervised,tschannen2019mutual,chen2020simple,chen2020big,chen2020improved}. 
 
Contrastive learning learns representations by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. 
 
Yet contrastive learning is vulnerable to shortcuts -- i.e., if simple features are contrastive enough to separate positive samples from negative samples, contrastive learning might learn such simple (or simpler) features even if irrelevant to the tasks of interest, and ignore other more relevant features. For example, the authors of \cite{chen2020simple} show that color distribution can be a shortcut to distinguish patches cropped from the same image, from patches from different images; yet such feature is not useful for object classification. Past work addresses this problem by designing handcrafted data augmentations to break such shortcuts, so that the network may learn the relevant information \cite{he2020momentum,chen2020simple,chen2020big,chen2020improved,chen2020intriguing}. 

However, it is not always possible to address shortcuts via data augmentation. In particular, machine learning tasks are expanding to new modalities, many of which are not directly interpretable by humans such as radio signals~\cite{zhao2018through,zhao2019through,li2019making,fan2020learning} or acceleration data~\cite{hsu2019enabling,hsu2017zero,fan2020learning}. Consider for example the task of through-wall pose estimation~\cite{zhao2018through}. This task leverages the fact that radio signals traverse walls and reflect off the human body; it designs neural networks that analyze radio signals to infer the human pose through walls and occlusions. Like RGB data, radio signals can have shortcuts that make contrastive learning ineffective (see the results section for empirical validation). But given a radio signal (Fig. \ref{fig:intro_rf} (a)), it is hard for humans to guess what shortcuts may exist, or how to alter the signal to create data augmentations that eliminate the shortcuts, while preserving the relevant information. 

\begin{figure}
\begin{center}
%\includegraphics[width=\linewidth]{pos-neg}
\vspace{-15pt}
\begin{tabular}{ccc}
\includegraphics[width=0.148\textwidth]{rf.png} & \hspace*{-0.12in}
\label{fig:intro_rf}
\includegraphics[width=0.148\textwidth]{digit.jpg} & \hspace*{-0.12in}
\includegraphics[width=0.148\textwidth]{face.jpg}\\
{\footnotesize (a) Radio Signal} & \hspace*{-0.12in} {\footnotesize (b) Digit \& Bkgd} & \hspace*{-0.12in} {\footnotesize (c) Face Attribute}
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{\footnotesize{(a) Radio signals can have shortcuts that are hard to eliminate via handcrafted data augmentations. (b) In Colorful-MNIST \cite{tian2020makes}, the input has two types of information: digit and background object. But contrastive learning methods focus on the background object and ignore the digit. (c) Each image in FairFace \cite{karkkainen2019fairface} has multiple attributes such as age, gender, ethnicity, etc. Existing contrastive learning methods focus on ethnicity and partially ignore other attributes.}}
\label{fig:intro}
\vspace{-11pt}
\end{figure}

Even if the modality is interpretable (e.g., RGB), it is hard to design augmentations that generalize across different downstream tasks.
For example, the authors of \cite{tian2020makes} highlight the scenario in Fig.~\ref{fig:intro} (b), where each image shows a digit (from MNIST) on a randomly chosen background object (from STL-10).  They show that features related to background objects can create a shortcut that prevents contrastive learning from learning features related to digits. It is unclear how to design augmentations to learn features useful for digit classification, while keeping good performance on background object classification. A similar problem exists in the task of human face attribute classification, where each face image can be used in multiple downstream tasks including gender, age, and ethnicity classification (Fig.~\ref{fig:intro} (c)), but the features learned by contrastive learning can be biased to only one of the attributes (e.g., ethnicity) and show poor performance on other attributes (gender and age) (Sec. \ref{sec:rgb}). In this case, it is hard to come up with data augmentations that eliminate the shortcut attribute without harming the corresponding classification task. 

To solve this problem, we propose reconstructive contrastive learning (\name), a new unsupervised learning framework that works across different modalities and tasks. The key idea underlying \name~is to learn representations using contrastive and reconstructive learning simultaneously. We use the term reconstructive learning to refer to tasks that force the representation to reconstruct the input, such as inpainting, colorization, or autoencoding. Such tasks counter the effect of shortcuts because they force the learned features to retain the information in the input. Once combined with reconstructive learning,  contrastive learning ensures that all useful features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples. Thus, reconstructive learning maximizes the useful information in the representation, whereas contrastive learning orders the information in the embedding space to make it easy for a simple classifier to slice the embedding space to satisfy a desired task. 

%The key idea underlying IPCL is to ensure that even when the data has potential shortcuts, the representation will learn features about all types of semantic information in the data (digit and background object), and contrastive learning will ensure that all of those features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples.  To ensure that these properties are satisfied, IPCL augments contrastive learning with an auxiliary task that uses the learned representation to restore randomly cropped patches in the anchor sample. By doing so, IPCL ensures that the learned representation summarizes all useful information in the input, but also enjoys contrastive properties. 


%We apply the IPCL framework to both RGB-based and RF-based tasks, designing neural network models appropriate for those modalities.   

We evaluate \name~and compare it with state-of-the-art contrastive learning baselines on four different RGB datasets: ImageNet-100 \cite{tian2019contrastive},  MPII \cite{andriluka20142d}, Colorful-MNIST \cite{tian2020makes}, and FairFace \cite{karkkainen2019fairface}, and three RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. For all tasks, \name~achieves superior performance and outperforms the state-of-the-art baselines by large margins, demonstrating its robustness against shortcuts and its ability to learn general features for different downstream tasks. 

To summarize, this paper makes the following contributions:
\begin{Itemize}
\vspace{-7pt}
    \item It introduces \name, the first self-supervised learning framework that integrates contrastive and reconstructive learning to automatically avoid shortcuts and provide a representation that supports multiple different downstream tasks.     
        \item It empirically shows the negative impact shortcuts have on contrastive learning and demonstrates that \name~outperforms SOTA contrastive learning in its ability to avoid shortcuts and learn general representations that support multiple downstream tasks.
        \item The paper is also the first to study unsupervised representation learning from radio signals, demonstrating the possibility of boosting the performance of radio-based human sensing tasks by leveraging unlabeled radio signals. 
\vspace{-8pt}
\end{Itemize}



%\begin{Itemize}
%\item 

%\item 
%{\it (a) Results on RGB Data:}
%we evaluate IPCL on four different RGB datasets: Colorful-MNIST \cite{tian2020makes}, FairFace \cite{karkkainen2019fairface}, MPII \cite{andriluka20142d} and ImageNet-100 \cite{tian2019contrastive}. On Colorful-MNIST, in comparison to the contrastive learning baselines, the \name~representation has 72\% higher accuracy on digit classification and comparable performance on background classification. On FairFace, \name~improves over baselines performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%). On MPII, \name~outperforms baselines by 3.7 PCKh under fixed feature encoder setting and 0.7 PCKh under fine-tuning setting. And on ImageNet-100, IPCL is much more robust to the choice of image augmentations than contrastive methods. It achieves comparable results as state-of-the-art contrastive learning methods under full sets of augmentations (\red{80.5\%} vs. \red{81.2\%}), and keeps displaying good performance when only a subset of augmentations are applied while the performance of other contrastive baselines drops significantly (\red{74.2\%} vs. \red{67.2}\% when only applying random crop as augmentation).
%
%{\it (a) Results on RF Data:}
%We evaluate IPCL on three real-world RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. 
%The results show that IPCL outperforms all contrastive learning baselines on all tasks.  In comparison to the best performing contrastive learning baseline, the IPCL representation improves performance by 30.6 mm, 81.4 mAP, and 24.5 mAP on the tasks of pose estimation, action recognition, and person re-id respectively.  
%%Further, initializing supervised learning with the IPCL representation improves performance for all three tasks, confirming that self-supervision is beneficial for learning from non-interpretable data. 
%Interestingly, the representations learned by the contrastive learning baselines perform worse than random features on pose estimation and action recognition. This shows that contrastive learning converged on a shortcut, and discarded key information necessary for these two  tasks.  

%\red{We also empirically show the complexity of reasoning about shortcuts even in RGB images, and how IPCL overcomes this complexity.}

%Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

%\end{Itemize}


==> source/intro-6.tex <==
\section{Introduction}
\vspace{-4pt}

% The RF-based vision 
Nowadays, RF-based vision has emerged as an attracting research direction that uses Radio Frequency (RF) signals to ``see'' the human and their pose and activities, even in the presence of occlusions and poor lighting conditions. While visible light is easily blocked by walls and opaque objects, RF signals in the WiFi range can traverse such occlusions. The RF signals reflect off the human body, provide information to track people and capture their shape and actions. Previous works have leveraged those properties to detect people and track their walking speed. More recent advances in RF-based learning system have demonstrated the feasibility of using neural network to learning from RF signals for pose estimation, action recognition, scene captioning, and human re-identification though walls and in dark settings. 


Most of these RF-based learning systems are using supervised learning on RF signals for specific tasks. However, unlike vision-based datasets which can be labeled by human workers, labeling RF signals is a daunting task because such signals are not human interpretable. Specifically, when collecting the RF datasets, people usually deploy a RF device and a camera system simoutaneously, and recording the synchronized RF data and RGB data. The annotator then generate the label based on the RGB data. However, in the home senario, most people would have privacy concerns about deploying cameras at home, particularly in the bedroom and bathroom. Also, a single camera usually has a limited field of view; thus, users would need to deploy multiple cameras covering different rooms, which would introduce a significant overhead. Moreover, cameras do not work well in dark settings and occlusions, which are common scenarios at home. Limited by the small amount of annotated RF dataset, some of the previous methods for RF-based vision task also use the transfer learning to leverage the RGB knowledge to the RF task. 

We want to ask the question -- can we use the self-supervised learning on unlabled RF data to learn the representations that help the RF-based vision tasks? The first reason is that, it is fairly easy to collect unlabelled RF signals. Second, previous transfer learning from RGB data may introduce some bias from the RGB modality, while learning from RF data itself may discover the information and property of RF modality. Therefore, one would like to leverage such unlabeled RF data to learn useful representations that can improve the accuracy of the aforementioned tasks.

The area of unsupervised or self-supervised representation learning in RGB-based computer vision is growing rapidly~\cite{he2020momentum,doersch2015unsupervised,ye2019unsupervised,hjelm2018learning,grill2020bootstrap,bachman2019learning,zhuang2019local,misra2020self,han2020memory}.
%pathak2016context,noroozi2016unsupervised,he2020momentum}. 
%~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,ji2019invariant,sohn2016improved,icmlunsupervised,ye2019unsupervised}.  
It refers to learning data representations that capture potential labels of interest, and doing so without human supervision. Contrastive learning is increasingly considered as a standard and highly competitive method for unsupervised representation learning. Features learned with this method have been shown to generalize well to downstream tasks,  and in some cases surpass the performance of supervised models~\cite{oord2018representation,caron2020unsupervised,tschannen2019mutual,chen2020simple,chen2020big,chen2020improved}. 
 
Contrastive learning learns representations by contrasting positive samples against negative samples. During training, a data sample is chosen as an anchor (e.g., an image);  positive samples are chosen as different augmented versions of the anchor (e.g., randomly cropping and color distorting the image), whereas negative samples come from other samples in the dataset. 
 
Yet contrastive learning is vulnerable to shortcuts -- i.e., if simple features are contrastive enough to separate positive samples from negative samples, contrastive learning might learn such simple (or simpler) features even if irrelevant to the tasks of interest, and ignore other more relevant features. For example, the authors of \cite{chen2020simple} show that color distribution can be a shortcut to distinguish patches cropped from the same image, from patches from different images; yet such feature is not useful for object classification. Past work addresses this problem by designing handcrafted data augmentations to break such shortcuts, so that the network may learn the relevant information \cite{he2020momentum,chen2020simple,chen2020big,chen2020improved,chen2020intriguing}. 

However, it is not always possible to address shortcuts via data augmentation. In particular, machine learning tasks are expanding to new modalities, many of which are not directly interpretable by humans such as radio signals~\cite{zhao2018through,zhao2019through,li2019making,fan2020learning} or acceleration data~\cite{hsu2019enabling,hsu2017zero,fan2020learning}. Consider for example the task of through-wall pose estimation~\cite{zhao2018through}. This task leverages the fact that radio signals traverse walls and reflect off the human body; it designs neural networks that analyze radio signals to infer the human pose through walls and occlusions. Like RGB data, radio signals can have shortcuts that make contrastive learning ineffective (see the results section for empirical validation). But given a radio signal (Fig. \ref{fig:intro_rf} (a)), it is hard for humans to guess what shortcuts may exist, or how to alter the signal to create data augmentations that eliminate the shortcuts, while preserving the relevant information. 

\begin{figure}
\begin{center}
%\includegraphics[width=\linewidth]{pos-neg}
\vspace{-15pt}
\begin{tabular}{ccc}
\includegraphics[width=0.148\textwidth]{rf.png} & \hspace*{-0.12in}
\label{fig:intro_rf}
\includegraphics[width=0.148\textwidth]{digit.jpg} & \hspace*{-0.12in}
\includegraphics[width=0.148\textwidth]{face.jpg}\\
{\footnotesize (a) Radio Signal} & \hspace*{-0.12in} {\footnotesize (b) Digit \& Bkgd} & \hspace*{-0.12in} {\footnotesize (c) Face Attribute}
\end{tabular}
\end{center}
\vspace{-10pt}
\caption{\footnotesize{(a) Radio signals can have shortcuts that are hard to eliminate via handcrafted data augmentations. (b) In Colorful-MNIST \cite{tian2020makes}, the input has two types of information: digit and background object. But contrastive learning methods focus on the background object and ignore the digit. (c) Each image in FairFace \cite{karkkainen2019fairface} has multiple attributes such as age, gender, ethnicity, etc. Existing contrastive learning methods focus on ethnicity and partially ignore other attributes.}}
\label{fig:intro}
\vspace{-11pt}
\end{figure}

Even if the modality is interpretable (e.g., RGB), it is hard to design augmentations that generalize across different downstream tasks.
For example, the authors of \cite{tian2020makes} highlight the scenario in Fig.~\ref{fig:intro} (b), where each image shows a digit (from MNIST) on a randomly chosen background object (from STL-10).  They show that features related to background objects can create a shortcut that prevents contrastive learning from learning features related to digits. It is unclear how to design augmentations to learn features useful for digit classification, while keeping good performance on background object classification. A similar problem exists in the task of human face attribute classification, where each face image can be used in multiple downstream tasks including gender, age, and ethnicity classification (Fig.~\ref{fig:intro} (c)), but the features learned by contrastive learning can be biased to only one of the attributes (e.g., ethnicity) and show poor performance on other attributes (gender and age) (Sec. \ref{sec:rgb}). In this case, it is hard to come up with data augmentations that eliminate the shortcut attribute without harming the corresponding classification task. 

To solve this problem, we propose reconstructive contrastive learning (\name), a new unsupervised learning framework that works across different modalities and tasks. The key idea underlying \name~is to learn representations using contrastive and reconstructive learning simultaneously. We use the term reconstructive learning to refer to tasks that force the representation to reconstruct the input, such as inpainting, colorization, or autoencoding. Such tasks counter the effect of shortcuts because they force the learned features to retain the information in the input. Once combined with reconstructive learning,  contrastive learning ensures that all useful features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples. Thus, reconstructive learning maximizes the useful information in the representation, whereas contrastive learning orders the information in the embedding space to make it easy for a simple classifier to slice the embedding space to satisfy a desired task. 

%The key idea underlying IPCL is to ensure that even when the data has potential shortcuts, the representation will learn features about all types of semantic information in the data (digit and background object), and contrastive learning will ensure that all of those features (not just the shortcut features) are closely mapped in the embedding space for positive samples, and stay distant for negative samples.  To ensure that these properties are satisfied, IPCL augments contrastive learning with an auxiliary task that uses the learned representation to restore randomly cropped patches in the anchor sample. By doing so, IPCL ensures that the learned representation summarizes all useful information in the input, but also enjoys contrastive properties. 


%We apply the IPCL framework to both RGB-based and RF-based tasks, designing neural network models appropriate for those modalities.   

We evaluate \name~and compare it with state-of-the-art contrastive learning baselines on four different RGB datasets: ImageNet-100 \cite{tian2019contrastive},  MPII \cite{andriluka20142d}, Colorful-MNIST \cite{tian2020makes}, and FairFace \cite{karkkainen2019fairface}, and three RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. For all tasks, \name~achieves superior performance and outperforms the state-of-the-art baselines by large margins, demonstrating its robustness against shortcuts and its ability to learn general features for different downstream tasks. 

To summarize, this paper makes the following contributions:
\begin{Itemize}
\vspace{-7pt}
    \item It introduces \name, the first self-supervised learning framework that integrates contrastive and reconstructive learning to automatically avoid shortcuts and provide a representation that supports multiple different downstream tasks.     
        \item It empirically shows the negative impact shortcuts have on contrastive learning and demonstrates that \name~outperforms SOTA contrastive learning in its ability to avoid shortcuts and learn general representations that support multiple downstream tasks.
        \item The paper is also the first to study unsupervised representation learning from radio signals, demonstrating the possibility of boosting the performance of radio-based human sensing tasks by leveraging unlabeled radio signals. 
\vspace{-8pt}
\end{Itemize}



%\begin{Itemize}
%\item 

%\item 
%{\it (a) Results on RGB Data:}
%we evaluate IPCL on four different RGB datasets: Colorful-MNIST \cite{tian2020makes}, FairFace \cite{karkkainen2019fairface}, MPII \cite{andriluka20142d} and ImageNet-100 \cite{tian2019contrastive}. On Colorful-MNIST, in comparison to the contrastive learning baselines, the \name~representation has 72\% higher accuracy on digit classification and comparable performance on background classification. On FairFace, \name~improves over baselines performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%). On MPII, \name~outperforms baselines by 3.7 PCKh under fixed feature encoder setting and 0.7 PCKh under fine-tuning setting. And on ImageNet-100, IPCL is much more robust to the choice of image augmentations than contrastive methods. It achieves comparable results as state-of-the-art contrastive learning methods under full sets of augmentations (\red{80.5\%} vs. \red{81.2\%}), and keeps displaying good performance when only a subset of augmentations are applied while the performance of other contrastive baselines drops significantly (\red{74.2\%} vs. \red{67.2}\% when only applying random crop as augmentation).
%
%{\it (a) Results on RF Data:}
%We evaluate IPCL on three real-world RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. 
%The results show that IPCL outperforms all contrastive learning baselines on all tasks.  In comparison to the best performing contrastive learning baseline, the IPCL representation improves performance by 30.6 mm, 81.4 mAP, and 24.5 mAP on the tasks of pose estimation, action recognition, and person re-id respectively.  
%%Further, initializing supervised learning with the IPCL representation improves performance for all three tasks, confirming that self-supervision is beneficial for learning from non-interpretable data. 
%Interestingly, the representations learned by the contrastive learning baselines perform worse than random features on pose estimation and action recognition. This shows that contrastive learning converged on a shortcut, and discarded key information necessary for these two  tasks.  

%\red{We also empirically show the complexity of reasoning about shortcuts even in RGB images, and how IPCL overcomes this complexity.}

%Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

%\end{Itemize}


==> source/intro-7.tex <==
\section{Introduction}
\vspace{-4pt}

% The RF-based vision 
Nowadays, RF-based vision has emerged as an attractive research direction that uses Radio Frequency (RF) signals to ``see'' the human and their pose and activities, even in the presence of occlusions and poor lighting conditions. While visible light can be easily blocked by walls and opaque objects, RF signals in the WiFi range can traverse such occlusions. The RF signals reflect off the human body, provide information to track people, and capture their shape and actions. Previous works have leveraged those properties to detect people and track their walking speed. More recent advances in RF-based learning systems have demonstrated the feasibility of using neural networks to perform various computer vision tasks like pose estimation, action recognition, scene captioning, and human re-identification using RF signals solely as inputs. Moreover, these systems are capable of working normally through walls and in dark scenarios, and thus go beyond the limitations faced with vision-based systems. 


Most of these RF-based learning systems are using supervised learning on RF signals for specific tasks. However, unlike vision-based datasets, which can be labeled by human workers, labeling RF signals is a daunting task because such signals are not human interpretable. To label such datasets, a synchronized human-interpretable stream, like video, should be presented to assist the annotator. Specifically, when collecting the RF datasets, people usually deploy a RF device and a camera system simoutaneously, and recording the synchronized RF data and RGB data. The annotator then generates the label based on the RGB data. However, using RGB as assistance could only label a small portion of RF data. RF data are typically collected indoor or in people's home, where most people would have privacy concerns about deploying cameras. Also, a single camera usually has a limited field of view; thus, users would need to deploy a multi-camera system covering different rooms, introducing significant overhead. Moreover, cameras do not work well in dark settings and occlusions, which are common indoor scenarios. 

Meanwhile, the area of unsupervised or self-supervised representation learning in RGB-based computer vision is growing rapidly~\cite{he2020momentum,doersch2015unsupervised,ye2019unsupervised,hjelm2018learning,grill2020bootstrap,bachman2019learning,zhuang2019local,misra2020self,han2020memory}.
%pathak2016context,noroozi2016unsupervised,he2020momentum}. 
%~\cite{noroozi2016unsupervised,pathak2016context,gidaris2018unsupervised,oord2018representation,chen2020improved,he2020momentum,chen2020simple,chen2020big,ji2019invariant,sohn2016improved,icmlunsupervised,ye2019unsupervised}.  
It refers to learning data representations that capture potential labels of interest and doing so without human supervision. 
Therefore, it is natural for one to ask the question -- can we use self-supervised learning on unlabeled RF data to learn the representations that help the RF-based vision tasks? 
 
Yet applying self-supervised learning methods on RF data is not straight forward. RF data is quite different from RGB images in nature. It is obtained by analyzing the signal  power reflected from different locations in the space, as shown in \ref{fig:rf-heatmaps}. As a result, the signal reflected from the person could be extremely sparse, occupying <1\% of the total pixels. Therefore, directly applying reconstructive or contrastive unsupervised learning methods on the whole RF heatmap could be strongly biased by the background noises and fail to learn useful information about the person. Moreover, although achieving the state-of-the-art performance on RGB-based unsupervised learning, contrastive learning methods could easily learn shortcut such as color distribution and discard useful information \cite{chen2020intriguing} in the input. This is avoided by adding strong augmentations to remove the shortcut semantics \cite{chen2020simple}, but since RF signals is hard to interpret by humans, understanding the shortcut on RF signals and designing proper augmentations to remove it could be an extremely hard problem.

In this paper, we propose \name, the first self-supervised learning framework for RF-based human sensing tasks. To solve the sparsity problem, we leverage a signal processing module which removes reflections from static objects in the environment and localizes the person. We then perform reconstructive or contrastive training only inside this region of interest. We evaluate \name~and compare it with state-of-the-art supervised baselines on RF-based sensing tasks, including 3D pose estimation, action recognition, and person re-identification. Our results show that contrastive learning methods could still be strongly biased to shortcut and discard useful information about the person, while reconstructive learning methods could learn useful information and consistently improves the performance over supervised baselines under finetuning setting. To summarize, this paper makes the following contributions:
\begin{Itemize}
\vspace{-7pt}
    \item The paper is the first to study unsupervised representation learning from radio signals, demonstrating the possibility of boosting the performance of radio-based human sensing tasks by leveraging unlabeled radio signals.    
    \item It empirically shows the negative impact shortcuts have on contrastive learning when applied to RF signals. It also shows that reconstructive learning methods could be more robust and suitable for self-supervised learning on RF signals.
\vspace{-8pt}
\end{Itemize}



%\begin{Itemize}
%\item 

%\item 
%{\it (a) Results on RGB Data:}
%we evaluate IPCL on four different RGB datasets: Colorful-MNIST \cite{tian2020makes}, FairFace \cite{karkkainen2019fairface}, MPII \cite{andriluka20142d} and ImageNet-100 \cite{tian2019contrastive}. On Colorful-MNIST, in comparison to the contrastive learning baselines, the \name~representation has 72\% higher accuracy on digit classification and comparable performance on background classification. On FairFace, \name~improves over baselines performance on age and gender classification by 5.7\% and 8.6\% respectively, while keeping comparable performance on ethnicity classification (61.2\% vs. 62.3\%). On MPII, \name~outperforms baselines by 3.7 PCKh under fixed feature encoder setting and 0.7 PCKh under fine-tuning setting. And on ImageNet-100, IPCL is much more robust to the choice of image augmentations than contrastive methods. It achieves comparable results as state-of-the-art contrastive learning methods under full sets of augmentations (\red{80.5\%} vs. \red{81.2\%}), and keeps displaying good performance when only a subset of augmentations are applied while the performance of other contrastive baselines drops significantly (\red{74.2\%} vs. \red{67.2}\% when only applying random crop as augmentation).
%
%{\it (a) Results on RF Data:}
%We evaluate IPCL on three real-world RF-based sensing tasks: 3D pose estimation, human action recognition, and person re-identification. 
%The results show that IPCL outperforms all contrastive learning baselines on all tasks.  In comparison to the best performing contrastive learning baseline, the IPCL representation improves performance by 30.6 mm, 81.4 mAP, and 24.5 mAP on the tasks of pose estimation, action recognition, and person re-id respectively.  
%%Further, initializing supervised learning with the IPCL representation improves performance for all three tasks, confirming that self-supervision is beneficial for learning from non-interpretable data. 
%Interestingly, the representations learned by the contrastive learning baselines perform worse than random features on pose estimation and action recognition. This shows that contrastive learning converged on a shortcut, and discarded key information necessary for these two  tasks.  

%\red{We also empirically show the complexity of reasoning about shortcuts even in RGB images, and how IPCL overcomes this complexity.}

%Our method can achieve 11.7\% error rate on digit classification and 54.0\% error rate on background object classification, while all other contrastive learning baselines have near-random error rate on digit classification ($\sim$90\%) and have comparable error rates to IPCL on background object classification (51\% to 64\%). The second dataset is FairFace~\cite{karkkainen2019fairface}, where we show that IPCL is more effective than state-of-the-art contrastive learning at learning a single representation that works for multiple downstream classification tasks based on race, gender and age. \name~outperforms SimCLR on age and gender classification by 5.7\% and 8.6\% in error rate, and achieves comparable results as SimCLR on ethnicity classification (38.8\% vs. 37.7\% error rate).

%\end{Itemize}


==> source/intro.tex <==
\section{Introduction}

Radio Frequency(RF) signals have been demonstrated to be effective for capturing human information, such as skeleton, action, or even 3D meshes. Moreover, as RF signals could traverse through occlusions and not depend on visible lights, RF-based systems have the ability to detect human information even when people are behind walls or in dark scenarios. Such characteristics could make up for the RGB-based systems to a large extent since they can't `see' people when they are behind the walls or in a completely dark room. Another advantage for RF signals are that they are privacy preserving, as these signals can not be interpretable by human. Thus people can deploy such systems in their homes without worrying about revealing privacy.

However, to equip such system with the ability to predict superior human poses or actions from RF inputs, one always need to have a large-scale RF dataset with accurate labels for each task, which requires massive human labor. Also, since RF signals are not human interpretable, to label such datasets, we need to collect synchronized RGB videos so that labelers know what's going on and can label human body key-points or actions accordingly. Moreover, this process would break the privacy-preserving property of RF signals and make the applicable scene quite limited, as most people would disagree to deploy a camera in their home.
Therefore it would be beneficial if we could have some unsupervised learning approaches to learn representations that are helpful for various downstream tasks from unlabeled RF data.

Meanwhile, unsupervised learning approaches on large scale image and video datasets are being developed rapidly. Recently literature has shown unsupervised learning trained models outperform models trained in a supervised manner.
It would be great if we could adapt these unsupervised learning methods to the modality of RF.

However, it is not easy to directly transfer off-the-shelf unsupervised learning approaches for image inputs to RF inputs due to several reasons: (1) RF contains massive irrelevant information that unsupervised learning approaches could easily bias to, like environment information, and such information is completely useless for downstream tasks like pose estimation or action recognition and may even harm the performance. (2) RF signals are much more sparse than RGB images. There are only limited regions containing useful information related to human-beings within each frame, and other parts contain mostly background noises, which are usually not helpful.

In this paper, we aim to design an effective unsupervised learning approach for input modalities with significant background noises, like radio signals.
We propose a theory for learning usable features from contrastive learning approaches, and proved why contrastive learning can easily bias to useless information like backgrounds or environments for RF signals. We then propose an approach to combine predictive learning and contrastive learning to boost performance while learning features meaningful for downstream tasks.

To demonstrate our theory and the effectiveness of our proposed, we use a synthesized dataset to show that, when multiple kinds of mutual information exist among positive samples, traditional contrastive learning approaches can learn ONLY one of them. We then show our proposed approach could learn all of the existing mutual information without performance drop for every one of the downstream tasks.
We also evaluate our approach on two real-world RF datasets: 3D Pose Estimation and Human action detection. Our experiment results show the proposed unsupervised learning approach can significantly improve the performance on each task, and outperform all existing unsupervised learning counterparts.

To summarize, our paper has the following contributions:
\begin{Itemize}
    \item We are the first to study unsupervised learning approaches for the modality of RF signals, showing the possibility to boost performance for RF-based sensing approaches with unsupervised learning.
    \item We prove that when multiple types of mutual information exist among positive samples, traditional contrastive learning can easily bias to one of them while completely ignoring others.      
    \item We further introduce an approach to combine predictive and contrastive learning to learn ALL possibly useful information from inputs while keeping high performance for each one of the downstream tasks. 
    \item We evaluate our proposed approach on both synthetic and real-world RF datasets, showing the effectiveness of our proposed Predictive-Contrastive Learning approach. 
\end{Itemize}



==> source/method-2.tex <==
\section{Predictive-Contrastive Learning}
Previous work has shown that contrastive learning can be easily biased to 'shortcut' semantics in the image. Traditional methods  address this bias through data augmentations to break the 'shortcut' semantics so that the network will learn the desired semantics. Such a design however suffers from multiple problems:

\begin{enumerate}
\item It requires knowing which types of semantics can be shortcut and designing specific augmentations to remove that shortcut. However for modalities like RF, which are not directly interpretable by humans, it is unclear to a human  which semantics in the RF signal create a shortcut.  As a result, it is hard to design augmentation techniques to remove the shortcut. 
\item
Another problem is that the shortcut semantics can be highly correlated with the useful semantics, in which case it may be impossible to remove the shortcut semantics while keeping those useful semantics untouched. 
\item
Last, as shown in \cite{xxx}, there might be multiple types of semantics that are useful for downstream tasks, and one type of them can be a shortcut with respect with respect to one task but a key useful feature for another task. In this case, removing a shortcut might help one downstream task but hurt the other, making it hard to learn a representation that generalizes well to multiple downstream tasks.
\end{enumerate}

To address the above problems, we need an unsupervised representation learning method that does not require knowledge of the potential shortcut semantics in the data, and can learn a representation that preserves the different semantics in the input, even when one type of semantic information can be a shortcut for contrastive learning. 


Our idea is to use the task of predicting missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a potential shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By predicting missing patches, we mean predicting randomly cropped regions in the input, e.g., image inpainting. This task has traditionally been used as a pretext task in self-supervised learning. Here however we use it as a regularization of contrastive learning. 


We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning. Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input. Such a representation contains all semantics of the input. Next,  we add the contrastive loss into the training procedure while keeping the predictive inpainting loss. This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.

In the following sections, we will show how we apply \name~on both a hand-crafted image dataset and real-world RF datasets, and extensive experiments shows that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/method-3.tex <==
\section{Predictive-Contrastive Learning}
Previous work has shown that contrastive learning can be easily biased to 'shortcut' semantics in the image. Traditional methods  address this bias through data augmentations to break the 'shortcut' semantics so that the network will learn the desired semantics. Such a design however suffers from multiple problems:

\begin{enumerate}
\item It requires knowing which types of semantics can be shortcut and designing specific augmentations to remove that shortcut. However for modalities like RF, which are not directly interpretable by humans, it is unclear to a human  which semantics in the RF signal create a shortcut.  As a result, it is hard to design augmentation techniques to remove the shortcut. 
\item
Another problem is that the shortcut semantics can be highly correlated with the useful semantics, in which case it may be impossible to remove the shortcut semantics while keeping those useful semantics untouched. 
\item
Last, as shown in \cite{xxx}, there might be multiple types of semantics that are useful for downstream tasks, and one type of them can be a shortcut with respect with respect to one task but a key useful feature for another task. In this case, removing a shortcut might help one downstream task but hurt the other, making it hard to learn a representation that generalizes well to multiple downstream tasks.
\end{enumerate}

To address the above problems, we need an unsupervised representation learning method that does not require knowledge of the potential shortcut semantics in the data, and can learn a representation that preserves the different semantics in the input, even when one type of semantic information can be a shortcut for contrastive learning. 


\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{framework}
\end{center}
\caption{Illustration of our \name framework. The goal for \name is to train a good encoder network $\theta$ which can encode inputs into a latent space which is useful for various downstream tasks. For the initialization step we only train the network using the predictive loss $l_p$ (blue box). In the full training step we use a combination of predictive loss $l_p$ and contrastive loss $l_c$ to train the network weights.}\label{fig:framework}
\end{figure}


Our idea is to use the task of predicting missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a potential shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By predicting missing patches, we mean predicting randomly cropped regions in the input, e.g., image inpainting. This task has traditionally been used as a pretext task in self-supervised learning. Here however we use it as a regularization of contrastive learning. 

We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning, as shown in Figure \ref{fig:framework}.
Denote the input as $x$, the mask operation as $\mathbb{M}$, and augmentation as $\tau_1, \tau_2$. The goal for \name is to train a good encoder network $\theta$ which could encode input $x$ into a embedding space which is useful for various downstream tasks.

Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input, as shown in the blue box on the left. 
Given an input image $x$, it is first masked randomly to get $\mathbb{M}(x)$. Then the input is passed through encoder network $\theta$ and decoder network $\delta$ to get the reconstruction result $\delta(\theta(\mathbb{M}(x)))$. The prediction loss is added between original input $x$ and the reconstructed one $\delta(\theta(\mathbb{M}(x)))$: 
$$
l_p = ||\delta(\theta(\mathbb{M}(x)))-x||_2
$$
This will force the representation to contain all semantics of the input.

Next,  we add the contrastive loss into the training procedure while keeping the predictive inpainting loss (both the blue box and the orange box in Figure \ref{fig:framework}). 
As for the additional contrastive branch, for each image, we generate a pair of positive samples by two random augmentations $\tau_1$ and $\tau_2$, then the augmented inputs are fed through the encoder $\theta$ and a multi-layer nonlinear head $h$ to get latent representations for contrastive loss $l_c$.
The training loss for this stage is the combination of the aforementioned two loss:
$$
l = \lambda_1  \cdot l_p + \lambda_2 \cdot  l_c
$$
This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.


%We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning, as shown in Figure \ref{fig:framework} Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input. Such a representation contains all semantics of the input. Next,  we add the contrastive loss into the training procedure while keeping the predictive inpainting loss. This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.

In the following sections, we will show how we apply \name~on both a hand-crafted image dataset and real-world RF datasets, and extensive experiments shows that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/method-4.tex <==
\section{Predictive-Contrastive Learning}
Previous work has shown that contrastive learning can be easily biased to 'shortcut' semantics in the image. Traditional methods  address this bias through data augmentations to break the 'shortcut' semantics so that the network will learn the desired semantics. Such a design however suffers from multiple problems:

\begin{enumerate}
\item It requires knowing which types of semantics can be shortcut and designing specific augmentations to remove that shortcut. However for modalities like RF, which are not directly interpretable by humans, it is unclear to a human  which semantics in the RF signal create a shortcut.  As a result, it is hard to design augmentation techniques to remove the shortcut. 
\item
Another problem is that the shortcut semantics can be highly correlated with the useful semantics, in which case it may be impossible to remove the shortcut semantics while keeping those useful semantics untouched. 
\item
Last, as shown in \cite{xxx}, there might be multiple types of semantics that are useful for downstream tasks, and one type of them can be a shortcut with respect to one task but a key useful feature for another task. In this case, removing a shortcut might help one downstream task but hurt the other, making it hard to learn a representation that generalizes well to multiple downstream tasks.
\end{enumerate}

To address the above problems, we need an unsupervised representation learning method that does not require prior knowledge of the potential shortcut semantics in the data, and can learn a representation that preserves the different semantics in the input, even when one type of semantic information can be a shortcut for contrastive learning. 


\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{framework}
\end{center}
\caption{Illustration of our \name framework. The goal for \name is to train a good encoder network $\theta$ which can encode inputs into a latent space which is useful for various downstream tasks. For the initialization step we only train the network using the predictive loss $l_p$ (blue box). In the full training step we use a combination of predictive loss $l_p$ and contrastive loss $l_c$ to train the network weights.}\label{fig:framework}
\end{figure}


Our idea is to use the task of predicting missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a potential shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By predicting missing patches, we mean predicting randomly cropped regions in the input, e.g., image inpainting. This task has traditionally been used as a pretext task in self-supervised learning. Here however we use it as a regularization of contrastive learning. 

We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning, as shown in Figure \ref{fig:framework}. Our method can be separated to two different branches, one is a common contrastive learning branch which uses random augmentation on same image to generate positive pairs and maximizes similarity between features from them. Another is a missing patch prediction branch which masks out some part of the input and forces the network to reconstruct the missing patches. The goal for \name is to train a good encoder network which could encode input into an embedding space that is useful for various downstream tasks.

Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input, as shown in the blue box on the left. 
Given an input image $x$, it is first masked randomly to get masked input $\mathbb{M}(x)$. Then the input is passed through encoder network $E$ with parameter $\theta$ and decoder network $D$ with parameter $\delta$ to get the reconstruction result $D(E(\mathbb{M}(x)|\theta) |\delta)$. The prediction loss is added between original input $x$ and the reconstructed one $D(E(\mathbb{M}(x)|\theta) |\delta)$: 
$$
l_p = ||D(E(\mathbb{M}(x)|\theta) |\delta)-x||_2
$$
This will force the representation to contain as much important semantics of the input as possible.

Next, we add the contrastive loss into the training procedure while keeping the predictive inpainting loss as a regularization (both the blue box and the orange box in Figure \ref{fig:framework}). 
As for the additional contrastive branch, for each image, we generate a pair of positive samples by two random augmentations $\tau_1$ and $\tau_2$, then the augmented inputs are fed through the encoder $E$ and a multi-layer nonlinear head $h$ to get latent representations for contrastive loss $l_c$. We follow commonly used InfoNCE loss \cite{xxx} for this contrastive loss. Namely, for a input batch of images $x$ with $N$ different images,
$$l_c = -\sum_{i=1}^N \log \sum \frac{\exp\big(\text{sim}(z_{2i}, z_{2i+1})/T\big)}{\sum_{k=1}^{2N} \mathbbm{1}_{k\neq 2i}\exp\big(\text{sim}(z_{2i}, z_k)/T\big)} $$

where $z_{2i},z_{2i+1}$ are encoded features of positive pairs generated using $\tau_1$ and $\tau_2$ from one image. Then the training loss for this stage is the combination of the aforementioned two loss:
$$
l = \lambda_1  \cdot l_p + \lambda_2 \cdot  l_c
$$
This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.


%We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning, as shown in Figure \ref{fig:framework} Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input. Such a representation contains all semantics of the input. Next,  we add the contrastive loss into the training procedure while keeping the predictive inpainting loss. This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.

In the following sections, we will show how we apply \name~on both RGB datasets and RF datasets, and extensive experiments shows that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/method-5.tex <==
\section{Information-Preserving Contrastive Learning}
\red{As clearly demonstrated in Section~\ref{sec:RF}, the RF signal is hardly interpretable by humans. When directly applying the prevalent RGB-based unsupervised contrastive learning on the RF modality, it is highly possible to encounter the `shortcut' issue. In RGB-based contrastive learning, this issue can be addressed through deliberately designed data augmentation to break the `shortcut' semantics and learn the desired semantics. However, this solution is infeasible for the RF signals. Due to the non-interpretable property of the RF signals, it is unclear to people which semantic creates which kind of shortcuts and which data augmentation corresponds to which kind of semantics. On the other hand, blindly removing the uncleared `shortcut' may also possibly accidentally remove the real useful semantics. Moreover, when applying the unsupervised pre-trained model to various downstream tasks~\cite{xxx}, some semantics may be a `shortcut' to one task while being useful information to another task. Blindly removing the uncleared `shortcut' during the unsupervised pre-training may benefit some downstream task while hurting the others, thus not be able to generalize well.}

\red{In this case, it is important to learn an unsupervised representation that preserves as much information of the input, and generalizes well to various downstream tasks, even when no prior knowledge of the potential shortcut semantics is available.}


% Previous work has shown that contrastive learning can be easily biased to `shortcut' semantics in the image. Traditional methods  address this bias through data augmentations to break the `shortcut' semantics so that the network will learn the desired semantics. Such a design however suffers from multiple problems:

% \begin{enumerate}
% \item It requires knowing which types of semantics can be shortcut and designing specific augmentations to remove that shortcut. However for modalities like RF, which are not directly interpretable by humans, it is unclear to a human which semantics in the RF signal create a shortcut.  As a result, it is hard to design augmentation techniques to remove the shortcut. 
% \item
% Another problem is that the shortcut semantics can be highly correlated with the useful semantics, in which case it may be impossible to remove the shortcut semantics while keeping those useful semantics untouched. 
% \item
% Last, as shown in \cite{xxx}, there might be multiple types of semantics that are useful for downstream tasks, and one type of them can be a shortcut with respect to one task but a key useful feature for another task. In this case, removing a shortcut might help one downstream task but hurt the other, making it hard to learn a representation that generalizes well to multiple downstream tasks.
% \end{enumerate}

% To address the above problems, we need an unsupervised representation learning method that does not require prior knowledge of the potential shortcut semantics in the data, and can learn a representation that preserves the different semantics in the input, even when one type of semantic information can be a shortcut for contrastive learning. 


\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{framework}
\end{center}
\caption{Illustration of our \name framework. The goal for \name is to train a good encoder network $\theta$ which can encode inputs into a latent space which is useful for various downstream tasks. For the initialization step we only train the network using the predictive loss $l_p$ (blue box). In the full training step we use a combination of predictive loss $l_p$ and contrastive loss $l_c$ to train the network weights.}\label{fig:framework}
\end{figure}


Our idea is to use the task of predicting missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a potential shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By predicting missing patches, we mean predicting randomly cropped regions in the input, e.g., image inpainting. This task has traditionally been used as a pretext task in self-supervised learning. Here however we use it as a regularization of contrastive learning. 

We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning, as shown in Figure \ref{fig:framework}. Our method can be separated to two different branches, one is a common contrastive learning branch which uses random augmentation on same image to generate positive pairs and maximizes similarity between features from them. Another is a missing patch prediction branch which masks out some part of the input and forces the network to reconstruct the missing patches. The goal for \name is to train a good encoder network which could encode input into an embedding space that is useful for various downstream tasks.

Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input, as shown in the blue box on the left. 

\red{Given an input image $x$, we first randomly mask several patches to get the masked input $\mathbb{M}(x)$. Then the masked input is passed through an encoder network $E$ with parameter $\theta$ and a decoder network $D$ with parameter $\delta$ to get the reconstruction result $ D_{\delta}(E_{\theta}(\mathbb{M}(x)))$. The prediction loss $\mathcal{L}_{p}$ is defined as the reconstruction error between the original input $x$ and the reconstructed one $D_{\delta}(E_{\theta}(\mathbb{M}(x)))$:
$$
\mathcal{L}_{p} = ||D_{\delta}(E_{\theta}(\mathbb{M}(x)))-x||_2.
$$}
This will force the representation to contain as much important semantics of the input as possible.

Next, we add the contrastive loss into the training procedure while keeping the predictive inpainting loss as a regularization (both the blue box and the orange box in Figure \ref{fig:framework}). 

\red{As for the contrastive branch, for each image, we first generate a pair of positive samples by using two random augmentations $\tau_1$ and $\tau_2$, then we forward the two augmented inputs seperately into the encoder $E$ parameterized by $\theta$ and a multi-layer nonlinear head $H$ parameterized by $h$ to get the latent representations $z_{1}$ and $z_{2}$ for these two positive samples. We use the commonly used InfoNCE loss \cite{xxx} as the contrastive loss $\mathcal{L}_{c}$. Namely, for a batch of $N$ different input images $x_{i}, i=1,...,N $,}
$$
\mathcal{L}_{c} = -\sum_{i=1}^N \log \sum \frac{\exp\big(\text{sim}(z_{2i}, z_{2i+1})/T\big)}{\sum_{k=1}^{2N} \mathbbm{1}_{k\neq 2i}\exp\big(\text{sim}(z_{2i}, z_k)/T\big)},
$$
\red{where $sim(u,v)=u^{T}v/||u|| ||v||$ denote the dot product between the normalized $u$ and $v$ (i.e., cosine similarity), $T\in \mathbb{R}^{+}$ is a scalar temperature paramete, and $z_{2i},z_{2i+1}$ are the encoded features of positive pairs generated from $x_{i}$, i.e., $z_{2i} = H_h(E_{\theta}(\tau_1(x_{i})))$ and $z_{2i+1} = H_h(E_{\theta}(\tau_2(x_{i})))$.} The overall training loss is the combination of the aforementioned two losses:
$$
\mathcal{L} = \lambda_1  \cdot \mathcal{L}_{p} + \lambda_2 \cdot \mathcal{L}_{c}
$$
This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.


%We propose Predictvie-Contrastive Learning (\name) which combines inpainting with contrastive learning, as shown in Figure \ref{fig:framework} Training in \name\ has an initialization step in which we learn a coarse representation that restores randomly cropped patches in the input. Such a representation contains all semantics of the input. Next,  we add the contrastive loss into the training procedure while keeping the predictive inpainting loss. This forces the network to learn fine-grained high-level semantics while keeping the predictive loss as a regularization so that the contrastive learning will not focus only on some shortcut semantics  and discard other semantics.

In the following sections, we will show how we apply \name~on both RGB datasets and RF datasets, and extensive experiments shows that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/method-6.tex <==
\section{Information-Preserving Contrastive Learning}
 Previous work has shown that contrastive learning can be easily biased to `shortcut' semantics, and addressed this bias through data augmentations that break the `shortcut' semantics so that the network may learn the desired semantics. Such a design however suffers from two problems:
 \begin{enumerate}
 \item It requires knowing which types of semantics can be shortcut and designing specific augmentations to remove that shortcut. However for modalities like RF, which are not directly interpretable by humans, it is unclear to a human which semantics in the RF signal create a shortcut.  As a result, it is hard to design augmentation techniques to remove the shortcut.
% \item
% Another problem is that the shortcut semantics can be highly correlated with the useful semantics, in which case it may be impossible to remove the shortcut semantics while keeping those useful semantics untouched.
 \item
 As shown in \cite{tian2020makes}, there might be multiple types of semantics that are useful for downstream tasks, and one type of them can be a shortcut with respect to one task but a key useful feature for another task. In this case, removing a shortcut might help one downstream task but hurt the other, making it hard to learn a representation that generalizes well to multiple downstream tasks.
 \end{enumerate}

To address the above problems, we need an unsupervised representation learning method that does not require prior knowledge of the potential shortcut semantics in the data, and can learn a representation that preserves the different semantics in the input, even when one type of semantic information can be a shortcut for contrastive learning.


\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-toy}
\end{center}
\caption{Illustration of the \name~framework on RGB data. The framework has two branches: 1) a reconstructive branch, illustrated in the blue box, which ensures that the representation has enough information to restore the missing patches in the input, and 2) a contrastive branch, illustrated in the orange box, which ensures that the representation keeps positive samples close to each other and away from negative samples.}\label{fig:framework}
\end{figure}


Our idea is to use the task of reconstructing missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By reconstructing missing patches, we mean reconstructing randomly cropped regions in the input, (e.g., image inpainting). This task has traditionally been used as a pretext task in self-supervised learning. Here, however, we use it as a regularization of contrastive learning.

We propose Information-Preserving Contrastive Learning (\name), which combines the task of reconstructing missing patches with contrastive learning. In Figure \ref{fig:framework}, we show how we apply \name~to RGB data. Later in Section \ref{sec:rf-exp}, we show how we apply it to RF data. As clear from Figure \ref{fig:framework}, a \name\ model has two branches, one is a common contrastive learning branch which uses random augmentation on the same image to generate positive pairs, and maximizes the similarity between their features (in comparison to the negative pairs). Another is a patch reconstruction branch, which masks out random patches in the input and forces the network to reconstruct the missing patches. The goal of \name is to train a good encoder network that
generates a representation that simultaneously minimizes the contrastive loss and the patch reconstruction loss.


\vskip 0.03in\noindent
{\bf (a) Reconstructive Branch:} The reconstructive branch  is illustrated in the blue box in Figure~\ref{fig:framework}. Given an input image $x$, we first randomly mask several patches to get the masked input $M(x)$. Then the masked input is passed through an encoder network $E$ with parameter $\theta$, and a decoder network $D$, with parameter $\delta$, to obtain the reconstruction result $ D_{\delta}(E_{\theta}(M(x)))$. The reconstruction loss $\mathcal{L}_{r}$ is defined as the reconstruction error between the original input $x$ and the reconstructed one $D_{\delta}(E_{\theta}(M(x)))$:
$$
\mathcal{L}_{r} = ||D_{\delta}(E_{\theta}(M(x)))-x||_2.
$$
The reconstruction branch forces the representation to preserve enough information to reconstruct the missing patches.

\vskip 0.03in\noindent
{\bf (b) Contrastive Branch:} The contrastive branch  is illustrated in the orange box in Figure~\ref{fig:framework}.
For each image, we first generate a pair of positive samples by using two random augmentations $\tau_1$ and $\tau_2$, then we forward the two augmented inputs separately into the encoder $E$ parameterized by $\theta$ and a multi-layer nonlinear projection head $H$ parameterized by $h$ to get the latent representations $z_{1}$ and $z_{2}$ for these two positive samples. We use the commonly used InfoNCE loss \cite{chen2020simple} as the contrastive loss $\mathcal{L}_{c}$. Namely, for a batch of $N$ different input images $x_{i}, i=1,...,N $,
$$
\mathcal{L}_{c} = -\sum_{i=1}^N \log \sum \frac{\exp\big(\text{sim}(z_{2i}, z_{2i+1})/t\big)}{\sum_{k=1}^{2N} \mathbbm{1}_{k\neq 2i}\exp\big(\text{sim}(z_{2i}, z_k)/t\big)},
$$
where $\text{sim}(u,v)=u^{T}v / (\|u\|_2 \|v\|_2)$ denotes the dot product between the normalized $u$ and $v$ (i.e., cosine similarity), $t \in \mathbb{R}^{+}$ is a scalar temperature parameter, and $z_{2i},z_{2i+1}$ are the encoded features of positive pairs generated from $x_{i}$, i.e., $z_{2i} = H_h(E_{\theta}(\tau_1(x_{i})))$ and $z_{2i+1} = H_h(E_{\theta}(\tau_2(x_{i})))$.

\vskip 0.03in\noindent
{\bf (c) Training Procedure:}
We have empirically found that it is better to train the model in two phases. In the first phase, only the reconstructive branch is trained. In the second phase both branches are trained together. In this latter case,
the overall training loss is the combination of the reconstruction loss and the contrastive loss, i.e.:
$$
\mathcal{L} = \lambda_1  \cdot \mathcal{L}_{r} + \lambda_2 \cdot \mathcal{L}_{c}
$$
This forces the network to learn fine-grained high-level semantics while keeping the reconstruction loss as a regularization so that contrastive learning will not focus only on some shortcut semantics and discard other semantics.



%In the following sections, we compare \name's performance with state-of-the-art contrastive learning methods on multiple RGB datasets and RF datasets, and demonstrate via extensive empirical results that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/method-7.tex <==
\input{source/method-ipcl-1}
\input{source/method-rf-1}

==> source/method-ipcl-1.tex <==
\section{Reconstructive Contrastive Learning (\name)}
Reconstructive contrastive learning (\name) is a framework for self-supervised representation learning. It aims to learn representations that are robust to shortcuts, and capable of supporting multiple diverse downstream tasks. \name~aims to provide these properties without knowing a priori the potential shortcuts or the  downstream tasks. 

The key idea underlying \name\ is as follows: Shortcuts are harmful because they cause the features to lose important information that was available in the input. Thus, to counter shortcuts, \name\ uses a reconstructive loss to ensure that the representation can restore the input, i.e., the features have the information available at the input. Yet, keeping all information in the features is not enough; the input already has all information. 
By adding a contrastive loss, \name\ reorganizes the information in the feature space to make it amenable to downstream classification, i.e., 
samples that have similar attributes/objects are closer to each other than samples that have different attributes/objects. Figure \ref{fig:framework} shows the \name\ framework for RGB data, which has two branches: a reconstructive branch and a contrastive branch. 




%Our idea is to use the task of reconstructing missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By reconstructing missing patches, we mean reconstructing randomly cropped regions in the input, (e.g., image inpainting). This task has traditionally been used as a pretext task in self-supervised learning. Here, however, we use it as a regularization of contrastive learning.


%Figure \ref{fig:framework} shows the \name\ framework for RGB data, which has two branches: a contrastive branch,  and a reconstructive branch. 
%one is a common contrastive learning branch, which uses random augmentation on the same image to generate positive pairs, and maximizes the similarity between their features (in comparison to the negative pairs). Another is a reconstructive learning branch, which requires the learned representation to reconstruct the input. 
%\name\ trains a good encoder network that generates a representation that simultaneously minimizes the contrastive loss and the  reconstructive loss.


\begin{figure}
\begin{center}
\vspace{-25pt}
\includegraphics[width=0.98\linewidth]{model-toy}
\vspace{-10pt}
\end{center}
\caption{\footnotesize{Illustration of the \name~framework for RGB data. \name\ has two branches: 1) a reconstructive branch, illustrated in the blue box, which ensures that the representation has enough information to restore missing patches in the input, and 2) a contrastive branch, illustrated in the orange box, which ensures that the representation keeps positive samples close to each other and away from negative samples.}}\label{fig:framework}
\vspace{-20pt}
\end{figure}

{\textbf{(a) Reconstructive Branch:} 
To choose a proper reconstructive task, we need to consider two aspects: its ability to summarize and abstract the input, and its applicability to diverse modalities. In fact, the vast majority of self-supervised learning tasks, such as Auto-encoder, Colorization, Inpainting and Jigsaw Puzzle, are reconstructive since they all aim to restore the input. But, those tasks do not have the same ability to both retain and abstract information.  For example, inpainting is a stronger reconstructive task than autoencoding in terms of its ability to both abstract and retain information. Thus, although both of them would help in strengthening contrastive learning against shortcuts, inpainting is likely to provide more gains. 

Another issue to consider is the  applicability of the chosen task to various modalities. For example, colorization is applicable only to RGB, and Jigsaw does not naturally translate to RF signals.\footnote{There is a complex dependence between the signals in the vertical heatmap and horizontal heatmap, which would be broken if one simply rearrange these voxels.} In contrast, a task like inpainting is easier to translate across modalities by cropping random windows of the signal. 

Given the above considerations, we adopt inpainting as the default reconstructive task.  In the appendix, we compare various reconstructive tasks and show that while they all improve performance, inpainting delivers higher gains and works across modalities.

Figure \ref{fig:framework} shows how \name~uses the inpainting task for RGB data, where given an input image $x$, we first randomly mask several patches to get the masked input $M(x)$. Then the masked input is passed through an encoder network $E$ with parameter $\theta$, and a decoder network $D$, with parameter $\delta$, to obtain the reconstruction result $ D_{\delta}(E_{\theta}(M(x)))$. The reconstruction loss $\mathcal{L}_{r}$ is defined as the reconstruction error between the original input $x$ and the reconstructed one $D_{\delta}(E_{\theta}(M(x)))$:
$$
\mathcal{L}_{r} = ||D_{\delta}(E_{\theta}(M(x)))-x||_2.
$$
%The reconstruction branch forces the representation to preserve enough information to reconstruct the missing patches.

{\bf (b) Contrastive Branch:} The contrastive branch is illustrated in the orange box in Figure~\ref{fig:framework}. Here, we use SimCLR as an example to demonstrate the basic idea. However, this contrastive branch can be easily adapted to any contrastive learning method such as CPC, MoCo, and BYOL. For each image, we first generate a pair of positive samples by using two random augmentations $\tau_1$ and $\tau_2$, then we forward the two augmented inputs separately to the encoder $E$, parameterized by $\theta$ and a multi-layer nonlinear projection head $H$ parameterized by $h$ to get the latent representations $z_{1}$ and $z_{2}$ for these two positive samples. We use the commonly used InfoNCE loss \cite{chen2020simple} as the contrastive loss $\mathcal{L}_{c}$. Namely, for a batch of $N$ different input images $x_{i}, i=1,...,N $,
$$
\mathcal{L}_{c} = -\sum_{i=1}^N \log \sum \frac{\exp\big(\text{sim}(z_{2i}, z_{2i+1})/t\big)}{\sum_{k=1}^{2N} \mathbbm{1}_{k\neq 2i}\exp\big(\text{sim}(z_{2i}, z_k)/t\big)},
$$
where $\text{sim}(u,v)=u^{T}v / (\|u\|_2 \|v\|_2)$ denotes the dot product between the normalized $u$ and $v$ (i.e., cosine similarity), $t \in \mathbb{R}^{+}$ is a scalar temperature parameter, and $z_{2i},z_{2i+1}$ are the encoded features of positive pairs generated from $x_{i}$, i.e., $z_{2i} = H_h(E_{\theta}(\tau_1(x_{i})))$ and $z_{2i+1} = H_h(E_{\theta}(\tau_2(x_{i})))$.

{\bf (c) Training Procedure:}
We have empirically found that it is better to train the model in two phases. In the first phase, only the reconstructive branch is trained. In the second phase, both branches are trained together. In this latter case,
the overall training loss is the combination of the reconstruction loss and the contrastive loss, i.e., $\mathcal{L} = \lambda_1  \cdot \mathcal{L}_{r} + \lambda_2 \cdot \mathcal{L}_{c}$.

%This forces the network to learn fine-grained high-level semantics while keeping the reconstruction loss as a regularization so that contrastive learning will not focus only on some shortcuts and discard other semantics.




==> source/method-ipcl.tex <==
\section{Information-Preserving Contrastive Learning}
 Previous work has shown that contrastive learning can be easily biased to `shortcut' semantics, and addressed this bias through data augmentations that break the `shortcut' semantics so that the network may learn the desired semantics. Such a design however suffers from two problems:
 \begin{enumerate}
 \item It requires knowing which types of semantics can be shortcut and designing specific augmentations to remove that shortcut. However for modalities like RF, which are not directly interpretable by humans, it is unclear to a human which semantics in the RF signal create a shortcut.  As a result, it is hard to design augmentation techniques to remove the shortcut.
% \item
% Another problem is that the shortcut semantics can be highly correlated with the useful semantics, in which case it may be impossible to remove the shortcut semantics while keeping those useful semantics untouched.
 \item
 As shown in \cite{tian2020makes}, there might be multiple types of semantics that are useful for downstream tasks, and one type of them can be a shortcut with respect to one task but a key useful feature for another task. In this case, removing a shortcut might help one downstream task but hurt the other, making it hard to learn a representation that generalizes well to multiple downstream tasks.
 \end{enumerate}

To address the above problems, we need an unsupervised representation learning method that does not require prior knowledge of the potential shortcut semantics in the data, and can learn a representation that preserves the different semantics in the input, even when one type of semantic information can be a shortcut for contrastive learning.


\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-toy}
\end{center}
\caption{Illustration of the \name~framework on RGB data. The framework has two branches: 1) a reconstructive branch, illustrated in the blue box, which ensures that the representation has enough information to restore the missing patches in the input, and 2) a contrastive branch, illustrated in the orange box, which ensures that the representation keeps positive samples close to each other and away from negative samples.}\label{fig:framework}
\end{figure}


%Our idea is to use the task of reconstructing missing patches in the input as a regularization of contrastive learning to force it to learn multiple types of semantics, even in the presence of a shortcut, and without requiring the designer to know which information in the input may create a shortcut.  By reconstructing missing patches, we mean reconstructing randomly cropped regions in the input, (e.g., image inpainting). This task has traditionally been used as a pretext task in self-supervised learning. Here, however, we use it as a regularization of contrastive learning.

We propose Information-Preserving Contrastive Learning (\name), which combines reconstructive learning with contrastive learning. In Figure \ref{fig:framework}, we show an example of how we apply \name~to RGB data. As clear from Figure \ref{fig:framework}, a \name\ model has two branches, one is a common contrastive learning branch which uses random augmentation on the same image to generate positive pairs, and maximizes the similarity between their features (in comparison to the negative pairs). Another is a reconstructive learning branch, which requires the learned representation to reconstruct the input. In the case of RGB data, we masks out random patches in the input and forces the network to reconstruct the missing patches. The goal of \name is to train a good encoder network that
generates a representation that simultaneously minimizes the contrastive loss and the  reconstructive loss.


\vskip 0.03in\noindent
{\bf (a) Reconstructive Branch:} The reconstructive branch  is illustrated in the blue box in Figure~\ref{fig:framework}. Given an input image $x$, we first randomly mask several patches to get the masked input $M(x)$. Then the masked input is passed through an encoder network $E$ with parameter $\theta$, and a decoder network $D$, with parameter $\delta$, to obtain the reconstruction result $ D_{\delta}(E_{\theta}(M(x)))$. The reconstruction loss $\mathcal{L}_{r}$ is defined as the reconstruction error between the original input $x$ and the reconstructed one $D_{\delta}(E_{\theta}(M(x)))$:
$$
\mathcal{L}_{r} = ||D_{\delta}(E_{\theta}(M(x)))-x||_2.
$$
The reconstruction branch forces the representation to preserve enough information to reconstruct the missing patches.

\vskip 0.03in\noindent
{\bf (b) Contrastive Branch:} The contrastive branch  is illustrated in the orange box in Figure~\ref{fig:framework}.
For each image, we first generate a pair of positive samples by using two random augmentations $\tau_1$ and $\tau_2$, then we forward the two augmented inputs separately into the encoder $E$ parameterized by $\theta$ and a multi-layer nonlinear projection head $H$ parameterized by $h$ to get the latent representations $z_{1}$ and $z_{2}$ for these two positive samples. We use the commonly used InfoNCE loss \cite{chen2020simple} as the contrastive loss $\mathcal{L}_{c}$. Namely, for a batch of $N$ different input images $x_{i}, i=1,...,N $,
$$
\mathcal{L}_{c} = -\sum_{i=1}^N \log \sum \frac{\exp\big(\text{sim}(z_{2i}, z_{2i+1})/t\big)}{\sum_{k=1}^{2N} \mathbbm{1}_{k\neq 2i}\exp\big(\text{sim}(z_{2i}, z_k)/t\big)},
$$
where $\text{sim}(u,v)=u^{T}v / (\|u\|_2 \|v\|_2)$ denotes the dot product between the normalized $u$ and $v$ (i.e., cosine similarity), $t \in \mathbb{R}^{+}$ is a scalar temperature parameter, and $z_{2i},z_{2i+1}$ are the encoded features of positive pairs generated from $x_{i}$, i.e., $z_{2i} = H_h(E_{\theta}(\tau_1(x_{i})))$ and $z_{2i+1} = H_h(E_{\theta}(\tau_2(x_{i})))$.

\vskip 0.03in\noindent
{\bf (c) Training Procedure:}
We have empirically found that it is better to train the model in two phases. In the first phase, only the reconstructive branch is trained. In the second phase both branches are trained together. In this latter case,
the overall training loss is the combination of the reconstruction loss and the contrastive loss, i.e.:
$$
\mathcal{L} = \lambda_1  \cdot \mathcal{L}_{r} + \lambda_2 \cdot \mathcal{L}_{c}
$$
This forces the network to learn fine-grained high-level semantics while keeping the reconstruction loss as a regularization so that contrastive learning will not focus only on some shortcut semantics and discard other semantics.



%In the following sections, we compare \name's performance with state-of-the-art contrastive learning methods on multiple RGB datasets and RF datasets, and demonstrate via extensive empirical results that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/method-rf-1.tex <==
\section{Adapting \name~to Radio Signals}
To show how \name\ deals with uninterpretable modalities, we adapt it to learn representations from unlabeled radio frequency (RF) signals. 
%
%Labeling RF signals is difficult since they cannot be directly interpreted by human labelers. Past work labels RF signals by deploying a multi-camera system synchronized with the RF device, which is labor-intensive and unscalable. If RF representations can be learned without supervision, it significantly reduces overhead.
%
%\subsection{Overview of Human Sensing using RF Signals}
%Radio Frequency (RF) signals have been studied a lot recently for pose estimation, action recognition, and person re-identification \cite{zhao2018through,zhao2018rf,li2019making,chetty2017low,zhang2018latern,fan2020home,zhao2019through,adib2015capturing,vasisht2018duet,tian2018rf,zhao2016emotion,zhao2017learning,hsu2019enabling,fan2020learning}, mainly due to its good properties that it can traverse occlusions and are insensitive to visible light. Therefore, these tasks can be performed through walls and in dark settings where RGB-based cameras fail. However, past works on these tasks are based on supervised learning using labeled RF datasets. 
%
RF signals have recently attracted much attention for their ability to sense humans through walls and occlusions~\cite{zhao2018through,zhao2018rf,li2019making,chetty2017low,zhang2018latern,fan2020home,zhao2019through,adib2015capturing,vasisht2018duet,tian2018rf,zhao2016emotion,zhao2017learning,hsu2019enabling,fan2020learning}, Here, 
we adapt \name\ to learn self-supervised representations for the following tasks:
\begin{Itemize}
\vspace{-5pt}
\item (a) RF-Based 3D Pose Estimation~\cite{zhao2018through,zhao2018rf}, which uses RF signals to infer the 3D locations of 14 keypoints on the human body including head, neck, shoulders, arms, wrists, hip, knees, and feet.
\item (b) RF-Based action recognition~\cite{li2019making}, which analyzes radio signals to infer human actions and interactions in the presence of occlusions and in poor lighting. 
\item (b) RF-Based Re-Id~\cite{fan2020home}, which recognizes a person-of-interest across different places and times by analyzing the radio signals that bounce off their bodies. 
\vspace{-5pt}
\end{Itemize}

%Before delving into the details of our unsupervised representation learning framework, we first explain the typical neural models used in these tasks. 
In all of these tasks, the input is a time sequence of RF frames. Each RF frame is a pair of  2D heatmaps: one horizontal heatmap and one vertical heatmap, as illustrated in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio signals on a plane parallel to the ground, and the vertical heatmap is a projection of the radio signals on a plane perpendicular to the ground. There are typically 30 pairs of heatmaps per second.
% i.e., 30 RF frames per second.



\begin{figure}[t]
\includegraphics[width=\linewidth]{rf-framework}
\centering
\vskip -0.15in
\caption{\footnotesize{RF-based human sensing framework. The RF heatmaps are first fed to a Feature Network to extract spatio-temporal features, and ROI Align with the given bounding box is used to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}}\label{fig:rf-framework}
\vspace{-0pt}
\end{figure}

%\begin{wrapfigure}{r}{70mm}
\begin{figure}[t]
\centering
\includegraphics[width=.9\linewidth]{rf-heatmaps}
\vspace{-10pt}
\caption{\footnotesize{Illustration of RF signals as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}}\label{fig:rf-heatmaps}
\vspace{-0pt}
\end{figure}


\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.95\linewidth]{model-rf}
\end{center}
\vspace{-15pt}
\caption{\footnotesize{\name~on RF signals.  For the reconstructive branch, we randomly mask some RF frames. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and then use ROI Align with the given bounding box to crop out regions containing humans. The reconstructive branch has a decoder to reconstruct inputs, while the contrastive branch has a non-linear projection head to generate normalized features. The combination of reconstruction loss and contrastive loss is used to train the model.}}
\label{fig:model-rf}
\vspace{-10pt}
\end{figure*}


The models used in RF-based sensing tasks have the general structure in Figure~\ref{fig:rf-framework}. The model first uses a spatio-temporal convolutional feature network to extract features from the input RF frames. It then crops out a bounding box around the person in the feature map. Finally, the cropped features are fed to a task-specific sub-network to generate frame-level features. The high-level structure is the same for all tasks, but different tasks have different sub-networks specifically designed for that task. 

\subsection{\name~for RF Signals}
To apply \name\ to RF signals, we use the network in Figure \ref{fig:model-rf}. The reconstructive task predicts missing RF frames. Specifically, for each RF sequence consisting of 100 RF frames, we randomly mask out 25 frames within this sequence and fill them with zeros. The reconstructive task reconstructs the original RF sequence using the learned feature. For contrastive learning, as shown in Figure \ref{fig:model-rf}, the anchor and positive sample share the same input RF frames with different random jitter of the bounding boxes. Frames that are within 0.3 seconds of the anchor frame serve as positive samples. Negative samples of an anchor are all samples in the batch except for itself and its positive sample. 

During the unsupervised learning phase, a spatio-temporal RF feature extraction network, the same as the feature network in Figure \ref{fig:rf-framework}, is used to encode the input RF frames. Then an ROI Align is applied to the extracted features to crop out the person, where the bounding boxes are generated using the WiTrack localization algorithm \cite{adib20143d}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual blocks and 2 fully-connected layers is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the reconstruction task, a decoder is added to reconstruct the masked RF frames, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed RF  and the ground truth RF frames. We then combine these two losses together as $ \lambda_1  \cdot \mathcal{L}_{r} + \lambda_2 \cdot \mathcal{L}_{c}$.

==> source/method-rf.tex <==
\section{Adapting \name~to RF Signals}
Radio Frequency (RF) signals have been studied a lot recently for pose estimation, action recognition, and person re-identification \cite{zhao2018through,zhao2018rf,li2019making,chetty2017low,zhang2018latern,fan2020home,zhao2019through,adib2015capturing,vasisht2018duet,tian2018rf,zhao2016emotion,zhao2017learning,hsu2019enabling,fan2020learning}, mainly due to its good properties that it can traverse occlusions and are insensitive to visible light. Therefore, these tasks can be performed through walls and in dark settings where RGB-based cameras fail. However, past works on these tasks are based on supervised learning using labeled RF datasets. 
Since RF signals are not interpretable by a human, the annotation is collected by deploying a camera system and synchronizing it with the RF device, which is labor-intensive and hard to scale.  If we can learn useful representation from unlabeled RF signals,  we can reduce overhead and improve the accuracy of the downstream tasks. 


% Radio Frequency (RF) signals have been used for pose estimation, action recognition, and person re-identification \cite{xx,xx,xx}.   Further, since RF signals can traverse occlusions and are insensitive to visible light,  these three tasks can be performed through walls and in dark settings. However, past works on these tasks are based on supervised learning using labeled RF datasets. We would like to demonstrate the possibility of improving accuracy on these tasks by learning useful representations from unlabeled RF signals.


%In this section, we adapt IPCL to learn useful representations from unlabeled RF signals.  We would like the learned representation to be useful for the following three downstream tasks:
%\begin{Itemize}
%\item (a) RF-Based 3D Pose Estimation~\cite{xxx}, which uses radio signals to infer the 3D locations of 12 keypoints on the human body that denote the head, shoulders, arms, wrists, hip, knees, and feet.
%\item (b) RF-Based action recognition~\cite{xxx}, which analyses radio signals to infer human actions and interactions in the presence of occlusions and in poor lighting conditions. 
%\item (b) RF-Based ReId~\cite{xxx}, which recognizes a person-of-interest across different places and times by analyzing the radio signals that bounce off their bodies. 
%\end{Itemize}

Before delving into the details of our unsupervised representation learning framework, we first explain the typical neural models used in these tasks. For all of these tasks, the input is a time sequence of RF frames. Each RF frame is a pair of  2D heatmaps: one horizontal heatmap and one vertical heatmap, as illustrated in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio signals on a plane parallel to the ground, and the vertical heatmap is a projection of the radio signals on a plane perpendicular to the ground. There are typically 30 pairs of heatmaps per second.
% i.e., 30 RF frames per second.

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-heatmaps}
\end{center}
\vspace{-5pt}
\caption{Illustration of RF signals as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}\label{fig:rf-heatmaps}
\vspace{-5pt}
\end{figure}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{rf-framework}
\end{center}
\caption{RF-based human sensing framework. The RF heatmaps are first fed into a Feature Network to extract spatio-temporal features, and ROI Align with the given bounding box is used to crop out the regions with humans. Each downstream task has a unique sub-network to extract task-specific features and predictions.}\label{fig:rf-framework}
\end{figure}

\begin{figure*}[t]
\begin{center}
\includegraphics[width=\linewidth]{model-rf}
\end{center}
\caption{\name~on RF signals. It has two branches: Reconstructive Branch and Contrastive Branch. For the reconstructive branch, we randomly mask some frames across time for reconstruction. For the contrastive branch, different transformation $\tau_1$ and $\tau_2$ to the bounding box are adopted to generate positive samples. Both branches share the same feature extraction network (Green Box), and then use ROI Align with the given bounding box to crop out regions containing humans. The reconstructive branch has a decoder to reconstruct inputs, while contrastive branch has a non-linear projection head to generate normalized features. The combination of reconstruction loss and contrastive loss is used to train the model.}\label{fig:model-rf}
\end{figure*}


The models used in RF-based human sensing tasks (e.g., pose estimation, action recognition, and person re-identification) have the general structure in Figure~\ref{fig:rf-framework}. The model first uses a spatio-temporal convolutional feature network to extract features from the input RF frames. It then crops out a bounding box around the person in the feature map. Finally, the cropped features are fed into a task-specific sub-network to generate frame-level features for downstream tasks. The high-level structure is the same for all tasks, but different tasks have different sub-networks specifically designed for that task. The goal of RF-based unsupervised representation learning is to learn a feature extraction network that can extract both informative and fine-grained features from input RF frames for different downstream tasks.

To apply \name~on RF signals, we design a framework shown in Figure \ref{fig:model-rf}. We design the reconstructive task to be predicting missing frames from a sequence of RF signals. Specifically, for each RF sequence consisting of 100 RF frames, we randomly mask out 25 frames within this sequence and fill them with zero. The reconstructive task is to reconstruct the original RF sequence using the learned feature. For the contrastive learning, as shown in Figure \ref{fig:model-rf}, the anchor and positive sample share the same input RF frames with different random jitter of the bounding boxes. Frames that are within 0.3 seconds of the anchor frame also serves as positive samples. Negative samples of an anchor are all other samples in the batch except for itself and its positive sample. 

During the unsupervised learning phase, a spatio-temporal RF feature extraction network same as the feature network in Figure \ref{fig:rf-framework} is used to encode the input RF frames. Then an ROI Align is applied on top of the extracted features to crop out the region around the person, where the region of interest bounding boxes come from the WiTrack localization algorithm \cite{adib20143d}. For contrastive learning, a non-linear projection head consisting of 3 convolutional residual block and 2 fully-connected layers is added on top of the cropped feature maps to project the features and apply the contrastive loss $l_P$ between features from positive and negative samples. For the reconstruction task, a decoder is added to reconstruct the masked RF frames, and a per-pixel reconstruction loss $l_C$ is added between the reconstructed RF  and the ground truth RF frames. We then combine these two losses together as $\lambda_1\cdot l_P + \lambda_2\cdot l_C$.

==> source/method.tex <==
\section{Method}

\subsection{Winner-Takes-All Theorem of Contrastive Learning}
In this section, we claim and prove the Winner-Takes-All Theorem of Contrastive Learning, i.e., that the global minimum of contrastive training on multiple semantics will be the same as the global minimum of contrastive training on just one of those semantics (the winner). We assume that during contrastive training on a target set of semantics, the target semantics between anchor and positive samples are the same while the semantics between anchor and negative samples are different. Formally, we define the similarity loss of contrastive learning as follows:

\begin{definition}[Similarity Loss] 
	
We define the similarity loss of a neural network with parameter $\pi$ for a set of $n$ different semantics on dataset $X$ as follows
$$L_A(X | \pi) = \frac{\sum\limits_{x_i, x_j\in X} \sigma_A(x_i, x_j)\frac{\pi(x_i)\cdot\pi(x_j)}{|\pi(x_i)||\pi(x_j)|}}{N_A}, A = \{1, \cdots, n\}$$ 
where 
\begin{equation}
  \sigma_A(x_i, x_j) =
    \begin{cases}
      1 & \text{if $k$-th semantics of $x_i$ and $x_j$ are the same , $\forall k\in A$}\\
      -1 & \text{if $k$-th semantics of $x_i$ and $x_j$ are different, $\forall k\in A$}\\
      0 & \text{otherwise}
    \end{cases}     
\end{equation}
$$    N_A=\sum\limits_{x_i, x_j\in X} |\sigma_A(x_i, x_j)|  $$

\end{definition}

Note that there are two different semantics here: semantics in the input and semantics in the feature. The semantics in the feature is a subset of semantics in the input. Moreover, on global minimum of contrastive learning, the semantics in the feature become those semantics shared between positive samples and varied between negative samples.

\begin{definition}[Orthogonal Semantics] 
Suppose a neural network $\pi$'s features of input $X$ forms a space $S(X|\pi)$. Then the $i$-th semantic in the feature forms a subspace of $S(X|\pi)$, denoted as $S_i(X|\pi)$ with orthonormal basis $v^i_1, \cdots, v^i_{n_i}$. We define the $i$-th and $j$-th semantics are orthogonal in the feature space of $\pi$ iff $S_i$ and $S_j$ are orthogonal subspaces, i.e., $\forall k, l, v^i_k \cdot v^j_l = 0.$ Moreover, we define the $i$-th and $j$-th semantics are orthogonal if they are orthogonal in the feature space of $\pi_i^*, \pi_j^*$ and $\pi_{i,j}^*$, where $\pi_i^*$ achieves the global minimum of $L_i$, $\pi_j^*$ achieves the global minimum of $L_j$, and $\pi_{i,j}^*$ achieves the global minimum of $L_{i, j}$.

\end{definition}

\begin{lemma}\label{lem:lem1}
If two semantics are orthogonal, then the corresponding similarity loss on each of them $L_1$ and $L_2$ has the following property: 
$$L_1(X|\underset{\pi}{\arg\min}L_2(X|\pi)) = \text{random},$$
$$L_2(X|\underset{\pi}{\arg\min}L_1(X|\pi)) = \text{random},$$
$$\text{ if } L_2(X|\pi) \text{ not random}, L_1(X|\pi) > \min\limits_\pi L_1(X|\pi)$$
$$\text{ if } L_1(X|\pi) \text{ not random}, L_2(X|\pi) > \min\limits_\pi L_2(X|\pi).$$ I.e., learning features for the first semantic will not help learning the second one but only consumes network capacity thus harms learning it, and vice versa.
\end{lemma}

\begin{theorem}[Winner-Takes-All theorem of contrastive learning]\label{theo:winner}
	
Given two orthogonal semantics, the global minimum of the loss of the contrastive learning on both semantics $\min\limits_\pi L_{1, 2}(X|\pi)$ is equal to $\min\limits_i\min\limits_\pi L_{i}(X|\pi)$.
\end{theorem}

\begin{proof}
Suppose $\pi^*$ is the global minimum parameter for contrastive learning on the two semantics, $\pi_1^*$ is the global minimum parameter for contrastive learning on the first semantic, and $\pi_2^*$ is the global minimum parameter for contrastive learning on the second semantic.
We first prove that 
$$\min(L_{1}(X|\pi_1^*), L_{2}(X|\pi_2^*)) \leqslant L_{1, 2}(X|\pi^*).$$
	 Since the two semantics are orthogonal for $\pi^*$, we can find orthonormal basis $v^{1}_1, \cdots, v^{1}_{n_1}$ and $v^{2}_1, \cdots, v^{2}_{n_2}$ for orthogonal subspaces $S_{1}(X|\pi^*)$ and $S_{2}(X|\pi^*)$ respectively. Since there are only these two semantics in the feature space, $v^{1}_1, \cdots, v^{1}_{n_1}, v^{2}_1, \cdots, v^{2}_{n_2}$ are one orthonormal basis for the whole feature space $S(X|\pi^*)$, and each $\pi^*(x)$ can be represented by $\pi_{1}(x)+\pi_{2}(x)$, where $\pi_{1}, \pi_{2}$ are networks whose feature space are $S_{1}(X|\pi^*)$ and $S_{2}(X|\pi^*)$. We assume that $\forall x \in X, \frac{|\pi_{1}(x)|}{|\pi(x)|}=c_1, \frac{|\pi_{2}(x)|}{|\pi(x)|}=c_2, c_1^2+c_2^2=1$. Then
\\
\begin{gather}
\begin{aligned}\label{eq:eq2}
	&L_{1, 2}(X | \pi) \cdot N_{1, 2}= \sum_{x_i, x_j\in X} \sigma_{1, 2}(x_i, x_j)\frac{\pi^*(x_i)\cdot\pi^*(x_j)}{|\pi^*(x_i)||\pi^*(x_j)|}\\
	&= \sum_{x_i, x_j\in X} \sigma_{1,2}(x_i, x_j)\frac{(\pi_{1}(x_i)+\pi_{2}(x_i))\cdot(\pi_{1}(x_j)+\pi_{2}(x_j))}{{|\pi^*(x_i)||\pi^*(x_j)|}}\\
	&= \sum_{x_i, x_j\in X} \sigma_{1,2}(x_i, x_j)(\frac{\pi_{1}(x_i)\cdot\pi_{1}(x_j)}{{|\pi^*(x_i)||\pi^*(x_j)|}}+\frac{\pi_{2}(x_i)\cdot\pi_{2}(x_j)}{|\pi^*(x_i)||\pi^*(x_j)|}) \\
	&=c_1^2\sum_{x_i, x_j\in X} \sigma_{1,2}(x_i, x_j)\frac{\pi_{1}(x_i)\cdot\pi_{1}(x_j)}{|\pi_{1}(x_i)||\pi_{1}(x_j)|}\\
	&\quad +c_2^2\sum_{x_i, x_j\in X}\sigma_{1,2}(x_i, x_j)\frac{\pi_{2}(x_i)\cdot\pi_{2}(x_j)}{|\pi_{2}(x_i)||\pi_{2}(x_j)|}
	\end{aligned}
\end{gather}
\\
Note that 
\begin{gather}
\begin{aligned}\label{eq:eq3}
	L_{1}(X | \pi_{1}) &= \frac{\sum\limits_{x_i, x_j\in X} \sigma_{1}(x_i, x_j)\frac{\pi_{1}(x_i)\cdot\pi_{1}(x_j)}{|\pi_{1}(x_i)||\pi_{1}(x_j)|}}{N_{1}}\\
	&\approx \frac{\sum\limits_{x_i, x_j\in X} \sigma_{1, 2}(x_i, x_j)\frac{\pi_{1}(x_i)\cdot\pi_{1}(x_j)}{|\pi_{1}(x_i)||\pi_{1}(x_j)|}}{N_{1, 2}}\\
	&=L_{1, 2}(X|\pi_{1})
\end{aligned}
\end{gather}
\\
This is because $\pi_{1}(x)$ only contains information about the first semantic. Therefore, no matter the positive and negative input samples share the same second semantic or not, it will not affect the performance of $\pi_{1}(x)$ on the contrastive loss. Similar approximation also holds for $L_{2}(X|\pi_{2})$.

Combining Equation \ref{eq:eq2} and Equation \ref{eq:eq3}, we can get 
$$L_{1, 2}(X | \pi^*) \approx c_1^2 L_{1}(X|\pi_{1}) + c_2^2 L_{2}(X|\pi_{2}).$$
Since $c_1^2+c_2^2 = 1$, we have 
\begin{gather}
	\begin{aligned}
	\min(L_{1}(X|\pi_1^*), L_{2}(X|\pi_2^*))&\leqslant \min(L_{1}(X|\pi_{1}), L_{2}(X|\pi_{2}))\\
	&\leqslant L_{1, 2}(X|\pi^*).
	\end{aligned}
\end{gather}


We then prove that 
$$\min(L_{1}(X|\pi_1^*), L_{2}(X|\pi_2^*)) \geqslant L_{1, 2}(X|\pi^*).$$
Without loss of generality, assume $L_{1}(X|\pi^*_{1}) \leqslant L_{2}(X|\pi^*_{2}$). Then
$$  L_{1}(X|\pi^*_{1}) = L_{1, 2}(X|\pi^*_{1})\geqslant L_{1, 2}(X|\pi^*) $$
The left equity comes from Equation \ref{eq:eq3} since $\pi_{1}^*$ will not contain information about the second semantic (Lemma \ref{lem:lem1}). 

Therefore, $\min\limits_\pi L_{1, 2}(X|\pi)=\min\limits_i\min\limits_\pi L_{i}(X|\pi)$
 
\end{proof}

%\begin{corollary} 
%
%If two mutual information $I_1$ and $I_2$ are orthogonal, the winner of the mutual information will take all capacity of the network to learn the easiest information and ignore the others.
%
%\end{corollary}


\subsection{Predictive-Contrastive Learning}
From the above theorem, we know that if we perform contrastive learning on a dataset where multiple semantics between anchor and positive sample are the same, then contrastive learning is likely to only learn the easiest semantic to achieve minimum contrastive loss. This phenomenon is also proved later by our experiments on Colorful-MNIST dataset. On the other hand, predictive unsupervised learning will preserve as much information about the input in the learnt representation as possible because this representation will bee used to reconstruct the original input. However, predictive learning typically fails to learn those high-level semantic features but focus more on low-level patterns in the input. 

To solve these problems, we propose Predictvie-Contrastive Learning (PCL) to combine the advantage of both methods. More specifically, we first use predictive learning to learn a coarse representation of the input that contains all semantics of the input. Then we add the contrastive loss into the training which force the network to learn fine-grained high-level semantics while keep the predictive loss as a regularization so that the contrastive learning will not discard any of the semantics. In the following sections, we will show how we apply \name~on both a hand-crafted image dataset and real-world RF datasets, and extensive experiments shows that \name~is effective in learning a high-quality representation containing multiple semantics that can be used for different downstream tasks.


==> source/related-1.tex <==
\section{Related Work}

\noindent{\bf (a) Unsupervised Contrastive Representation Learning: }
Early work on unsupervised representation learning has focused on designing pretext tasks and training the network to predict their pseudo labels. Such tasks include solving jigsaw puzzles \cite{noroozi2016unsupervised}, restoring a missing patch in the input \cite{pathak2016context}, or predicting image rotation \cite{gidaris2018unsupervised}. However, pretext tasks have to be handcrafted,  and the generality of their representations is typically limited~\cite{chen2020simple}.

Hence, researchers have recently focused on contrastive learning, which emerged as a competitive and systematic method for learning effective representations without human supervision. The learned features generalize well to downstream tasks, outperform representations learned through pretext tasks, and even surpass the performance of supervised models on some tasks \cite{chen2020simple,chen2020big,chen2020improved,he2020momentum}. Multiple successful contrastive learning frameworks have been proposed, which typically differ in the way they sample negative pairs. To name a few, SimCLR \cite{chen2020simple} uses a large batch size, and samples negative pairs within each batch. The momentum-contrastive approach (MoCo) \cite{he2020momentum} leverages a moving-average encoder and a queue to generate negative samples on the fly during training.  Contrastive-Multiview-Coding \cite{tian2019contrastive} maintains a memory-bank to store features and generate negative samples. Some recent methods, like BYOL, do not rely on negative pairs \cite{chen2020exploring,grill2020bootstrap}. Instead, they use two neural networks that learn from each other to boost performance.

Past work has also reported problems with contrastive learning. The authors of \cite{chen2020simple} showed that color distribution can be a shortcut and proposed to break this shortcut through color-distortion data augmentation. Further, the authors of \cite{tian2020makes} noted that when the data includes multiple types of semantics, one type may produce a shortcut that prevents contrastive learning from learning effective features of other semantics (as in Figure~\ref{fig:intro}(b) where the background object information can be a shortcut that prevents learning features related to digits).  They proposed a solution that learns contrastive views suitable for the desired downstream task. While they share our goal of supporting different downstream tasks, their method requires supervision since they learn their contrastive views from labeled data. In contrast, our representation learning is completely unsupervised. 
 
Another related work is contrastive-predictive-coding (CPC) \cite{oord2018representation,henaff2019data}. 
CPC has some similarity with \name~in that it has a predictive task that aims to reconstruct missing information. However, CPC aims to reconstruct the features of a future frame, while \name~reconstructs the raw input data. As a result,  the representation learned by CPC is not forced to contain necessary information to reconstruct the input, making it susceptible to shortcuts, just like other contrastive learning methods.

\noindent{\bf (b) Autoencoders (AE): } The family of auto-encoders provides  a popular framework for self-supervised representation learning using a reconstructive loss~\cite{hinton2006reducing,pu2016variational,vincent2008extracting}. It trains an encoder to generate low-dimensional latent codes that could reconstruct the entire high-dimensional inputs. There are many types of AEs, such as denoising auto-encoders \cite{vincent2008extracting}, which corrupt the input and let the latent codes reconstruct it, and variational auto-encoders \cite{pu2016variational}, which force the latent codes to follow a prior distribution. In fact, {\name} can be viewed as a special variant of the denoising auto-encoder that forces the latent codes to have a `contrastive' property regularized by a contrastive loss. As a result, the latent codes, not only are good for reconstructing the input, but also are good for downstream classification tasks. 



%However, contrastive learning could potentially bias to the training dataset. (cite infoMin paper).
\vskip 0.03in
\noindent{\bf (c) Learning from Radio Signals: }
There is a growing literature that uses radio signals for pose estimation, action recognition, captioning, and re-identifications through walls and occlusions~\cite{zhao2018through,zhao2018rf,zhao2019through, wang2019person,li2019making,chetty2017low,zhang2018latern,fan2020home,fan2020learning,hsu2019enabling,vasisht2018duet}. Past work however relies on supervised learning. Given the difficulty of annotating RF datasets with ground truth labels for pose or actions, past work is limited to relatively small datasets, which hampers its performance.  Our work allows these models to leverage large amounts of unannotated radio signals to improve the performance of their downstream tasks. 




==> source/related.tex <==
\section{Related Work}

\subsection{Unsupervised Representation Learning}
Unsupervised representation learning refers to learning useful representations of data that effectively capture certain labels of interest, and doing so without human supervision. Early work in this area has focused on designing pretext tasks and training the network to predict the pseudo labels for those tasks. Such tasks include solving Jigsaw Puzzles \cite{noroozi2016unsupervised}, filling a missing patch in the input \cite{pathak2016context}, or predicting image rotation \cite{gidaris2018unsupervised}. However, pretext tasks have to be handcrafted,  and the generality of their representations is typically limited~\cite{chen2020simple}.
 
Recently, contrastive unsupervised learning has emerged as a highly competitive method for learning features from visual datasets. The learnt features generalize to different downstream tasks, outperform representations learned through handcrafted pretext tasks by a large margin, and even surpass the performance of supervised models on some tasks. Instead of designing a pretext task, contrastive learning approaches learn representations by contrasting positive samples against negative samples. Different approaches typically differ in the way they sample positive and negative pairs. For generating positive pairs, a standard method is to create multiple variants of a datapoint using data augmentation \cite{chen2020improved,he2020momentum,chen2020simple,chen2020big}. There are also multiple ways of generating negative pairs. To name a few, SimCLR \cite{chen2020simple} uses a large batch-size, and samples negative pairs within each batch. Momentum-Contrastive approach \cite{he2020momentum} leverages a moving-average encoder and a queue to generate negative samples on-the-fly during training. Other approaches like Contrastive-Multiview-Coding \cite{tian2019contrastive} maintain a memory-bank to store features, and generate negative samples from this memory bank.

Despite the effectiveness of contrastive representation learning, previous work also shows that contrastive learning can be easily biased to focus on simple and potentially irrelevant 'shortcuts'. For example, \cite{chen2020simple} showed that color distribution can be a shortcut to distinguish two patches cropped from the same image, from two patches from different images. Past work addresses this problem by adding data augmentations to break the 'shortcut' semantics, so that the network may learn the desired semantics. Past work also shows that, when multiple factors are presented in an image, contrastive learning tends to learn semantics related to one factor and ignore the others \cite{tian2020makes}. For example, if the positive samples share multiple types of semantic information (e.g., digit and background), one factor can easily overwhelm the other factors (e.g., the representation will learn the shared background but not the same digit).


To the best of our knowledge, there is no existing work combining contrastive learning with the task of predicting a missing patch in the input. One work that seems to be close to ours is contrastive-predictive-coding (CPC) \cite{oord2018representation}, which leverages an RNN structure to predict latent features in the future. The positive samples of CPC are typically features at a certain time step, and features from all other time steps serve as negative samples. The key difference between CPC and our method is that the prediction target of CPC is the feature of a future frame, while the prediction target of our method is the raw input signal. As a result, the representation learnt by CPC is not forced to contain necessary information to reconstruct the input, making it also likely to be bias to one type of semantics, just like other contrastive learning methods.

%However, contrastive learning could potentially bias to the training dataset. (cite infoMin paper).


\subsection{Learning from Radio Signals}
There is a growing body of literature that leverages radio signals to learn pose estimation, action recognition, captioning, and re-identifications  through walls and occlusions~\cite{zhao2018through,zhao2018rf,li2019making,chetty2017low,zhang2018latern,fan2020home,fan2020learning,zhao2019through,hsu2019enabling,vasisht2018duet,tian2018rf}. All of this work however relies on supervised learning from annotated data. Given the difficulty of annotating RF datasets with ground truth labels for pose or actions, past work is limited to relatively small datasets which hampers its performance.  Our work allows these models to benefit from large amounts of unannotated RF signals to improve performance and their  downstream tasks. 




==> source/rf.tex <==
\section{RF Preliminary}
Past work on learning from RF signals typically uses multi-antenna FMCW radios \cite{li2019making,lien2016soli,zhao2018through,zhao2018rf,fan2020home,fan2020learning,zhao2019through,peng2016fmcw,chetty2017low,zhang2018latern,hsu2017extracting,hsu2019enabling,zhao2016emotion,zhao2017learning}. Thus, we use a similar radio based on FMCW that operates in the frequency band 5.4 to 7.2 GHz, and has two antenna arrays
organized vertically and horizontally, each equipped with 12 antennas. The antenna arrays provide angular resolution and  FMCW provides depth resolution~\cite{adib20143d}.


\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{rf-heatmaps}
\end{center}
\vspace{-10pt}
\caption{Illustration of RF signals expressed as a pair of horizontal and vertical heatmaps, and an RGB image recorded at the same time. Red color refers to high signal power and blue refers to low power.}\label{fig:rf-heatmaps}
\vspace{-15pt}
\end{figure}

The output of the radio consists of two sets of 2D heatmaps: horizontal heatmaps from the horizontal array, and vertical heatmaps from the vertical array. We illustrate these two kinds of heatmaps in Figure \ref{fig:rf-heatmaps}. The horizontal heatmap is a projection of the radio reflections on a plane parallel to ground, while the vertical heatmap is a projection of the reflections on a plane perpendicular to ground. We refer to a pair of horizontal and vertical heatmaps as RF frame.  The radio generates 30 pairs of heatmaps per second, i.e., 30 RF frames per second. 

From Figure \ref{fig:rf-heatmaps}, it is clear that RF heatmaps are significantly different from RGB images. Only the regions near the hotspots corresponding to humans have useful informations, other places may have irrelevant background noises (light blue dots), and reflections from other objects in the environment (other smaller hotspots). 

Further, given the specularity of RF signals within this frequency range, mirror-reflections will be more likely to happen than diffuse-reflections. Therefore, for each time step, some parts of the human body will reflect the RF signal away from the radio, which makes them transparent to the receiver based on this single RF heatmap.

%Prior works has demonstrated the RF signals have the ability to capture human information and achieve superior performance in tasks like 3D human pose estimation, human action recognition, person reidentification and so on. We sketch the process for these RF-based human sensing systems here in Figure \ref{fig:previous}.

%
%\begin{figure}[h]
%\begin{center}
%\includegraphics[width=\linewidth]{previous}
%\end{center}
%\vspace{-10pt}
%
%\caption{}\label{fig:previous}
%\vspace{-15pt}
%\end{figure}
